Measuring User Experience Inclusivity in Human-AI Interaction via Five User Problem-Solving Styles

Motivations: Recent research has emerged on generally how to improve AI product user experiences, but relatively little is known about an AI product's inclusivity. For example, what kinds of users does it support well, and who does it leave out? And what changes in the product would make it more inclusive? Objectives: Our overall objective is to help fill this gap, investigating what kinds of diverse users an AI product leaves out, and how to act upon that knowledge. To bring actionability to our findings, we focus on users' diversity of problem-solving attributes. Thus, our specific objectives were: (1) to reveal whether participants with diverse problem-solving styles were left behind in a set of AI products; and (2) to relate participants' problem-solving diversity to their demographic diversity, specifically, gender and age. Methods: We performed 18 experiments, discarding two that failed manipulation checks. Each experiment was a 2x2 factorial experiment with online participants. Each experiment compared two AI products: one deliberately violating an HAI guideline and the other applying the guideline. For our first objective, we analyzed how much each AI product gained/lost inclusivity compared to its counterpart, where inclusivity was supportiveness to participants with particular problem-solving styles. For our second objective, we analyzed how participants' problem-solving styles aligned with their demographics, namely their genders and ages. Results & Implications: Participants' diverse problem-solving styles revealed six types of inclusivity results: (1) the AI products that followed an HAI guideline were almost always more inclusive across diversity of problem-solving styles than the products that did not follow that guideline-but the "who" that got most of the inclusivity varied widely by guideline and by problem-solving style...

==> 0-TODO-list.tex <==
%\tableofcontents



\begin{enumerate}

\item Increase guideline body font size



\item VOCAB
    \begin{enumerate}
    %\item VOCAB: We're not going to use cognitive style or cognitive diversity. Instead, problem-solving diversity. So the word "cognitive" should not appear much if at all (except in related work) DONE ON: Aug 15, 10am, Jimena.
   %\item VOCAB: a "problem solving style TYPE" is a TYPE. DONE ON: Aug 15, 1am, Jimena.\\
        % VOCAB: a problem solving STYLE is a VALUE. DONE ON: Aug 15, 1am, Jimena.\\
        % VOCAB: a problem solving style TYPE has a RANGE of problem solving styles. DONE ON: Aug 15, 1am, Jimena.\\
        % VOCAB: RANGE(S): use instead of  the words SPECTRUM, SPECTRA. DONE ON: Aug 15, 1am, Jimena.
    %\item VOCAB: Instead of ``insights'', we're doing ``categories''. DONE ON: Aug 15, 3pm, Elizabeth.
    %\item VOCAB: the words "triangulate"/"triangulation" should not be in this paper. DONE ON: Aug 15, 1pm, Elizabeth.
    %\item VOCAB: the phrases "end user" and "end-user" should not be in this paper. DONE ON: Aug 15, 10am. 
    %\item VOCAB: the word "lens" should not be in this paper. DONE ON: Aug 15, 1am.
    %\item VOCAB: "problem solving Style Disaggregation" vs. "Diversity Disaggregation" vs. "Actionable Diversity Disaggregation vs. "Diversity Disaggregation via problem solving Styles" vs. ...?? DONE ON: Aug 15, 3pm, Jimena.
   % \item VOCAB: "AI product" is the thing participants  evaluated.  Not "system", not "vignette", not "guideline", ... DONE ON: Aug 15, 10am.
    \item GENDER vocab: Genders are: Man, Woman, CIS, Trans, Non-Binary, Gender-Nonconforming (can be combined). (and we have to include "Intersex" too, because it was a choice on the demographics survey, but strictly speaking, it's not a gender.)  Sex and Sexualities are: L, B, G, I, ...  which people don't like to see called "Genders".
    %\item VOCAB: change from this cumbersome phasing "the experiment for Guideline 3" to "Guideline 3's experiment" DONE ON: Aug 15, 3pm, Jimena.
   % \item VOCAB: Be careful about "Whether" vs. "That".  We aim to show WHETHER inequities, etc., exist, not THAT they exist. DONE ON: Aug 15, 3pm, Jimena.
    \item VOCAB: Categories (like a class), instances of each category/all categories.
    %\item VOCAB: inclusivity or inclusiveness would be ok. But NOT "inclusion": it seems to be a STATE of being included, not an action/attribute that a product can have. DONE ON: Aug 15, 3pm, Jimena.
   % \item VOCAB: we don't want to talk about "designers".  Instead, if you want to refer to folks like that, call them "HAI practitioners". (why: designers are too specific. UX folks do a lot more than just design.) DONE ON: Aug 15, 3pm, Jimena.
\end{enumerate} %vocab
   
\item AUDITS
    \begin{enumerate}

    % \item *URGENT*: AUDIT - For boxplots, do nothing until the end of our workflow. We do one pass of the figures, making sure that (1) in the includegraphics, it's pointing towards the correct file and (2) that the most most most most recent files have been uploaded. Only then do we freeze the files and NEVER TOUCH THEM AGAIN.

    % \item AUDIT: Don't imply this paper is about "fairness" , except in the Discussion section. \\
    % Corrolary: So this means "fairness" should not appear, except in Background/Related and Discussion). DONE ON: Aug 11, 5pm.
    
    %\item AUDIT: The meta-story of results is, does problem-solving style reveal something interesting about HAI-UX?  (Don't drift from this -- if the reader has lost the thread of "what did problem-solving style do for my understanding here", we've flunked the audit). DONE ON: Aug 14, 4pm.

    %\item AUDIT: The paper should NEVER talk about which product users preferred.  \\
   % Why: we didn't set it up as a DV we're analyzing.  And if we do set it up, now we have to report on it all over the place. DONE ON: Aug 11, 5pm
    
    % \item AUDIT: this paper should never claim to be  defining CONCEPTS like equity, inclusion, etc. Instead, we are defining MEASURES of those concepts. DONE ON: Aug 11, 5pm

    % \item AUDIT MIND-READING: we shouldn't be making claims about what's in participants' heads. So, avoid words like ``participants hypothesized', ``in their minds'', etc. unless you give a specific quote showing them saying that they're hypothesizing/guessing/assuming X, or "in my mind, Y is true". DONE ON: Aug 11, 5pm.
    
    % \item AUDIT TENSE: Beware present tense: it should be used only for definitions (good: ''blue IS a color'') or accepted facts (good: ``the sky IS above the ground''), never for Results (good: ``participants ATE unhealthy diets'').   We know what Participants DID, but not what People DO. DONE ON: Aug 14, 2pm.

    % \item AUDIT OVERLY GENERAL STATEMENTS: We know what PARTICIPANTS did, but not what PEOPLE do and not what USERS do/did. DONE ON: Aug 14, 2pm.
    
    % \item AUDIT FIGURES: Make sure that when you are introducing figures, if they're doubly encoded (i.e., colour AND position), then you introduce it in the caption. DONE ON: Aug 14, 5pm.

    % \item AUDIT CAPTIONS: make sure every table/fig caption says (or points to other captions) what the colors and symbols/abbreviations mean. DONE ON: Aug 14, 5pm.

    % \item AUDIT SIGNIFICANCE: When writing about the statistical difference between two entities, make sure that you list \textit{both}. DONE ON: Aug 15, 4pm, Elizabeth.\\
    % BAD: The risk-averse had significantly lower enjoyment of apples (<<stats go here>>). 
    % \\GOOD: The risk-averse had significantly lower enjoyment of apples (<<stats go here>>) THAN THEIR RISK-TOLERANT PEERS DID.

    % \item AUDIT [h] put this in ALL the figures and tables and everything that floats around. Make sure fig/table end up on the same page (+-1) as the first ref to that fig/table. DONE ON: Aug 15, 4pm, Jimena.

    \item AUDIT If we refer to something in some other section anywhere in the paper, we have to make sure that that thing exists and is where we say it is.  
    \\ eg, "As we pointed out in the Introduction..." -- check, did we point that out in the intro? 
    \\ eg, "The Appendices include x" -- check, do they actually include x?

    \item AUDIT

    
    \end{enumerate} %audits

\item ORDER
    \begin{enumerate}

    %\item *** Always list the facets in the same order as the paper. (in tables, in text, in figures). DONE ON: Aug 15, 4pm, Jimena.
    \item *** talk about Violation before Application. We know it's bad, but we don't how inequitably bad violating these guidelines is. (Tell the reader this)  (UNLESS you give the reader a huge about-face because it's super-important to not follow that constraint.)
    %\item Woman before Man?? or Man before Woman??  Be consistent in all text, figures, tables, ... unless there's a really good reason to make an exception somewhere. DONE ON: Aug 15, 3pm, Jimena.
    %\item Abi before Tim. Be consistent in all text, figures, tables, ... unless there's a really good reason to make an exception somewhere. DONE ON: Aug 15, 3pm, Jimena.

    \end{enumerate} %order 

\item FIGURES and TABLES
   %  \begin{enumerate}
   %  \item in all figs, use *, **, *** to show different levels of signif, not just *. Why: (1) Readers expect it when they see "*"s to mark signif. (2) Much more convincing because looks more like real data. DONE ON: Aug 14, 5pm.
   %  %\item FIGURE CAPTIONS: Every  figure or its caption needs to explicitly say (1) which guideline, (2) which dependent variables, and (3) which facets are in this figure. AND (4) which of the boxplots shown in that figure are significant. DONE ON: Aug 15, 2pm, Jeramie.
   %  %\item TABLE CAPTIONS: Every table caption about those triangulations among Gnums (checkmarks about guideline findings) needs to explicitly clarify which facets and which dependent variables are being included, and what a checkmark means in terms of stat significance. DONE ON: Aug 15, 2pm, Jeramie.
   %  %\item CAPTIONS: Don't put the t-test stuff in the caption -- that belongs in the text. Instead, annotations in the fig/table entries themselves are enough with the right number of STARs, or say NS. DONE ON: Aug 14, 5pm.
   %  %\item ROWHEIGHTS: look into the row height stuff. Currently, there's a bunch of white space below each of the figures that's going to annoy reviewers.
   % % \item VERTICALLY center the guideline names in a cell. (ie, don't let them print at the bottom of that cell). DONE ON: Aug 15, 4pm, Jeramie

   %  \end{enumerate} %figures and tables

\item GRAMMAR and PUNCTUATION:
    % \begin{enumerate}
    % \item GRAMMAR: check demonstratives surrounding ``participants'' (who vs that) DONE ON: Aug 15, 4pm, Jeramie
    % % \item GRAMMAR: "i.e.," means "that is,".  "e.g.," means "for example, " -- it appears that they may both being used to try to say "for example". DONE ON: Aug 15, 4pm, Jeramie
    % % \item GRAMMAR: The word ``data'' is plural.  \\BAD: ``This data is interesting.'' \\GOOD: ``These data are interesting.'' or ``The data are interesting.'' DONE ON: Aug 15, 4pm, Jeramie
    % % \item GRAMMAR: invalid grammar to use a citation be the subject of a sentence or clause.  
    % % \\BAD: [Kulesza 2015] reported that birds fly. \\GOOD: Kulesza reported that birds fly [Kulesza 2015].\\
    % % \item PUNCTUATION: Use M-dashes (like this: ---), not N-dashes (like this: --).  N-dashes belong ONLY in numeric ranges (like 3--16).\\
    % % \item PUNCTUATION: the periods are often messed up for our participant quotes. DONE ON: Aug 15, 3pm, Jimena. \\BAD: ``The birds are flying.'' (R94). \\BAD: ``The birds are flying.'' (R94) \\GOOD: ``The birds are flying'' (R94).
    % % \\BEST: I think its clearer and better with the Participant ID first, like this: \\(R94): ``The birds are flying.''\\

    % \end{enumerate} %grammar and punctuation
    
    \item WRITING WELL
    \begin{enumerate}
   
    \item TOPIC SENTENCE: is the 1st sentence a good topic sentence?  \\
    GOOD: "To answer RQs 1 \& 2, we". \\
    BAD: "Figure 4a (top) shows..." (starts out well, but then:) "...that participants had a wide variety of responses." (Bad if the parag's point isn't going to be  "wide variety").
    \item WRITING NIT: ``There are'' is a particularly weak way of writing a sentence.  \\
    Bad: ``There are bad apples in this barrel.''  Good: ``This barrel has bad apples.''\\
    Bad: ``There were situations in which participants ate the bad apples anyway.''  Good: ``In some situations, participants ate the bad apples anyway.''
    \item WRITING NIT: ``Only'' goes as close as possible to the thing it's "ONLYing"!  (eg: "I only eat pears." BAD if you mean pears are the only thing you eat. GOOD if the only thing you do with pears is eat them.
    \item WRITING CONSIDERATION TO THE READER: If you must refer to a table in the appendix, say so. (e.g., instead of ``Table 8'', say ''Appendix Table 8'' or some such.)

    \end{enumerate} %writing rules

\item Spell check\\
\item Global search ``FIXME'' 
\item Global search "**"
\item ADD IN THOSE PAPERS THAT WERE SENT A WHILE AGO.
\end{enumerate}


\clearpage


\setcounter{fixmeTotalCounter}{0}



==> doc/ZZZ-More-Leftovers.tex <==
\FIXME{MMB to AAA: please move the following old obsolete stuff to leftovers.  It's really hard for me to make sense of the paper with these things in there.}





\boldify{But why was there no change? In this case, it was \textit{because} the inclusiveness had not changed.}

Inequities in the \appProduct{} is a less-than-ideal outcome for HAI practitioners, but investigating user experience inclusiveness helps to make sense of this phenomenon.
As the right column of Table~\ref{tab:no-equity-or-inclusiveness} suggests, the \textit{largest} user experience change between the \vioProduct{} and \appProduct{} in these seven instances was the risk-averse participants' feeling secure (-0.464), and even this change was not statistically significant (t(26) = 0.9874, \textit{p} = 0.333, \textit{d} = .181).
This suggests that the inequities found in the \appProduct{} were a direct result of the proposed changes not inclusively meeting the needs of the risk-averse participants.







\boldify{However, it's not what it looks like! It's not that applying these guidelines is bad, just that applying them is better for some (look at the new table's inclusiveness column!) Looking at inclusiveness, the first reason was that applying these guidelines was good for both risk attitudes but better for one}

\FIXME{MMB to AAA -- this subsection is not about inequities.  Please delete everything from here down or move it into equities subsection***}

Investigating inclusiveness once more helped to make sense of \textit{why} these inequities formed, and it was not because the \vioProduct{} was ``better'' than the \appProduct{}.
Instead, as in this example (Table~\ref{**FIXME**}, top row, third column), both the risk-averse \textit{and} risk-tolerant participants' average response significantly increased between Guideline 9's \vioProduct{} and \appProduct{} (risk-averse: t(25) = 2.8859, \textit{p} = 0.008, \textit{d} = 0.568; risk-tolerant: t(30) = 5.7868, \textit{p} $<$ .0001, \textit{d} = 1.029).
These results illustrate that these risk-averse participants received only \textit{half} of the benefit to their feelings of productivity than their risk-tolerant peers.
    This suggests for the HAI community that although violating these guidelines is clearly worse overall than applying them, some designs intended to apply the guidelines may benefit some more than others, resulting in an inequitable user experience for people with diverse attitudes toward risk.

\boldify{Another reason this inequity formed was that the application was good for one but not worse for the other!}




%-----------------------------------------------



% \FIXME{I think there's an implications for research here. This is showing that for any dependent variable, you can understand it further by disaggregating by problem solving style. It's not about the specific guideline but rather how to further understand your data.}


\boldify{After we define equity, look at Table~\ref{fig:G8-illustrative-example}. You can see from that middle column that the \appProduct{} is equitably good compared to the \vioProduct{}, which highlights for designers another reason why they should avoid violating the guidelines and actively apply them.}



% Figure~\ref{fig:risk-agg} (top) shows that participants had a wide variety of responses to whether or not they agreed that they would feel suspicious of the product's intent, action or outputs with Guideline 8's \vioProduct{}.
% However, as Li et al.~\cite{li-MSR-work} reported, participants clearly felt less suspicious with Guideline 8's \appProduct{} (bottom), highlighting that applying the guidelines is better than violating overall (i.e., before considering attitudes toward risk).
% A paired t-test corroborates this finding (t(60) = 4.4063, p $<$ .0001).

% In Section~\ref{sec:Results-Insights}, the hatched , white boxes represent \textit{all} participants' responses (i.e., without considering attitudes toward risk) to the \vioProduct{} for that dependent variable in that experiment.
% Similarly, the solid white boxes (Figure~\ref{fig:risk-agg}, bottom) represent all participants' responses to the \textit{\appProduct{}} in that experiment.





% In this work, we define equity in the following way: 
% To show that using this definition of equity will empower HAI practitioners, we look at how these participants' responses changed between the \vioProduct{} and \appProduct{}.
Throughout this paper, we measure user experience equity in the following way:
``\textit{For any user experience dependent variable in any AI product, the user experience between two groups of participants is equitable if no statistically significant differences exist between the participants' average responses. }''
As such, significant differences in the \vioProduct{} or the \appProduct{} indicate the presence of user experience inequity\footnote{Two-sample t-tests used to test differences between diverse participants' averages in the \vioProduct{} and \appProduct{} independently.}.
% Results like these show that not only is violating Guideline 8 (i.e., to \textit{not} support efficient dismissal) bad from a design-practices perspective  but also that violating Guideline 8 may be inequitably bad to the user experience between risk-averse and risk-tolerant participants in human-AI interaction.

\input{tables/04-Equity-Risk-Walkthrough}
% Such inequities are similar to the algorithimic unfairness  ``quality-of-service'' harm identified by other researchers~\cite{bird2020fairlearn}, except in this paper, these are \textit{user experience} unfairness harms instead.




% \boldify{However, consider the aplication product... it resolved the inequity, and it wasn't the only time}

% The \appProduct{} made the button to dismiss the AI feature visible for participants, and this change statistically resolved the user experience inequity between the risk-averse and risk-tolerant participants with only a \textit{small} effect size (t(59) = -1.2474, p = .217, d = .322).
% This suggests in this case that not only is applying Guideline 8 a good idea for user experiences, it is an \textit{equitably} good idea to support those with diverse attitudes toward risk.


% shows the four guidelines where this ideal outcome occurred---achieving user experience equity between participants with two diverse problem-solving styles by applying the guidelines.

% This pattern shows what it means to achieve the ideal outcome of applying some guidelines---improving inclusivity \textit{and} achieving equity.
% A guideline exhibited this pattern if there was a statistically significant difference between the 
% \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} and \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants in the \vioProduct{}, but there was no significant difference between the two risk attitudes in the \appProduct{} for at least one dependent variable.
% The four instances of this pattern were in Guidelines 4, 7, 8, and 11. 





\boldify{We can see that it happened in different dependent variables too! Like violating guidelines $\implies$ control inequity, and applying the guideline fixes it!}


This user experience equity phenomenon occurred **FIXME** times across both multiple experiments and dependent variables, and both the risk-averse and risk-tolerant participants were disadvantaged across these instances (Table~\ref{tab:equity-and-inclusiveness-improve}).
For example, in  Guideline 7's experiment (top row), the button to invoke the AI-powered feature in the \vioProduct{} was not visible to these participants, and this created an inequity between the risk-averse and risk-tolerant participants' feelings \textit{of control} (t(56) = 2.7112, p = .009, d = .714).
Fitting the definition of this pattern, the inequity between these participants with diverse attitudes toward risk no longer existed in the \appProduct{}  (t(56) = 1.3941, p = .169, d = .368).
However, unlike in Figure~\ref{fig:G8-illustrative-example}, notice that the risk-averse participants felt significantly \textit{more} in control than their risk-tolerant peers.
In all of the experiments, the \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} were inequitably disadvantaged in only five instances.
With so little data, it remains an open question on what the risk-tolerant may need to close user experience inequities between them and the risk-averse when some guidelines are violated.

\input{tables/15-Applications-Improved-Equity}



% Figure~\ref{tab:equity-improved} provides additional examples of this in the experiments for Guideline 7 (top row) and Guideline 11 (bottom row).
% Demonstrating that these inequities , the \vioProduct{} for Guideline 7 caused a user experience inequity where the risk-averse participants had a significantly \textit{higher} feeling of control than the risk-tolerant participants (t(56) = 2.7112, p = .009, d = .714)


% For the risk-averse and risk-tolerant participants in Guideline 7's experiment, the \vioProduct{} created a user experience inequity but in their feelings \textit{of control}.
% The \appProduct{} resolved this inequity between 
% Additionally, in this case,  the \vioProduct{} for Guideline 7 caused a user experience inequity where the risk-averse participants had a significantly \textit{higher} feeling of control than the risk-tolerant participants (t(56) = 2.7112, p = .009, d = .714)%
% \footnote{Appendix~{\color{blue}\href{https://web.engr.oregonstate.edu/~anderan2/MSR-Appendices/Appendix-Boxplots.pdf}{D}} has all statistics for all tests we ran.}. %
% %        End Footnote
% %= .716)
% %, and the \appProduct{} closed this disparity.
% The \appProduct{} for Guideline 7 made the button to invoke the AI-powered feature visible, and similar to before, the \appProduct{} statistically resolved this inequity between these two sets of participants, with only a small effect size (t(56) = 1.3941, p = .169, d = .368).

% \boldify{What I want you to notice is that of these identified inequities, very rarely were the risk-tolerant left behind. We don't know what they need (they're often not the ones unsupported), leaving it an open question!}

% %Begin FIXED
% \FIXED{
% When considering this closure of user experience inequity in these data, there is one important observation to note;
% across the 32 equity insights discovered in this investigation, the \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} were inequitably disadvantaged instead of the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} in only five instances.
% With so little data, it remains an open question on what the risk-tolerant may need to close user experience inequities between them and the risk-averse when some guidelines are violated.
% %End FIXED
% }

\boldify{There was a second equity and inclusiveness insight in these data, where applying the guideline didn't change equity BECAUSE inclusiveness didn't changed. This happened 13/32 times, but Guideline 4 was by far the most prevalent. }

A second user experience equity pattern emerged in these data and occurred 13 times, where user experience equity did not change between the two products.
This pattern was defined by a statistically significant user experience difference between the risk-averse and risk-tolerant participants in \textit{both} the \vioProduct{} and \appProduct{}.


\input{tables/16-Inequities-Remain}

\boldify{Consider participants' responses to the ``I would feel secure'' DV. Notice that the risk-averse participants felt significantly less secure with the \vioProduct{}? It remained in the \appProduct{}}

Of the 13 identified cases, \textit{seven} of them arose in Guideline 4's experiment\footnote{Guideline 4's text: \textit{Show contextually relevant information}}.
In this experiment, the \vioProduct{} did not provide contextually relevant information by showing only a standard list of possible definitions taken from a popular acronym dictionary (as opposed to ``...\textit{definitions that are used in [the] workplace and pertain to the topic of the current document}'').
Table~\ref{tab:no-equity-or-inclusiveness} shows the risk-averse and risk-tolerant participants' responses to the seven statements.
In every instance of these seven, there was an inequitable user experience between the risk-averse and risk-tolerant participants;
the risk-averse participants \textit{always} had a the significantly lower user experience.
For example, the risk-averse reported that they would feel significantly less secure than their risk-tolerant peers (t(62) = -2.3006, p = .025, d = .575).
Similarly, they also felt significantly less adequate (t(61) = -2.9179, \textit{p} = .005, \textit{d} = .743) than the risk-tolerant participants\footnote{All statistical test results can be found in Appendix **FIXME**}.
Although the \appProduct{} did provide the workplace definitions, the design changes did not change  user experience inequity change;
the risk-averse participants \textit{still} felt significantly less secure (t(61) = -3.1984, \textit{p} = .002, \textit{d} = .814) and adequate (t(62) = -2.4955, p = .015, d = .629) than the risk-tolerant participants.





\boldify{The third and last user experience equity and inclusiveness pattern occurred 14 times, and was a most unexpected result---equity \textit{decreased} when the guidelines were \textit{applied} (see the new table) }

Considering participants' attitudes toward risk also uncovered a third and final pattern in user experience equity that was the most unexpected---the \vioProduct{} seemed to be \textit{more} equitable to participants' user experience than the \appProduct{}.
This pattern was defined by \textit{no} statistically significant user experience difference in the \vioProduct{} which \textit{became significant} in the \appProduct{}.
Table~\ref{**FIXME**} shows examples of this pattern from multiple experiments.
For example, consider participants' responses to how productive they would feel with Guideline 9's \vioProduct{} (top row).
In this case, both the risk-averse and risk-tolerant participants felt that they would be similarly productive with the product (t(55) = 0.4391, \textit{p} = .662, \textit{d} = .117).
However, a user experience inequity formed for these same participants when they saw the \appProduct{};
the risk-averse participants felt that they would be significantly less productive (t(56) = -2.1404, \textit{p} = .037, \textit{d} = .559) with the \appProduct{} than their risk-tolerant peers did.
This equity decrease pattern occurred 11 times across six experiments in these data.

\input{tables/17-Equities-Form}



% \boldify{There was another flavour of this lack of equity change, and it's when the \appProduct{} inclusively improved the user experience but at the SAME RATE, which is progress but more is needed to understand how to meet these needs.}






\emph{Implications for Researchers and Practitioners: } %Pattern \#1
For practitioners, considering participants' attitudes toward risk while analyzing their quantitative and qualitative data can provide actionable avenues to apply these guidelines.
For example, when participants were asked to explain which of the two systems they preferred, some of the risk-averse participants' responses suggested \textit{how} designers may better support efficient invocation (i.e., Guideline 7) by ensuring that the invocation method is easy to locate:
\quotateInset{I like that [the Application AI product's feature] is easy to locate ... nothing more frustrating than trying to find something and not being able to...}
{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G7-2138-risk-averse}}{}{I like the idea of getting suggestions or being able to access suggestions when none pop up.  I like that it is easy to locate because there is nothing more frustrating than trying to find something and not being able to find it.}

Further, some participants sent warning signals to designers about their experiences when explanations were not provided in the \vioProduct{} for Guideline 11:

\quotateInset{[Violation AI product] would be a call to the help desk and a big time suck...}{}{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G11-2921-risk-averse}}{I believe I could pinpoint any insights with lone. Kelso would be a call to the help desk and a big time suck if there was inaccurate data.}

G7-2138-risk-averse's and G11-2921-risk-averse's comments are reminiscent of Blackwell's theory of Attention Investment~\cite{blackwell2002first}.
In this theory, users weigh their expectation of the cost of learning/using the new feature set against their expectation of benefits they will receive (including time saved)---tempered by their expectation of risk (probability) that spending that time will not result in benefits after all. 
This is pertinent within AI-powered systems, since not only are risk-averse users often hesitant to spend extra time learning unfamiliar technologies~\cite{charness2012strong}, but users can also become wary of accessing features of AI-powered technologies where there is a high perceived cost of obtaining uncertain benefits from using them~\cite{bunt2012explanations}.

As such, a possibility is to empower users to ``guess-timate'' cost/benefit/risk trade offs reasonably correctly.
To accomplish this, designers may have to design for users' expectations of the trade offs between accepting an AI's decision (expecting low cost, potentially good benefits if the AI is right, but potentially high risk it is wrong), vs. arriving at the decision themselves (expecting higher cost for the same benefits, at lower risk if they trust themselves).
If designers do not consider how to help users' expectations align reasonably well with the AI feature's actual costs, benefits, and risk, risk-averse users could choose to avoid using the AI feature, opting to do the work themselves to reduce risks arising if the AI makes an inappropriate decision.

\boldify{One explanation for \textit{why} this equity gap closed was that the \appProduct{} was inclusively good for participants with diverse attitudes toward risk. Let's show you what I mean.}


One possible explanation for this is that the \appProduct{} was equitably good because it was also \textit{inclusively good} for these participants.
As such, for a single group of participants with diverse problem-solving styles, a significant differences their responses for  the \vioProduct{} and the \appProduct{} indicate the presence of user experience inequity\footnote{Paired t-tests used to test significant differences for participants' responses between the \vioProduct{} and \appProduct{}.}.
The right column of Table~\ref{fig:G8-illustrative-example} shows how participants' feelings of suspicion changed between Guideline 8's two \vioProduct{} and \appProduct{}, in the same ordering as the boxplots (i.e., all participants, risk-averse, risk-tolerant).
Both the risk-averse (t(25) = 3.2354, \textit{p} = .003, \textit{d} = .635) and risk-tolerant (t(34) = 3.002, \textit{p} = .005, \textit{d} = .507) participants' suspicions of the product's intent, action, or outputs were significantly reduced, but the risk-averse received enough benefit from the \appProduct{} to close the equity gap.




% We define a guideline as exhibiting this pattern if 1)~the \vioProduct{} did not significantly differ between the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} and \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants; 2)~participants with both attitudes towards risk were more positive in the {\appProduct{}}, i.e.,  inclusivity improved; but 3)~\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} and \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants then statistically differed in the \appProduct{}.
% Thus, in this pattern, the \appProduct{} results were better for everyone, but also introduced an inequity.

\clearpage

%\input{tables/12-One-More-Than-Other}



























%-------------------------------}

\boldify{Consider Table~\ref{tab:one_helped_more}, which illustrates another data phenomenon. 
In these cases, participants on both ends of the spectrum's averages improved between Violation and Application AI products, but one end of the spectrum was helped more, thus inadvertently introducing a gap. }

Like Pattern \#1, this inclusivity pattern is an indicator of progress.
In Pattern \#2, applying the guideline resulted in improved inclusivity;
however, unlike Pattern~\#1, this improvement did not achieve equity.
We define a guideline as exhibiting this pattern if 1)~the \vioProduct{} did not significantly differ between the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} and \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants; 2)~participants with both attitudes towards risk were more positive in the {\appProduct{}}, i.e.,  inclusivity improved; but 3)~\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} and \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants then statistically differed in the \appProduct{}.
Thus, in this pattern, the \appProduct{} results were better for everyone, but also introduced an inequity.

Of the three patterns, this pattern occurred the most frequently, with 16 instances arising over eight of the experiments.
Figure~\ref{tab:one_helped_more} shows an instance of Pattern \#2 from each of these experiments.




For example, in Guideline 4's experiment (left), the risk-averse and risk-tolerant participants' rated the \vioProduct{} similarly useful on average (i.e., the distance between their average ratings was less than 0.5).
Although both the risk-averse and risk-tolerant participants rated the usefulness of the \appProduct{} higher on average, the risk-averse participants benefited less than the risk-tolerant: risk-averse participants reported the \appProduct{} to be significantly less useful (t(63) = -2.9810, p = .004, d = .744) than their risk-tolerant peers did.
Guideline 4 is discussed in more detail in Section~\ref{sec:category-3}, expanding upon why such patterns may have arisen in these data.

Across the eight experiments exhibiting this pattern, two dependent variables were especially common: the ``I perceived it as useful'' (Guidelines 4, 9, 10, and 18) and ``I would feel adequate'' (Guidelines 5, 11, 13, and 15) dependent variables.
This raises the possibility for practitioners that, when evaluating user experiences after applying some of the guidelines in an AI product, these dependent variables may have particular pertinence to whether that design is inclusive across the full range of users' diverse attitudes toward risk.

%Begin FIXED
\FIXED{
\emph{Implications for Researchers and Practitioners: } %Pattern \#2
The 16 occurrences of Pattern~\#2 reveal two implications.

First, users' diverse attitudes toward risk can affect their experiences in multiple ways, as the significant differences across multiple dependent variables show.
For researchers and practitioners who analyze user data, this points out the need to analyze user data by not only diversity \textit{input} variables (here, attitude toward risk) but also by multiple \textit{outcome} variables (e.g., feeling of control).

Second, even when a design change is an inclusivity ``win'' by helping users with diverse values across the risk problem solving style type, inequities can remain or even emerge as the result of the change.
This points out that improving inclusivity for the whole risk spectrum is not the only goal---the other goal is for the user experience to be equitable across the risk spectrum.  
%End FIXED
} 

%------------------------------

\boldify{The last category of insight was Persistent disparities, exemplified in G4.}

The last inclusivity pattern occurred when the  \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} and \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants differed significantly from each other in their ratings, in \textit{both} the \vioProduct{} and the \appProduct{}.

Participants in Guideline 4's experiment (``show contextually relevant information'') exhibited this pattern in six dependent variables (Figure~\ref{fig:third-category-guideline-4}).
%The six instances of dependent variables with this last category of insight are highlighted in the top and bottom halves of Table~\ref{tab:G4-Stats} (p-value column).
In fact, in this experiment the risk-averse participants always gave significantly lower ratings than the risk-tolerant participants in both the \vioProduct{} (Table~\ref{tab:G4-Stats}, top, p-value column) {and} the \appProduct{} (bottom).
Even with Bonferroni corrected p-values (sixth column), the risk-averse participants felt significantly less certain with the \vioProduct{} (t(62) = 3.6258, $p = .005$, d = .910) and with the \appProduct{} (t(63) = 4.7513, $p < .001$, d = 1.186) than the risk-tolerant participants did.
The same pattern also manifested in their responses to the ``I would be suspicious'' dependent variable.

%\boldify{Li et al. also found that G4 had its problems, and participants on both sides of the attitudes toward risk spectrum held similar concerns.}


\FIXME{Unhoused Implications from 4.1 starts here}


\emph{Implications for Researchers and Practitioners:}
The results of disaggregating in this particular case have three implications.

First, disaggregating by problem solving style value can help researchers and designers answer questions about mysterious peaks and valleys in HAI user experience data.
For example, the results suggests that violating Guideline~11 (i.e., \textit{not} explaining why the AI Product did what it did) may result in users who are more risk-averse in using technology viewing such products much less favorably than users who are risk-tolerant.

% \FIXME{AAA@MMB: Really didn't like the ``data from users who are risk-averse...'' verbiage. I tried applying Zinsser to this and hope I didn't break anything.}

Second, disaggregating data by participants' attitude toward risk helped to explain these data, pointing the way toward potential design remedies that HAI designers can consider to help improve more users' experiences with the product, or at least clarify what additional data needs to be collected from user studies.
In the Guideline~11 vignette, the \appProduct{} offered an explanation \textit{button}, but participants did not see the actual explanation. 
Here, risk-tolerant individuals felt in control just from knowing an explanation would be available, but risk-averse individuals may have needed to see what the explanation would actually explain before they could feel in control.

Finally, an implication from these results for designers of AI products is that failing to follow Guideline~11 by providing an explanations of the AI's outputs may lead risk-averse users to abandon the AI-powered feature because they may not feel in control.

\FIXME{Unhoused implications from 4.1 ends here}
%Begin FIXED
\FIXED{
\emph{Implications for Researchers and Practitioners:}
These six instances of Pattern~\#3 suggest that sometimes applying such guidelines is not enough to meet the needs of risk-averse participants.
In this experiment, one possible reason for the risk-averse participants' lower ratings might have arisen over concerns about privacy with the \appProduct{}:

\quotateInset{I would prefer to use [Violation AI product] because [Application AI product] feels a bit more intrusive. I would be nervous that [Application AI product] is pulling data from things like my other software and my browsing history.}
{}
{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G4-3905-risk-averse}}
{Whole quote - I would prefer to use Ione because Kelso feels a bit more intrusive. I would be nervous that it is pulling data from things like my other software and my browsing history. This would be unacceptable since I work with sensitive PII.}


For designers, one possible way to address such privacy concerns may be using AI explanations to increase transparency into how the system makes its decisions.
For example, Lim \& Dey's ``inputs'' and ``outputs'' intelligibility types~\cite{lim2019these} provide one possible direction.
Mueller et al.~\cite{mueller2019explanation} provide a compilation of works from the eXplainable AI (XAI) literature with other possible directions.

\input{figure/07-All-Boxes/Risk/03-G4}
\input{tables/Risk/2-G4-PostStrat}

\boldify{Dear reader, we had enough evidence to demonstrate that \newline H1-CognitiveDiversity-RiskStyle held; it was in fact the case that the risk-averse users' user experiences were more frequently disparately impacted across the 16 experiments than their risk-tolerant peers.}

Overall, Sections~\ref{subsec:why-disaggregate} and~\ref{subsec:3-categories} have shown the data repeatedly supported \textbf{H1-CognitiveDiversity-RiskStyle}.
10 of the dependent variables in the Guideline~4 experiment exhibited instances of all three patterns; Table~\ref{tab:G4-Stats} shows all the results from that experiment.
Complete results from the remaining experiments are given in Appendix~\href{https://web.engr.oregonstate.edu/~anderan2/MSR-Appendices/Appendix-Boxplots.pdf}{{\color{blue}D}}.
Across all experiments, the data revealed a total of 33 disparities between risk-averse and risk-tolerant human-AI interaction participants. 

Of these 33 instances, in 30 of them (90.9\%) the risk-averse participants rated the AI products significantly lower than the risk-tolerant participants did.
This suggests that when designers apply the guidelines for human-AI interaction, additional considerations beyond the guidelines may be needed to reduce inclusivity gaps among users who have diverse attitudes toward risk in using technology.

%End FIXED
}


\FIXME{MMB to AAA: see ** above}

\subsection{Beyond the Illustrative Case: RQ1 Results
\draftStatus{MMB thinks...?}} 
\label{subsec:3-categories}

\FIXME{C - Improved inclusivity and equity

V - Improved inclusivity but not equity

P - As inclusive and equitable to vio/apply

Report on equity and inclusion, have Elizabeth help me with classifying these}

Although Section~\ref{subsec:why-disaggregate} provided an illustrative example of whether and how applying \textit{one} guideline impacted user experience fairness (i.e., equity and inclusiveness) for participants with diverse problem-solving styles.
\textbf{RQ1} seeks to understand such phenomena across \textit{16} guidelines.  
%Do results like those in Section 4.1 extend beyond that single case?
%\textbf{H1-CognitiveDiversity-RiskStyle} hypothesizes that risk-averse and risk-tolerant HAI users' experiences will exhibit disparities in UX metrics for human-AI interaction across experiments.
To answer this, we considered every dependent variable in each of the 16 experiments, disaggregating participants' data by their attitudes toward risk.
This disaggregation by risk revealed 37 user experience fairness instances across **FIXME** categories.


% \subsubsection{Pattern \#1: Applying Guidelines Improved Inclusivity \& Equity}
% \label{subsec:category-1}

\boldify{The first category shows the promise for applying the guidelines. Here's the criteria for this category, as well as where we found it and walking through an example of it.}

The example illustrated in Figure Section~\ref{subsec:why-disaggregate} appeared
Instances of the first user experience fairness category were uncovered when applying the guidelines significantly improved inclusiveness but not equity, similarly to Section~\ref{subsec:why-disaggregate}'s results.
However, instances of this category arose 
This pattern shows what it means to achieve the ideal outcome of applying some guidelines---improving inclusivity \textit{and} achieving equity.
A guideline exhibited this pattern if there was a statistically significant difference between the 
\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} and \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants in the \vioProduct{}, but there was no significant difference between the two risk attitudes in the \appProduct{} for at least one dependent variable.
The four instances of this pattern were in Guidelines 4, 7, 8, and 11. 

Figure~\ref{tab:applications_closed_gaps} (left) shows an instance of this pattern for Guideline 7's dependent variable of feeling in control.
In contrast to the Guideline 11 case with this variable shown in Section~\ref{subsec:why-disaggregate}, with Guideline 7 the risk-averse participants felt significantly \textit{more} in control on average than the risk-tolerant participants when seeing the \vioProduct{} (t(56) = 2.7112, p = .009, d%
%        Begin Footnote
\footnote{Cohen's d measures practical significance~\cite{ramsey2012statistical}, where $d < .2$ is unsubstantiated, $d \in [0.2, 0.5)$ is small, $d \in [0.5, 0.8) = $ medium, and $d \geq 0.8 $ is large} = .538)% 
%        End Footnote 
%        Begin new Footnote
\footnote{Appendix~{\color{blue}\href{https://web.engr.oregonstate.edu/~anderan2/MSR-Appendices/Appendix-Boxplots.pdf}{D}} has all statistics for all tests we ran.}. %
%        End Footnote
%= .716)
%, and the \appProduct{} closed this disparity.
(The difference between the \vioProduct{} and \appProduct{} was that the button to toggle the AI-powered feature was visible in the \appProduct{} but not in the \vioProduct{}.)
Similar to the Guideline 11 case (statistical details in Appendix~\href{https://web.engr.oregonstate.edu/~anderan2/MSR-Appendices/Appendix-Boxplots.pdf}{{\color{blue}D}}), Guideline 7's \appProduct{} closed the disparity statistically between these two sets of participants  with a small effect size (t(56) = 1.3941, p = .169, d = .368).
%Begin FIXED
\FIXED{
Across the 16 experiments, this was one of only three instances where the risk-averse participants had a significantly higher average rating for a dependent variable than the risk-tolerant.
This highlights for researchers and practitioners the importance of considering the needs on \textit{both} ends of the attitudes toward risk problem solving style type.
The infrequency of results where the risk-averse did not have significantly lower UX metrics leaves it an open question on what the risk-tolerant may need to avoid disparities between them and the risk-averse when some guidelines are violated.
%End FIXED
}




Guideline 8's experiment (Figure~\ref{tab:applications_closed_gaps}, right), showed this statistical pattern with a different variable: the risk-averse participants felt significantly more \textit{suspicious} of the \vioProduct{} (t(59) = -2.1958, p = .032, d = .569) than the risk-tolerant did.
Appendix~\href{https://web.engr.oregonstate.edu/~anderan2/MSR-Appendices/Appendix-Boxplots.pdf}{D} also shows this pattern statistically in Guideline 4 participants' feelings of productivity.
%Begin FIXED
\FIXED{

\emph{Implications for Researchers and Practitioners: } %Pattern \#1
For practitioners, disaggregating participants' quantitative and qualitative data by their attitudes toward risk can provide actionable avenues to apply these guidelines.
For example, when participants were asked to explain which of the two systems they preferred, some of the risk-averse participants' responses suggested \textit{how} designers may better support efficient invocation (i.e., Guideline 7) by ensuring that the invocation method is easy to locate:
\quotateInset{I like that [the Application AI product's feature] is easy to locate ... nothing more frustrating than trying to find something and not being able to...}
{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G7-2138-risk-averse}}{}{I like the idea of getting suggestions or being able to access suggestions when none pop up.  I like that it is easy to locate because there is nothing more frustrating than trying to find something and not being able to find it.}

Further, some participants sent warning signals to designers about their experiences when explanations were not provided in the \vioProduct{} for Guideline 11:

\quotateInset{[Violation AI product] would be a call to the help desk and a big time suck...}{}{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G11-2921-risk-averse}}{I believe I could pinpoint any insights with lone. Kelso would be a call to the help desk and a big time suck if there was inaccurate data.}

G7-2138-risk-averse's and G11-2921-risk-averse's comments are reminiscent of Blackwell's theory of Attention Investment~\cite{blackwell2002first}.
In this theory, users weigh their expectation of the cost of learning/using the new feature set against their expectation of benefits they will receive (including time saved)---tempered by their expectation of risk (probability) that spending that time will not result in benefits after all. 
This is pertinent within AI-powered systems, since not only are risk-averse users often hesitant to spend extra time learning unfamiliar technologies~\cite{charness2012strong}, but users can also become wary of accessing features of AI-powered technologies where there is a high perceived cost of obtaining uncertain benefits from using them~\cite{bunt2012explanations}.

As such, a possibility is to empower users to ``guess-timate'' cost/benefit/risk trade offs reasonably correctly.
To accomplish this, designers may have to design for users' expectations of the trade offs between accepting an AI's decision (expecting low cost, potentially good benefits if the AI is right, but potentially high risk it is wrong), vs. arriving at the decision themselves (expecting higher cost for the same benefits, at lower risk if they trust themselves).
If designers do not consider how to help users' expectations align reasonably well with the AI feature's actual costs, benefits, and risk, risk-averse users could choose to avoid using the AI feature, opting to do the work themselves to reduce risks arising if the AI makes an inappropriate decision.
%End FIXED
}

%-------------------------------
\subsubsection{Pattern \#2: Applying Guidelines Improved Inclusivity, but Not Equity}
\label{subsec:category-2}
\draftStatus{MMB says draft status is now 2.75-3ish?}

\boldify{Consider Table~\ref{tab:one_helped_more}, which illustrates another data phenomenon. 
In these cases, participants on both ends of the spectrum's averages improved between Violation and Application AI products, but one end of the spectrum was helped more, thus inadvertently introducing a gap. }

Like Pattern \#1, this inclusivity pattern is an indicator of progress.
In Pattern \#2, applying the guideline resulted in improved inclusivity;
however, unlike Pattern~\#1, this improvement did not achieve equity.
We define a guideline as exhibiting this pattern if 1)~the \vioProduct{} did not significantly differ between the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} and \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants; 2)~participants with both attitudes towards risk were more positive in the {\appProduct{}}, i.e.,  inclusivity improved; but 3)~\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} and \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants then statistically differed in the \appProduct{}.
Thus, in this pattern, the \appProduct{} results were better for everyone, but also introduced an inequity.

Of the three patterns, this pattern occurred the most frequently, with 16 instances arising over eight of the experiments.
Figure~\ref{tab:one_helped_more} shows an instance of Pattern \#2 from each of these experiments.

\input{tables/12-One-More-Than-Other}


For example, in Guideline 4's experiment (left), the risk-averse and risk-tolerant participants' rated the \vioProduct{} similarly useful on average (i.e., the distance between their average ratings was less than 0.5).
Although both the risk-averse and risk-tolerant participants rated the usefulness of the \appProduct{} higher on average, the risk-averse participants benefited less than the risk-tolerant: risk-averse participants reported the \appProduct{} to be significantly less useful (t(63) = -2.9810, p = .004, d = .744) than their risk-tolerant peers did.
Guideline 4 is discussed in more detail in Section~\ref{sec:category-3}, expanding upon why such patterns may have arisen in these data.

Across the eight experiments exhibiting this pattern, two dependent variables were especially common: the ``I perceived it as useful'' (Guidelines 4, 9, 10, and 18) and ``I would feel adequate'' (Guidelines 5, 11, 13, and 15) dependent variables.
This raises the possibility for practitioners that, when evaluating user experiences after applying some of the guidelines in an AI product, these dependent variables may have particular pertinence to whether that design is inclusive across the full range of users' diverse attitudes toward risk.

%Begin FIXED
\FIXED{
\emph{Implications for Researchers and Practitioners: } %Pattern \#2
The 16 occurrences of Pattern~\#2 reveal two implications.

First, users' diverse attitudes toward risk can affect their experiences in multiple ways, as the significant differences across multiple dependent variables show.
For researchers and practitioners who analyze user data, this points out the need to analyze user data by not only diversity \textit{input} variables (here, attitude toward risk) but also by multiple \textit{outcome} variables (e.g., feeling of control).

Second, even when a design change is an inclusivity ``win'' by helping users with diverse values across the risk problem solving style type, inequities can remain or even emerge as the result of the change.
This points out that improving inclusivity for the whole risk spectrum is not the only goal---the other goal is for the user experience to be equitable across the risk spectrum.  
%End FIXED
} 

%------------------------------
\subsubsection{Pattern \#3: Applying Guidelines Did Not Change Inclusivity}
\label{sec:category-3}
\draftStatus{MMB says ??**}

\boldify{The last category of insight was Persistent disparities, exemplified in G4.}

The last inclusivity pattern occurred when the  \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} and \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants differed significantly from each other in their ratings, in \textit{both} the \vioProduct{} and the \appProduct{}.

Participants in Guideline 4's experiment (``show contextually relevant information'') exhibited this pattern in six dependent variables (Figure~\ref{fig:third-category-guideline-4}).
%The six instances of dependent variables with this last category of insight are highlighted in the top and bottom halves of Table~\ref{tab:G4-Stats} (p-value column).
In fact, in this experiment the risk-averse participants always gave significantly lower ratings than the risk-tolerant participants in both the \vioProduct{} (Table~\ref{tab:G4-Stats}, top, p-value column) {and} the \appProduct{} (bottom).
Even with Bonferroni corrected p-values (sixth column), the risk-averse participants felt significantly less certain with the \vioProduct{} (t(62) = 3.6258, $p = .005$, d = .910) and with the \appProduct{} (t(63) = 4.7513, $p < .001$, d = 1.186) than the risk-tolerant participants did.
The same pattern also manifested in their responses to the ``I would be suspicious'' dependent variable.

%\boldify{Li et al. also found that G4 had its problems, and participants on both sides of the attitudes toward risk spectrum held similar concerns.}


\FIXME{Unhoused Implications from 4.1 starts here}


\emph{Implications for Researchers and Practitioners:}
The results of disaggregating in this particular case have three implications.

First, disaggregating by problem solving style value can help researchers and designers answer questions about mysterious peaks and valleys in HAI user experience data.
For example, the results suggests that violating Guideline~11 (i.e., \textit{not} explaining why the AI Product did what it did) may result in users who are more risk-averse in using technology viewing such products much less favorably than users who are risk-tolerant.

% \FIXME{AAA@MMB: Really didn't like the ``data from users who are risk-averse...'' verbiage. I tried applying Zinsser to this and hope I didn't break anything.}

Second, disaggregating data by participants' attitude toward risk helped to explain these data, pointing the way toward potential design remedies that HAI designers can consider to help improve more users' experiences with the product, or at least clarify what additional data needs to be collected from user studies.
In the Guideline~11 vignette, the \appProduct{} offered an explanation \textit{button}, but participants did not see the actual explanation. 
Here, risk-tolerant individuals felt in control just from knowing an explanation would be available, but risk-averse individuals may have needed to see what the explanation would actually explain before they could feel in control.

Finally, an implication from these results for designers of AI products is that failing to follow Guideline~11 by providing an explanations of the AI's outputs may lead risk-averse users to abandon the AI-powered feature because they may not feel in control.

\FIXME{Unhoused implications from 4.1 ends here}
%Begin FIXED
\FIXED{
\emph{Implications for Researchers and Practitioners:}
These six instances of Pattern~\#3 suggest that sometimes applying such guidelines is not enough to meet the needs of risk-averse participants.
In this experiment, one possible reason for the risk-averse participants' lower ratings might have arisen over concerns about privacy with the \appProduct{}:




For designers, one possible way to address such privacy concerns may be using AI explanations to increase transparency into how the system makes its decisions.
For example, Lim \& Dey's ``inputs'' and ``outputs'' intelligibility types~\cite{lim2019these} provide one possible direction.
Mueller et al.~\cite{mueller2019explanation} provide a compilation of works from the eXplainable AI (XAI) literature with other possible directions.

\input{figure/07-All-Boxes/Risk/03-G4}
\input{tables/Risk/2-G4-PostStrat}

\boldify{Dear reader, we had enough evidence to demonstrate that \newline H1-CognitiveDiversity-RiskStyle held; it was in fact the case that the risk-averse users' user experiences were more frequently disparately impacted across the 16 experiments than their risk-tolerant peers.}

Overall, Sections~\ref{subsec:why-disaggregate} and~\ref{subsec:3-categories} have shown the data repeatedly supported \textbf{H1-CognitiveDiversity-RiskStyle}.
10 of the dependent variables in the Guideline~4 experiment exhibited instances of all three patterns; Table~\ref{tab:G4-Stats} shows all the results from that experiment.
Complete results from the remaining experiments are given in Appendix~\href{https://web.engr.oregonstate.edu/~anderan2/MSR-Appendices/Appendix-Boxplots.pdf}{{\color{blue}D}}.
Across all experiments, the data revealed a total of 33 disparities between risk-averse and risk-tolerant human-AI interaction participants. 

Of these 33 instances, in 30 of them (90.9\%) the risk-averse participants rated the AI products significantly lower than the risk-tolerant participants did.
This suggests that when designers apply the guidelines for human-AI interaction, additional considerations beyond the guidelines may be needed to reduce inclusivity gaps among users who have diverse attitudes toward risk in using technology.

%End FIXED
}

\FIXME{MMB to AAA: see ** above}

\subsection{User Experience \textit{Inclusiveness}: What diverse attitudes toward risk reveal
\draftStatus{MMB thinks...?}} 
\label{subsec:inclusiveness-risk}

\boldify{but disagg'ing shows more: Abi's improved and so did Tim's.  Yay: inclusivity.}


Disaggregating these participants' data by their attitudes toward risk also revealed information about the inclusiveness between the \vioProduct{} and \appProduct{}.
\begin{tcolorbox}
    \underline{\textbf{Definition---User Experience Inclusiveness:}}\\
    Between two treatments, there is a change in the inclusiveness of users' experiences if, for users of either problem solving style, a statistically significant differences exists between the two treatments. 
\end{tcolorbox}
For example, consider the bottom trio of boxes in Figure~\ref{fig:risk-app-disagg} that shows the distribution of participants' responses to feeling in the control for the \appProduct{}.
Notice that the participants' averages improved (i.e., the x's moving to the right) for both the risk-averse and risk-tolerant participants, and a paired t-test suggests that both the\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} (paired t-test, t(30) = 4.5412, p $<$ .0001) and the \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} (paired t-test, t(31) = 4.0000, p = .0004) felt significantly more in control with the \appProduct{} than they had with the \vioProduct{}.
%Begin FIXED
\FIXED{
This suggests by definition that in this experiment, applying Guideline 11 was not only beneficial for users on average, it was also \textit{inclusively} beneficial for users with diverse attitudes toward risk.
%End FIXED
}

\subsection{Discussion: User Experience Equity, Inclusiveness, and their interaction
\draftStatus{MMB thinks...?}}
\label{Discussion:Equity-Inclusion}

\FIXME{HERE would be a great spot to discuss the "how much more/less equitable" discussion.
You have to mention that you're drawing inspiration from the odds ratio, which tells you how much more/less likely an event is to occur.
There's nothing in the literature}

%\subsection{Actionable possibilities for designers of Human-AI systems: 5 explicit risks\\}
\subsection{Inclusivity gaps on the spectrum of risk attitudes: What might designers \textit{do}?
\draftStatus{AAA says 2.5}}
% \subsubsection{Actionable possibilities for designers of Human-AI Systems **d1}
\label{subsubsec:Risk-forDesigners}

\boldify{wow, this is actionable. In general, a designer has to address the risk - either the perception of risk  or the actual risk.}
%

When participants picked which system they preferred, their free-form comments about why they preferred it sometimes reflected their attitudes toward risk.
The four types of risks participants raised may suggest possible avenues for designers to address insights like those in Section~\ref{subsec:3-categories}.

%After seeing both AI systems, participants were asked to pick which system they preferred and why, and their attitudes toward risk were sometimes reflected in their text responses.
%Understanding the insights they raised might help designers of human-AI powered systems anticipate users' potential reactions to various designs.
%, so they might generate designs to address such concerns.
%We highlight 5 types of risks participants raised across multiple experiments.


% Participants' attitudes toward risk sometimes arose when they explained why they preferred one of the systems (whether the Application or Violation).
%
%In experiments where a large majority of participants preferred the guideline Application, some participants across the spectrum of risk attitudes brought up risk-related subjects.
%that not only helped to justify their preference but also manifested in how the Application changed their responses to certain dependent variables.

\boldify{1. Intrusiveness (aka, privacy of input data) - This really ties to ``targeted oucomes''. They're trying to make the system ``better'', but it's going over like a lead balloon.}

%
% Looking at their responses, some participants expressed concerns over the intrusiveness of the Application system (Table~\ref{table:G4-Vignette}):
%

\textbf{AI Risk 1--How the AI gathers inputs:}
Participants sometimes raised concerns about if the products gathered information about them without their consent.
Some preferred the \vioProduct{} and stated that they thought the \appProduct{} might be tracking them%
\footnote{Note in Appendix~\ref{appendix:vignettes} that none of the vignettes mentioned if/how the systems gathered information about the participants}.
For example, \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G3-1959-risk-averse} stated that

\quotateInset{[Application AI product] is tracking me somehow because it holds the notifications, so I prefer the less invasive [Violation AI product].}
{}
{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G3-1959-risk-averse}}
{Whole quote - [Application AI product] is tracking me somehow because it holds the notifications, so I prefer the less invasive [Violation AI product].}
%

In another experiment, participants who preferred the \vioProduct{} raised similar concerns:
\quotateInset{I would prefer to use [Violation AI product] because [Application AI product] feels a bit more intrusive. I would be nervous that [Application AI product] is pulling data from things like my other software and my browsing history.}
{}
{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G4-3905-risk-averse}}
{Whole quote - I would prefer to use Ione because Kelso feels a bit more intrusive. I would be nervous that it is pulling data from things like my other software and my browsing history. This would be unacceptable since I work with sensitive PII.}

%Participant: There are ears everywhere. I don't like this.
\quotateInset{%I don't like the idea of [Application AI product] taking definitions from my workplace. 
[Application AI product] makes me worry I'm being listened to or that my network is being monitored, etc.
}
{}
{\colorboxBackgroundForegroundText{TimBlueQuote}{black}{G4-3947-risk-tolerant}}
{I don't like the idea of Ione taking definitions from my workplace. It makes me worry I'm being listened to, or that my network is being monitored, etc.}

For designers, statements like these suggest the need to empower users to know how the system gathers its inputs and decides how to show its outputs.
One potential avenue may be using AI explanations to increase transparency into how the system makes its decisions.
For example, Lim \& Dey's ``inputs'' and ``outputs'' intelligibility types~\cite{lim2019these} provide one possible direction.
Mueller et al.~\cite{mueller2019explanation} provide a compilation of works from the eXplainable AI (XAI) literature with other possible directions.

\boldify{... 2. the risk that they'll waste a whole bunch of time...}

\textbf{AI Risk 2--Human's wasted time:}
Participants also stated their preference for the \appProduct{} because of the risk of them pointlessly wasting time:
\quotateInset{I like that [the Application AI product's feature] is easy to locate ... nothing more frustrating than trying to find something and not being able to...}
{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G7-2138-risk-averse}}{}{I like the idea of getting suggestions or being able to access suggestions when none pop up.  I like that it is easy to locate because there is nothing more frustrating than trying to find something and not being able to find it.}

\quotateInset{[Violation AI product] would be a call to the help desk and a big time suck...}{}{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G11-2921-risk-averse}}{I believe I could pinpoint any insights with lone. Kelso would be a call to the help desk and a big time suck if there was inaccurate data.}

Since participants had only just been introduced to the proposed products, the products were new to the participants.
As such, these comments are reminiscent of Blackwell's theory of Attention Investment~\cite{blackwell2002first}, which proposes that in deciding whether to use a new system or feature set, users often perform a cost/benefit/risk calculation.
Specifically, in this theory, users weigh their expectation of the time cost of learning/using the new feature set against their expectation of benefit (time saved, in Blackwell's theory) they will receive---tempered by their expectation of risk (probability) that spending that time will not result in the benefits after all. 
Risk-averse users are hesitant to spend extra time learning unfamiliar technologies~\cite{charness2012strong}.
One possibility to address \textit{this} aspect of risk that designers may consider is how to empower such users in correctly guess-timating cost/benefit trade offs.
In this instance, they may have to design for the trade offs between the costs of potential errors in the AI system and the benefits of accepting the AI's decisions as opposed to doing all of the work themselves, along the lines of the surprise-explain-reward strategy~\cite{wilson2003harnessing}.
%(benefit) and how much time they might have to spend fixing errors the AI makes (cost).

%so designers might consider how to support such users in guess-timating

%in guess-timating how much time they might spend in such interactions.


%When people get us to answer survey, they say how long the survey is (minutes, number of clicks)

% For example, one possible avenue to facilitate participants like G7-2138's interaction might be to apply the Gestalt principle of proximity~\cite{palmer1999vision} to support ease of finding how to invoke the AI-powered feature.
%That theory describes how users weigh their \textit{expectation} of the risk of trying out a new software feature and failing at it, vs. how much they value the benefit they \textit{expect} to gain if they succeed, vs. the cost \textit{expect} to spend learning and using the feature.


\boldify{...3. risks of harms to people actively recognized in the Violations (fairness). There are entire conferences devoted to solving it. We refer designers to these conferences to adopt some proposed changes there....}

\textbf{AI Risk 3--Unfairness in AI:}
Participants also raised concerns about the risk of the AI being harmful to others.
% This risk specifically arose in the  which deals with how AI-powered systems can harm other people.
For example, Bird et al.'s ``harm of denigration'' occurs when one group of people are being stereotyped in a derogatory way~\cite{bird2020fairlearn}.
Some participants remarked on this point:
%Participants across the risk spectrum called out this risk in Guideline 6's experiment:

\quotateInset{[Violation AI product] obviously doesn't think that women and people of color can hold highly-regarded, high-paying, and/or highly-educated positions. The search results I've landed upon on [Application AI product] are more inclusive and represent the values that are important to me...}{}{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G6-1162-risk-averse}}{[Violation AI product] obviously doesn't think that women and people of color can hold highly-regarded, high-paying, and/or highly-educated positions. The search results I've landed upon on [Application AI product] are more inclusive and represent the values that are important to me...the values that are held by (I believe) the majority of people share when it comes to equality and respect. [Violation AI product] sounds like it was created by a group of individuals who believe in white supremcy [sic] and don't think women are capable of being in these positions. [Violation AI product] encourages negative stereotypes, that women and minorities aren't capable or intelligent enough to be holding these positions and that goes against everything I believe.}

\quotateInset{[Application AI product] is not trying to be harmful by indicating that women and people of color are not as smart or successful. [Violation AI product] sounds like something a white nationalist group would come up with to indicate their superiority over everyone, including women.}{}{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G6-1410-risk-averse}}{[Application AI product] is not trying to be harmful by indicating that women and people of color are not as smart or successful. [Violation AI product] sounds like something a white nationalist group would come up with to indicate their superiority over everyone, including women..}


Although there are emerging efforts to start highlighting and solving fairness-related concerns from an algorithmic perspective (e.g.,\cite{acm_facct,bias_2022,fairlearn}), remedies to solve such insights for designers of human-AI interfaces remain an open problem.

%remedies for designers of human-AI interfaces might solve fairness-related concerns are relatively scarce.
% Research investigating fairness insights in AI (e.g.,~\cite{acm_facct,bias_2022}) and tools like the FairLearn package~\cite{fairlearn} might assist designers in finding and addressing algorithmic fairness-related concerns.




%\FIXME{6. Control}

% \FIXME{G1 - 224 - Risk-tolerant: I have <like to have> input on what [Application AI product] does. [Violation AI product] makes me very nervous.}

\boldify{... and lastly 4. control.}
%There are two sides to the control coin that we need to discuss. The first deals with how people want to retain control.

\textbf{AI Risk 4--Human control in the AI-powered system:}
Lastly, some risk-averse participants mentioned preferring certain products because they could exert more control over it:

\quotateInset{[Application AI product] would give me a limited amount of acronyms... [Violation AI product] seems like it would give me more control.}
{}{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G4-3897-risk-averse}}{
Probably because I would want more control over what acronyms I have to select from.
Ione would give me a limited amount of acronyms for the workplace and document, but Kelso would allow me to work with all documents even outside of the workplace.  
I hate autocorrect sometimes because it corrects words that need to correcting and assumes things, Kelso seems like it would give me more control.
}
%and a participant in guideline 3 also commented on this:

\quotateInset{I prefer manual control rather than having an app decide when something should or should not happen automatically.}{}{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G3-953-risk-averse}}{I prefer manual control rather than having an app decide when something should or should not happen automatically. For example, I would rather turn off all notifications or volume than an application deciding for me when to do so. Ideally, an application would provide the option of whether to exhibit such behavior or not.}
%A few participants also expressed sentiments about the system making decisions for them:
\quotateInset{I would rather have to pick the word I want if the program is not sure. I don't want the program to insert a word I don't want or that does not really fit the context.}
{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G10-1833-risk-averse}}{}
{I would rather have to pick the word I want if the program is not sure. I don't want the program to insert a word I don't want or that does not really fit the context. Stopping and checking as I went would be easier if the project is one that is very long and would require a lot of proofreading to find the automatic insertions that might be off.}
% G10 - preferred application
%\quotateInset{I would feel more in control of the writing process if there was a list and I could choose what I wanted rather than having a machine force a word into a sentence for me.}
%{\colorboxBackgroundForegroundText{TimBlueQuote}{black}{G10-1906-risk-tolerant}}{}
%{I would feel more in control of the writing process if there was a list and I could choose what I wanted rather than having a machine force a word into a sentence for me.}


% \FIXME{Over-reliance = the other side of the control coin}

Others mentioned how they might bear the responsibility of the AI's mistakes if they ended up relying too much on the \appProduct{}: 
%Another participant mentioned that they preferred the Violation AI product because they might possibly overly-rely on the Application AI product:

\quotateInset{With [Application AI product], if I relied on it too much and it make a mistake, of course I would be the one held responsible...
I would feel safer relying on my own expertise and using [Violation AI product].}
{}{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G4-3936-risk-averse}}{
With Ione, I can rely on my own expertise to choose the correct acronym definition.
So if there is a mistake, it would be me making the mistake, not Ione. 
I feel I have more control/responsibility with Ione.
With Kelso, if I relied on it too much and it make a mistake, of course I would be the one held responsible, not the document program.
I would feel safer relying on my own expertise and using Ione.
}

These results align with other researchers' findings, such as users' unwillingness to give up control without the ability to regain it, who may be hesitant about relying on an unproven technology~\cite{howard2014public,haboucha2017user}, fearing over-reliance of a system's outputs~\cite{kaur2020interpreting}, or fearing that a lack of control may lead users to boredom and inattention~\cite{cunningham2015autonomous}.
Designers may consider how to alert the users when they should regain control of the car, such as Schneider et al.~\cite{Schneider_AV_modalities}, who tested audio, visual, and haptic feedback modalities in the context of autonomous vehicles.
Russell~\cite{russell2019human} discusses the insight of how to control artificial intelligence in more depth.

\FIXME{Deliver on concrete suggestions for designers about what they might \textit{do} to ``solve'' the control problem in their interfaces.}

For designers, these suggest possible considerations when designing AI-powered products for users with diverse attitudes toward risk in such ways that may help them become more reliable, safe, and trustworthy~\cite{shneiderman2021tutorial}.


\FIXME{AAA - Need glue to tie together what they've read with what they're going to read. A sentence similar to what you did for 4.2.}

\subsection{Beyond Risk: H2-CognitiveDiversity-5Styles
\draftStatus{2.6}
}
\label{sec:other-styles}

\input{tables/4-Triangulation-table}

\boldify{Table~\ref{tab:triangulation-table} shows 4 things: (1) Abi's are usually impacted (98/114 insights) but not always (look at information processing), (2) the facets are triangulated (rows), and (3) the guidelines are triangulated (columns).}


Going beyond attitudes toward risk, \textbf{H2-CognitiveDiversity-5Styles} posited that disaggregating HAI participants' data by \textit{any} of their five problem solving style types will reveal the same abstract patterns as those that emerged for the risk style.
Our analyses across experiments supported this hypothesis for every problem solving style.  
To spare the reader pages and pages of statistical tables here, we simply summarize the evidence in 
Table~\ref{tab:triangulation-table}.

Table~\ref{tab:triangulation-table}'s summary shows that evidence of all three abstract patterns...

\begin{enumerate}
    \item ...triangulated across all five problem solving style types for every abstract pattern except one, namely Information Processing's Pattern~\#3 (rows).
    \item ...triangulated across multiple experiments: when pattern instances arose in any experiment, they tended to arise across multiple problem solving style types with at least two instances of each pattern (columns).
    \item ...arose for participants with both \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{``Abi''-like}%
    %
    \footnote{For each problem solving style type, participants were \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{``Abi''-like} if their value for that style was the \textit{left} column of Table~\ref{table:personas} (i.e., risk-averse, task-oriented motivations, process-oriented learning style, comprehensive information processing style, or lower computer self-efficacy)}
    %
     and \colorboxBackgroundForegroundText{TimBlueQuote}{black}{``Tim''-like}%
    %
    \footnote{For each problem solving style type, participants were \colorboxBackgroundForegroundText{TimBlueQuote}{black}{``Tim''-like} if their value for that style was the \textit{ right} column of Table~\ref{table:personas} (i.e., risk-tolerant, tech-oriented motivations, tinkering-oriented learning style, selective information processing style, or higher computer self-efficacy)}
    %
    values across all five problem solving style types
\end{enumerate}


\boldify{For item (1), consider all of the 48 colored cells. The majority of the colored cells were \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{``Abi''-like}, providing additional information about such participants in 95 of the 112 dependent variables.}

For item (3), the disparities between participants with \colorboxBackgroundForegroundText{white}{black}{``Abi''-like}  and ``Tim''-like problem solving style values most often showed that the ``Abi''-like participants had the significantly lower average responses to the UX metrics in 95 of the 112 (84.8\%) pattern instances. 
Of the 17 pattern instances uncovered about the participants with ``Tim''-like problem solving style values, 10 were for those with selective information processing styles.

\textit{Implications for Researchers and Practitioners:} 
The mix of results for participants with ``Abi''-like and ``Tim''-like problem solving style values, along with the concentration of insights about the selective information processors, suggests that the focus of researchers and practitioners designing AI products should not exclusively be on those with certain problem solving style values instead of others (e.g., exclusively the\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} or the \colorboxBackgroundForegroundText{TimBlueQuote}{black}{selective information processors}).
Instead, researchers and practitioners of AI-powered systems should consider the needs of HAI users who have diverse problem solving style values to support their user experiences both inclusively and equitably.


\subsection{Leftovers from "no inclusivity improvements for anyone"}

%-------MMB says: do not use this, it introduces another dependent vble that we never set up and are not consistent about measuring. If we ever reinstate it, we'll have to give that vble full status -- set it up at the beginning, measure it consistently, report it in all our tables, etc., etc.
%
%\boldify{Despite this seemingly tepid response in the user experience outcomes, we were surprised to see that participants still overwhelmingly preferred the application over the violation, which seemed ``not too bad'' for designers.}
%
%At face value, this category of results may suggest that considering attitudes toward risk may \textit{not} help our understanding.
%However, we were surprised to see that despite these statistically imperceptible changes in HAI-UX inclusivity, a strong majority of both the risk-averse and risk-tolerant participants preferred the \appProduct{} over the \vioProduct{}.
%When participants had to choose one of the two AI products products, 23/26 (88.46\%) of risk-averse participants stated that they would prefer to use the \appProduct{}.
%Similarly, 28/31 (90.32\%) of the risk-tolerant participants stated that they would prefer the \appProduct{}.
%-------end of do not use

% \FIXME{AAA - I feel like something might be missing here, but I'm not sure. I had the idea to put a boldify and paragraph about ``participants liked the appProduct for many a reason'', but I'm not sure that it really contributes much to the narrative that the odds don't already. Turns out that it did}

%%\boldify{Why: Risk-averse participants reasons were...}
%For example, 19/26 risk-averse participants mentioned something about the application description's detailed nature or that they just didn't know how the violation worked.

%------------MMB: DO NOT USE THIS.
% Why: the theme is: nobody liked these (in the DVs we're covering).  So then going to quotes saying why people liked it makes no sense.
%
%When participants did rate one product above the other, their reasoning often clustered by attitude toward risk.
%For example, 19 of the **howmanyTOTAL**FIXME** risk-averse participants  appreciated the increased level of detail, such as:
%\quotateInset{I strongly prefer [\appProduct{}] based on the more detailed input it gives you...}
%{}
%{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G1-235-risk-averse}}
%{Whole quote - I strongly prefer Ione based on the more detailed input it gives you and the advice it can give you is very important for presentations.}
%G1-235 then went on to implicitly tie their appreciation to risk---i.e., minimizing the risk of an inadeqaute presentation:
%\quotateInset{...the advice it can give you is very important for presentations.}
%{}
%{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G1-235-risk-averse}}
%{Whole quote - I strongly prefer Ione based on the more detailed input it gives you and the advice it can give you is very important for presentations.}
%Participant G1-187 expressed the same reasoning:
%\quotateInset{The Presenter Coach with [\appProduct{}] is more specific and offers more of a direct line on how it will help improve my presentation. In contrast, [\vioProduct] seems to be more vague and unspecific in terms of how it would assist me with my presentation styling.}
%{}
%{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G1-187-risk-averse}}
%{Whole quote - The Presenter Coach with lone is more specific and offers more of a direct line on how it will help improve my presentation. In contrast, Kelso seems to be more vague and unspecific in terms of how it would assist me with my presentation styling.}
%
%In contrast, not a single one of the \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants mentioned the level of detail.
%Instead, they largely focused on utility.
%For example, 21 risk-tolerant participants expected the \appProduct{} to provide more detailed feedback, which would help them:\quotateInset{[\appProduct{}] would be the better option for me because I am highly motivated to improve each and every presentation that I give.}
%{}
%{\colorboxBackgroundForegroundText{TimBlueQuote}{black}{G1-240-risk-averse}}
%{Whole quote - Kelso would be the better option for me because I am highly motivated to improve each and every presentation that I give..}
%or how such features would change their usage over time:
%\quotateInset{I think I can see and understand how [\appProduct{}] works better and so I feel more comfortable in using it and knowing it is will impact my usage and aid me over time...}
%{}
%{black}{G1-870-risk-averse}}
%{Whole quote - I think I can see and understand how Ione works better and so I feel more comfortable in using it and knowing it is will impact my usage and aid me over time, it feels like a predictive sort of platform whereas Kelso I don't quite understand.}
%---------end of do-not-use-this

%**MMB to start here**
%These results demonstrate for HAI practitioners that the value of considering participants' attitudes toward risk is not only useful when considering HAI-UX inclusivity but also that considering attitudes toward risk helps to uncover trends in participants' reasoning.
%In this case, considering participants' attitudes toward risk for their HAI-UX inclusivity change revealed no viable results, but considering this problem-solving style \textit{did} help to uncover that when participants preferred the \appProduct{}, they preferred it for different reasons.

% \FIXME{AAA@MMB: Yeah, I'm much happier with this component here}

%\boldify{However, there was one exception to this, namely Guideline. In this case, the tepid response to the applications did not mean they preferred it. In fact, nearly half of the risk-averse participants preferred the \textit{violation}.}

%Investigating participants' attitudes toward risk uncovered that of the 10 experiments exhibiting this category of HAI-UX inclusivity, more than 70\% of the risk-averse and risk-tolerant participants preferred the \appProduct{} in 9 of them.
%The one exception to this was for Guideline 4\footnote{Guideline text: \textit{Show contextually relevant information}}, where only 51.72\% of risk-averse participants and 69.4\% of risk-tolerant participants preferred the \appProduct{}.
%In this experiment, the products were document editing applications, and the AI-powered feature explained the meanings of acronyms, such as ``CDC'' standing for ``Centers for Disease Control''.
%The \vioProduct{} derived its explanations from a standard list of possible definitions, whereas the \appProduct{} showed definitions that were used in the participants' workplace and pertained to the topic of the document being worked on. 
%Table~\ref{tab:no-inclusivity-change} shows that similarly to before, this design change did not yield a statistically perceivable change for either the risk-averse or the risk-tolerant participants.
%In fact, the risk-averse participants' average feeling of being secure insignificantly \textit{decreased} for the \appProduct{} \tTestResult{26}{-0.9874}{.333}{**FIXME**}, whereas the risk-tolerant participants' average response hardly changed \tTestResult{35}{0.3468}{.731}{**FIXME**}.


% \boldify{Tables~\ref{**FIXME**} \&~\ref{**FIXME**} show how frequently these categories turned up across all five problem-solving styles. In the interest of space, I'm just pointing out a couple of nuances, but we'll provide everything in the appendices }

% Tables~\ref{**FIXME**} and~\ref{**FIXME**} summarize the answer to \textbf{RQ**FIXME**}, which was a resounding ``yes''---the HAI-UX inclusivity and equity categories \textit{did} generalize to all five of the problem-solving styles.
% These tables, in the interest of space, only highlight how frequently these significant phenomena arose, along with potential differences in who derived benefits from the way that certain guidelines were applied.
% For example, Table~\ref{**FIXME**} shows that although only the ``Abi''-like risk-averse participants received significant inclusivity benefit from the \appProduct{}s about half as often as the ``Tim''-like risk-tolerant (13 times as opposed to 28), the \appProduct{}s were especially useful for the participants with ``Abi''-like task-oriented motivations, who received the signiciant inclusivity benefit more often than those with ``Tim''-like tech-oriented motivations.
% A complete list of every dependent variable and every statistical test performed on these data exists in Appendix**FIXME**.

% \input{tables/06-Everyone-Else}

\boldify{Hark, reader, at G18! What once was Tim is also Abi, just a different problem-solving style (learning style).}

This phenomenon at the level of experimental guideline was not isolated to motivations.
For example, Table~\ref{tab:Risk-Inclusivity-Frequency} showed that that in Guideline 18's experiment, the ``Tim''-like risk-tolerant participants derived significant HAI-UX inclusivity gains from the \appProduct{} in five of the dependent variables.
However, the top of Table~\ref{tab:Learn-Info-Inclusivity-Frequency} suggests that as well as the risk-averse participants, the ``Abi''-like process-oriented learners also derived a significant HAI-UX inclusivity gain from Guideline 18's \appProduct{}.
This highlights that different problem-solving styles receive different benefits from applications of these guidelines.


\boldify{And these participants' learning styles showed up in their reasoning for which of the two products they preferred.}

Considering all five problem-solving styles can also uncover more relevant ways to understand qualitative data.
For example, when Guideline 18's participants commented on which of the two products they preferred, their learning styles revealed additional information, whereas their comments did not reflect anything about attitude towards risk.
One such concept reflective of learning style was a desire to learn about how the AI product reasoned.
28\% (9/32) of process-oriented participants commented on preferring the \appProduct{} because it would help them learn how the product reasoned:

\FIXME{USE THE TERM ``LEARN'' about how THIS AI works, not how AI works, cite the empirical journey paper with Peggy, Minsuk, and Jon.}
% As process-oriented learners (Abis) learn about the new tech updates, they want to learn how to react and what steps to take depending on the changes.
% It becomes a step-by-step process where first, Abi wants to learn about the changes and how the AI determined its actions and updates. 
% Then, Abi evaluates if the update is a good change for their purposes to lastly, decide on keeping the changes, adjusting them or overriding them. 
% This is portrayed in the quotes below.

\quotateInset{I would want to know what [\appProduct{}] is thinking and how they are behaving so I can adjust it if needed. }
{}
{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G18-3037-process-oriented}}
{Whole quote - I would want to know what Kelso is thinking and how they are behaving so I can adjust it if needed. }
Comments like these are reminiscent of Dodge et al.'s concluding remarks~\cite{dodge2021no}, where these process-oriented participants seemed to be setting their own learning goals to learn about how \textit{this} AI-powered feature made its decisions.

% G18-1460-process-oriented: "I would like to be made aware of changes made so that I can still work with the system or overide it if required."
% G18-3037-process-oriented: "I would want to know what Kelso is thinking and how they are behaving so I can adjust it if needed."

On the other end of the learning style spectrum, the tinkering oriented learners' comments exhibited a different pattern.
Only 6\% (2/35) of these tinkering-oriented learners commented on the desire to learn \textit{how} the AI reasoned, whereas 71\% (25/35) of them indicated wanting to be informed only of the changes that took place but \textit{not} about the AI's internal workings to arrive at these updates.

\quotateInset{I like the fact that [\appProduct{}] informs me of changes that I may not notice right away. }
{}
{\colorboxBackgroundForegroundText{TimBlueQuote}{black}{G18-1708-tinkering-oriented}}
{Whole quote - I like the fact that Kelso informs me of changes that I may not notice right away.}

\quotateInset{I would like to be alerted to the change.}
{}
{\colorboxBackgroundForegroundText{TimBlueQuote}{black}{G18-2078-tinkering-oriented}}
{Whole quote - I would like to be alerted to the change.}

\quotateInset{I like to know when a change is made. It gives me a sense of control.}
{}
{\colorboxBackgroundForegroundText{TimBlueQuote}{black}{G18-2118-tinkering-oriented}}
{Whole quote - I like to know when a change is made. It gives me a sense of control.}

\FIXME{AAA@Jimena: Is there a better quote than 1679? Their saying ``how it sorted...'' gives the impression that this was one of the 6 who commented on the how.}

\boldify{One of the things that's important to note here is that whereas for risk, the focus was on providing a sense of control (per Result \#3), providing interpretable explanations for how AI like this reasoned will help process-oriented learners}



\Result{8}{\textit{Exposing how this AI worked significantly improved the HAI-UX inclusivity for process-oriented learners.}
In Guideline 18, the \appProduct{} provided more information about how the AI made its decisions, which process-oriented learners desired to learn.
This helped explain why there were so many HAI-UX inclusivity benefits for the process-oriented learners.}

%\subsection{Motivations}




\subsection{Leftovers from Section 6.1}

%-----------MMB: cutting this for now
\FIXME{MMB: cutting all of this, not because there's anything wrong with it, but because I don't think it's adding anything interesting, and our readers are tired!

For attitudes toward risk, our participants' gender-age differences are consistent with those of other researchers who have found an inverse relationship between people's age and their willingness to take risks.
%that people are less willing to take risks as they grow older.
Our results for the men resemble, for example, Dohmen et al.'s~\cite{dohmen2017risk} findings, in which their participants' risk-aversion increased linearly until around 65 years old.
%Our results also add to Dohmen et al.'s results: our analysis showed that, in contrast to the men, the women became \textit{decreasingly} risk-averse.
These differences in attitudes toward risk by gender and by age may help explain other researchers' reports (e.g.,~\cite{hulse2018perceptions,gish2017driving,van2019exploring}) of demographic differences between people's experiences with AI products.
%
%For designers, such results suggest that by supporting individuals who are risk-averse, technologies may become more gender inclusive, especially for younger individuals.
%
%
%
\boldify{Let's talk about self-efficacy with age}

% \textbf{\textit{Computer self-efficacy: }}
For computer self-efficacy , other researchers have found a relationship between people's gender and/or age and their computer self-efficacy~\cite{lopez2017teacher,schreder2013age, flandorfer2012population, chang2014specialization, liberatore2022gender, dutta2018modeling, gunbatar2018gender}.
%Lopez et al.~\cite{lopez2017teacher} found a strong negative correlation between their participants' computer self-efficacy and age, a result that Schreder et al.~\cite{schreder2013age} had also found.
For example, Vsabic et al.~\cite{vsabic2021teachers} found an interaction between computer self-efficacy, gender, and age.
Specifically, their study reported gender differences in self-efficacy for using Information Communication Technology that were prevalent among older teachers and practically non-existent among younger teachers.
%
Our participants' trends seem to mirror Vsabic et al.'s finding;
there was hardly any difference in the proportion of lower self-efficacy women and men in the 18---24 years old group.
However, the gap in the proportions between these two genders increased across the age groups, where the women had a greater percentage of lower self-efficacy participants than the men.
Thus, gender and age differences in computer self-efficacy may provide an additional possible explanatory factor to help explain demographic differences in people's experiences with some AI products.


%Similar to risk-averse people, supporting those with lower computer self-efficacy might make technologies more gender inclusive, except for \textit{older} individuals.
%This suggests that supporting individuals with lower computer self-efficacy might make technologies both {age} inclusive \textit{and} gender inclusive.




%\textbf{\textit{Information processing style:}}
For information processing style (no figure shown), others' research has shown both gender differences~\cite{meyers2015infoProcessing,showkat2018identifying} and age differences~\cite{geerligs2018age,guest2015aging,mcintosh2021evaluating,torrens2020lacking}.
% One example of such works, Gell et al.~\cite{gell2015patterns}, found age-related barriers in older people interacting with information-rich technology like email, such as vision and memory impairments as they grow older~\cite{gell2015patterns}.
In contrast to these findings, our sample of participants showed no evidence of a difference in participants' information processing style across gender or age.
% Thus, it is an open question as to how information processing style might help explain gender and age differences in human-AI interaction.


For styles of learning new technologies (Figure~\ref{fig:learn-by-age}), both Papavlasopoulou et al.~\cite{papavlasopoulou2020coding} and Ichinco et al.~\cite{ichinco2017NoviceProgrammers} found gender difference suggesting that male%
\footnote{Male \& female used for faithfulness to their terminology.} %
children relied more on tinkering, whereas female children followed a more process-oriented style.
In samples of older participants, researchers have also discovered this same trend~\cite{showkat2018identifying,meyers2015infoProcessing}.
Our participants echo such findings, where women had more process-oriented learners in each age group---the greater the age, the greater the percentage of process-oriented learners for both of these genders.
%and the proportions in both groups increased steadily across age groups.
These results suggest that styles of learning new technologies may be a possible third explanation for gender and/or age differences.


%\textbf{\textit{Motivations: }}
For motivations for using technologies (Figure~\ref{fig:mot-by-age}), researchers have found both gender~\cite{hallstrom2015gender,noguti2019gender} and age differences~\cite{van2019exploring,gish2017driving} about their participants' motivations to interact with technologies.
Consistent with these findings, our data showed differences across both gender and age, which provides a fourth possible avenue by which gender and/or age differences in user experiences with AI products may be explained.
}


%-----------------cutting this for now From Section 7----------
\FIXME{MMB: cutting this subsec -- it's perfectly fine, but not really adding that much
%---------------------------------
\subsection{Even equality is difficult for some AI products \draftStatus{MMB: d2.25}}
\label{subsec:equality discussion}


In addition to inclusivity and equity, a third concept in considering HAI fairness is that of equality.
Equality differs from both inclusivity and equity.
Unlike inclusivity or equity, equality can be thought of as an ``input-related'' concept, i.e., providing exactly the same materials, same system, etc., to everyone. 

For non-AI software products, equality is almost a given property---if the product is the same and does not behave differently depending on the user or the hardware/software environment, then equality is present.
However, consider the many AI products that adapt dynamically to their own users.
If the product trains on user A's data on their computer, then it will behave differently than the product on user B's computer, making it no longer possible to  assume equality.

Equality can help with equity, but it does not automatically provide it. 
An example of equality would be providing the same AI product trained on exactly the same data to everyone.
Although this is an example of equality (of inputs), it would not be equitable if, for example, the AI product required sophisticated AI knowledge that only some of its users possessed.


This property some AI products have of dynamically varying their behavior according to their \textit{particular} user's experiences and contexts adds a unique and difficult challenge, which in turn adds complexity to the goal of ultimately providing equitable and high-quality user experiences to users of AI products.  
} %end of subsection we cut (for now)

==> doc/z-Leftovers.tex <==
%-------------
\section{Leftovers from Intro}


%
%\boldify{Since we're dealing with diversity, we are doing the responsible thing with a Researcher Self-Disclosure.}

%\textit{Researcher Self-Disclosure:} Our multidisciplinary team of researchers, some of whom are members of the LGBTQIA* community or the PoC community, recognize that as academic researchers, we are in positions of privilege.
%We are committed to using that privilege to improve technology's inclusivity and equity for users who are disproportionately disadvantaged by today's user experience.
%
%\FIXME{MV-7: If we include this, it should be more meaningful and include a bit more info, be a bit more reflexive on what we bring to the table.}

% \FIXME{AAA - Other researcher self-disclosures:\\
% \textbf{CHI '21 - Exploring a Makeup Support System for Transgender Passing
% based on Automatic Gender Recognition}\\
% \\
% On the basis of
% this initial research as well as their HCI/CG/ML background, the
% first author proposed the initial idea of a virtual makeup system that
% supports transgender people’s need. Building on this initial idea, we
% formed an interdisciplinary team of researchers of diverse gender
% identities and different cultural backgrounds (Japan, Hong Kong
% and France) to develop this project. In terms of positionality [5] we
% also need to note that our experience with gender studies as well
% as transgender experiences is heavily influenced by our physical
% location: Japan.
% \\
% we argue,
% alongside many HCI researchers, that as a community we need
% to diversify the populations we are working with to let different
% voices be heard and acknowledged [19, 34].\\
% \\
% \textbf{It’s Complicated”: Negotiating Accessibility and
% (Mis)Representation in Image Descriptions of Race, Gender, and
% Disability}\\
% \\
% We then detail our interviews with 25 screen reader
% users, all of which identified as at least one of the following: Black,
% Indigenous, person of color (BIPOC), non-binary, or transgender}



%----------------
\section{Attitude Towards Risk}

\boldify{This is what attitude towards risk means, according to the GenderMag literature.}

In the GenderMag method, attitude towards risk (referred to just as ``Risk'' herein) is a spectrum of how people behave with technology when there are risks involved.
On one end of this spectrum are the risk-averse people, who do not like to use unfamiliar features because they would have to spend extra time to learn it;
if the feature fails, their attitude towards technology is negatively impacted. 
On the other end are the risk-tolerant people, who do not mind taking risks using unproven features of technology to achieve their task;
even if the feature does not work as intended, the person does not change their attitude towards technology.
In this section, we will discuss specifically how looking at people's attitude towards risk with the 10 dependent variables from Table~\ref{table:dependent_variables} led to some nuanced understanding of Li et al.'s results.

\FIXME{AAA@MMB: This safe to say? Feels too advertise-y.}

\input{doc/4.1-Init-Results}
% $Score_{Risk} = (\sum\limits_{q \in Q_{Risk}} q ) (\frac{ |Q_{Risk}| - numIDKs}{|Q_{Risk}|})$

\newpage

\input{doc/4.2-During-Results}

\newpage

\input{doc/4.3-WhenWrong-Results}

\newpage

\input{doc/4.4-OverTime-Results}

\newpage


%$Score_{Risk} = (\sum\limits_{q \in Q_{Risk}} q ) (\frac{ |Q_{Risk}| - \sum_{idk \in Q_{Risk}}idk}{|Q_{Risk}|})$

\subsection{``Initially'' Phase}

\input{figure/Risk/1-Initially/Risk-G1}

\input{tables/Risk/1-G1}

% \input{figure/Risk/1-R-G1}

\FIXME{\\
F5 - Overall, paired t-test, t(55) = 2.1566, p = .0354\\
PU - Overall, paired t-test, t(55) = 1.9606, p = .055\\
F5-Apply (Abi v. Tim), t(54) = 2.4985, p = .0155\\
PU-Apply, t(54) = 1.7751, p = .0814
} 

\boldify{Of the 10 dependent variables, the two that stood out was F5 and PU, so let's talk about their p-values and eta-squared}

Figures~\ref{fig:Risk-G1-F5} show the distributions for people's responses to the question ``I would feel productive while using the product'' (F5), and Figure~\ref{fig:Risk-G1-PU} shows the distributions for the question ``I would find the product useful'' (PU).
When considering people's attitude towards risk (left side of the figures) for F5, it is notable that both the risk-averse (orange) and risk-tolerant (blue) people had similar distributions when Guideline 1 -- Make clear what the system can do -- was violated.
However, although the guideline application significantly helped everyone on average (Paired%
\footnote{Levene's test for homogeneity of variance used to determine whether to use Welch's t-test (p < .05) or not, explicitly stated in our results. For within-subjects tests, we explicitly state that we use a paired t-test. }
%
t-test, t(55) = 2.1566, p = .0354), the risk-averse people received a significantly greater benefit than the risk-tolerant people (t-test, t(54) = 2.4985, p = .0155).
Some participants even noted this when asked why they preferred the application vignette, such as: \quotateInset{I prefer getting feedback as I go, it [would] really help me see where I can improve things on and fix it on the spot
}{Risk-Averse-}{95}{I think this reflects F5 the best because it's speaking about doing something better and improving i.e., being more productive.}
The PU dependent variable demonstrated a similar result, where the guideline application led to a marginally significant boost in people's averages overall (paired t-test, t(55) = 1.9606, p = .055%
\footnote{We consider $p \in (0,\ 0.05]$ to be significant, and $p \in (0.05,\ 0.1)$ to be marginally significant, by convention~\cite{cramer2004sage}}%
), but applying the guideline left a marginal disparity between the two groups' averages for perceived usefulness (t-test, t(54) = 1.7751, p = .0814), such as:
\quotateInset{[The Application] seems like it would provide more detailed and helpful feedback}{Risk-Averse-}{136}{PU quote}
%Further, for the PU dependent variable, people's averages for the guideline violation started off in similar areas, but applying the guideline provided a marginally significant advantage to the average for the risk-averse people (t-test, t(54) = 1.7751, p = .0814).
The eta-squared effect sizes (Table~\ref{table:Risk-G1}) triangulated these results, where the risk-averse people underwent a small effect change, but the risk-tolerant people did not undergo any observable effect.
These results represent the first kind of cognitive disparity in our findings, where post-stratifying by people's attitude towards risk unveiled a subset of dependent variables where people on one end of the spectrum (the risk-averse) underwent a change in their average when the guideline was applied, but those on the other end (the risk-tolerant) did not undergo any perceivable change.

\FIXME{AAA@MMB, this ending feels weak. The reader wants to know what these results mean in the larger context. I wanted to tie this into the fact that although AI is becoming more ubiquitous, it's still relatively mysterious to the masses. Then, tying it into people's attitude towards risk using unproven features... Dunno how to do it though, at least not right now.}

\subsection{``During Interaction'' Phase}




\input{figure/Risk/2-DuringInteraction/3-R-G4}

\subsubsection{Guideline 4 - ``Show contextually relevant information''}

\boldify{Figure 4 shows that post-stratifying by attitude towards risk tells a considerably different story than not, shown in Table~\ref{tab:G4-Stats} }

Figure~\ref{fig:Risk-G4-All}'s top row shows the post-stratified data, which considers people's attitude towards risk.
The bottom row, which does not post-stratify, tells the story that 8 of the dependent variables were not significantly different, and although \textit{two} of the dependent  variables (T1 \& T2) provided evidence for statistical differences (Paired t-tests, T1 -- t(63) = 2.0712, p = .0424; T2 -- t(63) = 2.0712, p = .0424) between the guideline violation and application, these differences failed to reach practical significance ($T1: \eta^2 = .012,\ T2: \eta^2 = .008$).
However, as Table~\ref{tab:G4-Stats} shows, post-stratifying by their attitude towards risk reveals significant disparities in the averages for \textit{90\%} of the guideline applications dependent variables between the risk-averse and risk-tolerant participants.
These opposing problem solving styles essentially cancelled each other out, masking the effects;
this points to the importance of considering such styles, with a ``worst case scenario'' of multiple response disparities between them.

% Figure~\ref{fig:Risk-G4-All}'s bottom row, which looks at all participants without considering cognitive diversity, shows that only \textit{two} of the dependent  variables (T1 \& T2) provided evidence for statistical differences (Paired t-tests, T1 -- t(63) = 2.0712, p = .0424; T2 -- t(63) = 2.0712, p = .0424) between the guideline violation and application, but  these differences failed to reach practical significance ($T1: \eta^2 = .012,\ T2: \eta^2 = .008$).



\input{tables/Risk/2-G4-PostStrat}


% \FIXME{\textbf{Guideline 4}\\
% Testing Overall F1 -- Paired t-test, t(63) = 1.227, p = .224\\
% Testing Overall F2 -- Paired t-test, t(62) = .7533, p = .4541\\
% Testing Overall F3 -- Paired t-test, t(62) = .51, p = .6119\\
% Testing Overall F4 -- Paired t-test, t(63) = 1.2786, p = .2057\\
% Testing Overall F5 -- Paried t-test, t(63) = 1.0442, p = .3004\\
% Testing Overall PU -- Paired t-test, t(63) = 1.5151, p = .1347\\
% Testing Overall T1 -- Paired t-test, t(63) = 2.4108, p = .0188\\
% Testing Overall T2 -- Paired t-test, t(64) = 2.0712, p = .0424\\
% NOTE - These last two were significantly different, but LOOK AT THE DISPARITY!!!!\\
% Testing Overall T4 -- Paired t-test, t(63) = 1.0433, p = .3008
% } 

%\subsubsection{Guideline 3 - ``Time services based on context''}
%\\

\input{figure/Risk/2-DuringInteraction/1-R-G3}

\FIXME{\textbf{Guideline 3}
\\Testing F3-Tims-- Paired t-test, t(33) = 2.9390, p = .006 (Abi not significant)\\
Testing T3-Tims -- Paired t-test, t(33) = 3.0767, p = .0042 (Abi not significant)\\
Testing T4-Tims -- Paired t-test, t(33) = 3.884, p = .0005 (Abi not significant)\\
What's notable is that all 3 of these are, overall, significant. It's like ANOVA really, because if we REMOVE observations and then lose the significance, the removed values are responsible for the significance.
}

% \input{figure/Risk/2-R-G3}


% \input{figure/Risk/4-R-G5}

% \input{figure/Risk/5-R-G6}

\subsection{``When Wrong'' Phase}

\FIXME{AAA@ALL - So I know that of the 5 values reported here for the differences between te applications, 4 of them are ``marginally'' significant. I want to make the argument that though there's a temptation to dismiss this, but we can't afford to for inclusivity's sake.}

% \input{figure/Risk/6-R-G7}

% \input{figure/Risk/7-R-G8}

% \input{figure/Risk/8-R-G9}

% \input{figure/Risk/9-R-G10}

% \input{figure/Risk/91-R-G11}

\boldify{Risk averse people prefer using features that they'll get more from, and some people mentioned this when they had to justify why they preferred the application vignette over the violation vignette, which we see in this quote and in the F1 dimension.}

Risk averse people prefer using features that they will get more benefit from~\cite{charness2012strong}, which might influence how they interact with an AI that helps make decisions in their lives.
Some of the participants provided insights to how they would feel in control when presented with the guideline application:
\quotateInset{Averse-2780}{}{I think [the application vignette] would make me feel more comfortable and in control of my data and information. It may only be a psychological sense of security, but I stand by my choice.}

Since the F1 dependent variable (Table~\ref{table:dependent_variables}) covers people's perceptions of control, we wanted to look if this was an isolated occurrence or not.
The striped boxplots in Figure~\ref{fig:Risk-G11} show the distribution of ratings when the guideline violated, and for feeling ``in control'', the average rating for the orange risk averse people is significantly lower than that of the blue risk tolerant people (Student's t-test, t(61) = 2.1352, p = .037), indicating that failure to apply the guideline will create a significant disparity between the two problem solving styles at opposing ends of this spectrum.


\boldify{Applying the guideline helped people, but the risk averse people found a greater benefit from it, with a medium effect size ($\eta^2 = 0.13$) over the risk tolerant people with a small effect size ($\eta^2 = .11$), but it wasn't enough to fully close the gap.}

Looking at how the distributions changed for guideline application (the solid box plots), both problem solving styles' averages changed by more than 1 point on the 7-point agreement scale.
This change is reflected in the $\eta^2$ effect size\footnote{ $\eta^2 = \sigma^2_{effect}/\sigma^2_{total}$, where we estimate the population variance with the sample variance.}, which is the amount of variation explained by the predictor variable (guideline application/violation) in the total variation for the outcome variable (feeling in control).
The risk averse people experienced a medium effect size ($\eta^2 = .13$), compared to the small effect for the risk tolerant people ($\eta^2 = .11$).
However, this did not fully close the initial disparity between the averages, since there was a marginally significant difference between the means (Student's t-test, t(61) = 1.8004, p = .077).
\FIXME{AAA@MMB: I wanted a call to action from this point, because we're seeing that applying the guideline doesn't close the gap (but it does help). Don't know if I should though, because any claim either opens me up to getting scooped or that it feels like an overreach.}

\subsubsection{Implications for theory}

\boldify{ Make an argument for why we shouldn't disregard marginal significance here, since it's based on the sample you got. There could still be a difference!}

In this section, 4 of the results (F1, F5, T1, and T2) had $p \in (.05, .1)$, which falls outside of $\alpha = .05$.
Thus, there's a temptation to disregard the result, because marginal significance has been a topic of debate for some time.
However, since the t-tests rely on the drawn \textit{sample} of participants, rather than the population, we argue that these results are still valid from an inclusive design perspective;
they are worth further investigation to see if the risk tolerant people's average \textit{does} end up significantly higher (or not), and the XAI research community should be aware of this to see if we can close this gap further.





\boldify{This wasn't the only attitude that people had, so we should take a look at them.. }



\quotateInset{Averse}{}{I would like to see the explained results, that way if I question them I have a reason why they may be wrong.
}

\quotateInset{Averse}{}{I don't necessarily like the ``smart'' aspects of either program (it feels inherently invasive to go beyond just mathematical equations), but I would prefer to see a detailed explanation of why/how a program came to the conclusion or suggestion that it did so that I can understand where it sees the patterns.}

% \subsection{Guideline 11 - Information Processing Style}

\quotateInset{Tolerant-2142}{}{I assume that if I give [the Application] data in the right way, it can automatically do a useful thing.}

%2142 demonstrates almost a nonchalance about why the system is doing what it's doing. They give the system data, and it spits out something useful.

\subsection{``Over Time'' Phase}

% \input{figure/Risk/92-R-G12}

% \input{figure/Risk/93-R-G13}

% \input{figure/Risk/94-R-G14}

% \input{figure/Risk/95-R-G15}

% \input{figure/Risk/96-R-G17}

% \input{figure/Risk/97-R-G18}



\subsubsection{One end of the spectrum needed more help}


\boldify{However, they weren't alone. In 4 of the experiments with differences in the aggregate, it turned out that half of the sample was driving that significance }

Participant 534 above commented that they thought the Application of Guideline 1 would empower the user to know what to expect from the system, and Figure~\ref{fig:R-G1-Productive} demonstrates that they were not alone in thinking so.
In fact, without disaggregating by attitudes toward risk, participants felt significantly more productive with the guideline Application over the Violation with a small effect size (paired t-test, t(55) = 2.1566, p = .0354, Cohen's d%
\footnote{Since this was a paired t-test, see Eq. (3) in Section~\ref{sec:analysis-methods}.}%
= .221 ), disaggregating by people's attitudes towards risk revealed that it was actually the \colorboxBackgroundForegroundText{AbiOrange}{black}{risk-averse} participants who felt significantly more productive with a medium effect size (paired t-test, t(25) = 2.6093, p = .0151, d = .512), but the \colorboxBackgroundForegroundText{TimBlue}{black}{risk-{tolerant}} participants' average did not perceptibly move  (paired t-test, t(31) = 1.0555, p = .2994, d = .122).
This suggests that the \colorboxBackgroundForegroundText{TimBlue}{black}{risk-{tolerant}} participants might have needed more help from the guideline Application.
Figures~\ref{fig:R-G1-Productive} \&~\ref{fig:R-G3-F3-T4} show that it was possible for either end of the attitudes toward risk spectrum could undergo such a change, while the other end needed more help, and this phenomenon showed up in half of the experiments (Table~\ref{table:Risk-NeedHelp}).
Notably, in 7 of the 8 experiments exhibiting this phenomenon, it was the \colorboxBackgroundForegroundText{AbiOrange}{black}{risk-averse} participants who had a lower mean (though not necessarily significant) for the Application vignette, which we turn to next.

\input{figure/01-Results-1/05-Risk-G1-G3-Drive}




%%%An old version of Section 4.3

% Now looking at Table~\ref{tab:triangulation-table} again,
% one of the insights that arose from this table was that of the 114, the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{``Abi''-like} participants were disparately impacted in 98 of them (85.96\%).
% However, one notable exception  to this was when the participants' data were disaggregated by their Information Processing Style %
% \footnote{The information processing style spectrum refers to how people process new information to solve problems.
% \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{comprehensive} problem-solvers gather fairly complete information before proceeding, whereas \colorboxBackgroundForegroundText{TimBlueQuote}{black}{selective} processors follow the first promising information, then potentially backtrack, in "depth first" order.
% }. %end of learning style footnote
% In 11 experiments, there were a total of 19 dependent variables exhibiting one of the three inclusiveness insights.
% What differentiated the information processing style disaggregation from the other four was that the 
% There were a total of 19 insights found across 11 of the 16 experiments, it was the \colorboxBackgroundForegroundText{TimBlueQuote}{black}{Tim-like selective} information processors who were disparately impacted in 11 of them (57.9\%).

% \colorboxBackgroundForegroundText{TimBlueQuote}{black}{Tim-like selective} information processors who were disparately impacted about half of the time.
% This highlights the importance of considering all 5 problem solving style spectra, rather than focusing on one.


% suggesting the need for further research to find (and fix) inclusiveness issues with AI-powered systems through problem solving style disaggregation.



% \subsubsection{Motivations, Learning Style, \& Information Processing Style %**beginning is D2, end is D0.5
% }


% % \FIXME{MMB@AAA: not happy with how this subsubsection is fitting into the "plot".  We've already talked about a "mystery" (InfoProce) and the only thing to say after saying the differences is that we have even less info about these two. Must fix, not sure how.\\
% % One idea: ?move this first, so that we can lead into Info Proc with "here's another mystery, but for this one it's clearer to proceed"?\\
% % Open to other ideas too...}

% \boldify{The dependent variables for motivations \& learning style didn't appear to make sense, and the qualitative data also didn't help us make sense of it. It remains an open question about this.}

% Although disaggregating participants' data by their motivations%
% \footnote{The motivations problem solving style is about the spectrum of reasons why people interact with technology: from being \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{mainly to accomplish a task} to interacting with technology \colorboxBackgroundForegroundText{TimBlueQuote}{black}{for the enjoyment of technology}.
% } %end of motivations footnote 
% , learning style%
% \footnote{The learning styles spectrum referred to is specific to how people go about figuring out new technologies: from a \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{``top-down'', process-oriented style} (i.e., learning the features in the context of a process that involves those features) to a more \colorboxBackgroundForegroundText{TimBlueQuote}{black}{``bottom-up'', tinkering style} of exploring new features without the context of a process.
% } %end of learning style footnote
% , and information processing style%
% \footnote{The information processing style spectrum refers to how people process new information to solve problems.
% \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{comprehensive} problem-solvers gather fairly complete information before proceeding, whereas \colorboxBackgroundForegroundText{TimBlueQuote}{black}{selective} processors follow the first promising information, then potentially backtrack, in "depth first" order.
% } %end of learning style footnote
% uncovered significant differences in 13 unique experiments for the three categories of insights in Section~\ref{subsec:3-categories} (Appendices~\ref{subsec:Appendix-Motivations},~\ref{subsec:Appendix-LearningStyle}, \&~\ref{subsec:Appendix-InfoProc}),
% participants' free-text responses did not help us understand why these differences existed, like in Section~\ref{subsubsec:Risk-forDesigners}.
% For example, there was no references to concepts commonly associated with their motivations (such as ``accomplishing a task/having fun''), learning style (like ``following a process/clicking around''), or information processing style (like needing ``more/less'' information).
% Without additional information to ground ourselves in, like the discussion in Section~\ref{subsubsec:Risk-forDesigners}, we could only conjecture why such differences existed for these three problem solving styles.


% \input{figure/2-G5-SE}
% %----
% \subsubsection{Computer Self-Efficacy %**D2.2
% }


% %\FIXME{MMB@AAA: same problem as previous two subsections. Same hint as for those.}
% % \FIXME{MMB@AAA -- this one needs some rework.  There's little content  here, but I thought we said it was an  interesting one.  Needs quotes, or discussion, or more about what SE is as it relates to this, or some such.  See if you can make it at least as interesting as the Info Proc section.}

% \boldify{First, SE. This might look the same, but each disaggregation brings new perspective and understanding.}

% However, participants' qualitative responses across multiple experiments did leave clues that tied explicitly to their Computer Self-Efficacy, and we found examples of \textit{all three insight categories} from Section~\ref{subsec:3-categories}.
% Prior research with computer self-efficacy has uncovered information about how people solve problems, apply cognitive strategies, and how persistent they will be in getting through a problem~\cite{stumpf2020gender,bandura1986explanatory}.


% % \FIXME{AAA@MMB: Really want to make a tie to adequacy here, perhaps the ``blames themselves'' for Abi? I think that's what we want to strike on for the reader here.
% % }

% Guideline 13 (learn from user behavior) was the only guideline where disaggregating by participants' computer self-efficacy uncovered all three categories of insights, shown in Figure~\ref{fig:SE-G5}.
% On the left, notice that the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{lower self-efficacy} participants' rating of feeling certain was significantly lower with the Violation AI (t(67) = -2.0091, p = .0468, d = .484) than their \colorboxBackgroundForegroundText{TimBlueQuote}{black}{higher self-efficacy} peers.
% However, in the Application AI product, this disparity \textit{closed} (t(66) = -1.2674, p = .210), reminiscent of the result in Section~\ref{subsec:category-1}.

% Although the Application AI product closed this gap in feeling certain, it inadvertently \textit{introduced} a different gap (Section~\ref{subsec:category-2}), seen in the ``Not Harmful'' plots.
% With the Violation AI product, there was already evidence pointing towards the lower self-efficacy participants rating the system significantly more harmful than the higher self-efficacy participants (t(55) = -1.7962, p = .078, d = .478).
% However, the Application AI product did not shift the lower self-efficacy participants' average much (0.039), but the higher self-efficacy participants derived 14 times more benefit (0.55), which tipped the difference enough to result in a significant difference (t(55) = -3.9091, p = .0003, d = 1.040).

% The right of Figure~\ref{fig:SE-G5} shows the ``Pervasive Gaps'' category, where the lower self-efficacy participants felt significantly less in control than the higher self-efficacy participants in both the Violation AI product (t(55) = -3.0581, p = .005, d = .0.813) and the Application AI product (t(55) = -3.0859, p = .003, d = .830) cases.

% Similarly to Section~\ref{subsubsec:Risk-forDesigners}, participants' responses to why they preferred either the Violation or Application AI system also tied explicitly to their computer self-efficacy. 
% For example, some lower self-efficacy participants thought that the Violation AI product's word choice for Guideline 5 (match relevant social norms) was abrasive, which helped explain why the lower self-efficacy participants felt significantly less secure with the Violation AI product (t(67) = -2.2141, p = .030, d = .534):

% \quotateInset{I do think that the wording used by [Violation AI product product] is a little too abrasive and straight to the point. It could potentially upset someone...}{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G5-1196-lower}}{}{I do think that the wording used by Ione is a little too abrasive and straight to the point. It could potentially upset someone, whereas "Consider using..." from Kelso likely would not upset anyone directly by implying that they made a mistake. All other aspects of the applications being equal, I would prefer to use Kelso and its neutrality, because I would expect the get to the same result without the added negativity that surrounds the word "mistake".}

% \quotateInset{It would be disconcerting to be constantly told I was making mistakes.  Much prefer a suggestion like [Application AI product product].}{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G5-2493-lower}}{}{It would be disconcerting to be constantly told I was making mistakes.  Much prefer a suggestion like Kelso.}

% The prevalence of the Category 2 and 3 insights for self-efficacy in Table~\ref{tab:summary-table} suggested that neither the Violation nor the Application products seemed to meet the needs of the lower self-efficacy participants for these experiments;
% this is an important note for designers, since Stumpf et al. reported that a failure to meet the needs of people like these participants could lead them to not be as willing to use it in the future~\cite{stumpf2020gender}.






% \FIXME{This is the last sentence. No more after this one.}




%-------






This is the old facet-by-facet analyses from Section 5.
I stopped buying them because the reviewer, if they're stat heavy, is looking for logistic regression, rather than simple trend lines.
Having two categorical variables really screwed us up.

Were there patterns in any of the five problem solving styles that might help explain why these skews existed across the two demographic dimensions?




\textit{Attitudes towards risk:}
Research studying attitudes toward risk and age has found that 18--24 year old people were more likely than older age groups to engage in potentially dangerous activities~\cite{fruhauf2017qualitative,zicat_2018}.
Dohmen et al. also found that their participants' willingness to take risks declined linearly until around 65 years old~\cite{dohmen2017risk}.
In autonomous systems, work tying risk to technology usage found that older people's perceptions of autonomous vehicles were more negative than younger people's, due to perceived risks~\cite{hulse2018perceptions}.
Further, McIntosh et al. found a usability bias against elderly people by leveraging people's risk attitudes in their e-commerce analysis~\cite{mcintosh2021evaluating}.
\input{figure/6-risk-se-info-trends}

% Others have studied how gender aligns with attitudes toward risk.
% For example, Umamaheswar \& Tan~\cite{umamaheswar2020dad} discovered that even when the amount of risk to men and women is comparable (in their case, the risk of the novel coronavirus), the attitude and response to that risk is different for these two genders, where women reported more frequently than men the heightened concerns and anxieties of contracting the virus.
% They also highlight the rich body of research that supports differences between gender and attitudes toward risk (e.g., ~\cite{gustafsod1998gender,panno2018women,reid2004gender}).
% \boldify{Isn't it interesting how the skews are moving ever leftward for both genders as ages progress?  Why might this be? Well... }

\boldify{The literature surrounding the intersection of gender and risk is relatively unexplored. We have a graph to try and fill a wee bit of that gap.}

% \begin{wrapfigure}{o}{.47\linewidth}
%     \centering
%         \includegraphics[width = 0.9\linewidth]{assets/Risk-by-age-trend.pdf}
%         \caption{The trend lines for the proportion of risk-averse women (orange) and men (blue) across different age groups (x-axis).
%         The men mimicked Dohmen et al.'s finding of increasing risk-aversion as age increased (i.e., decreasing willingness to take risks), whereas the women grew \textit{less} risk-averse. 
%         }
%     \label{fig:risk-by-age}
%     \vspace{-8pt}
% \end{wrapfigure}

Our participants' data for their gender, age, and attitudes toward risk are shown in Figure ~\ref{fig:risk-by-age}.
For each of the age groups (x-axis), the data show the proportion of men (blue) and women (orange) who were more risk-averse.
Although the men followed a similar pattern to Dohmen et al.~\cite{dohmen2017risk}, becoming increasingly more risk-averse as age increased, the women's showed an inverted pattern to this, becoming \textit{decreasingly} risk-averse with age.





\boldify{Others have shown that there's a negative relationship between age and SE/Mot.}
%



\boldify{Let's talk about self-efficacy with age}

\textit{Computer self-efficacy: }
Other researchers have investigated the relationship between computer self-efficacy and age.
For example, Lopez et al.~\cite{lopez2017teacher} found a strong negative correlation between people's ages and their self-efficacy with information communication technology%
\footnote{Their correlation coefficient was significant even under $\alpha = .01$.}.
Further, Schreder et al.~\cite{schreder2013age} found that age was typically linked to lower computer self-efficacy.

Researchers have attempted to establish an interaction between computer self-efficacy, gender, and age.
For example, Schreder et al.~\cite{schreder2013age} looked for such a relationship but did not find evidence of an interaction between gender and age when people used self-service terminals.
However, Vsabic et al.~\cite{vsabic2021teachers} found ``minor gender differences in self-efficacy for using [Information Communication Technology] ICT that are more prominent among older teachers and practically non-existent among younger teachers.''
 
Figure~\ref{fig:self-by-age} shows the proportion of women and men who had lower self-efficacy relative to their peers.
The participants' self-efficacy seem to mirror Vsabic et al.'s finding;
there was hardly any difference in the proportion of lower self-efficacy women and men in the 18---24 years old group, but the trend in this difference increased in the older groups, with a higher percentage of women who had lower computer self-efficacy than the percentage of men.
%suggesting a main effect between gender and computer self-efficacy when considering age, but with little-to-no interaction.

\textit{Information processing style:}
Research surrounding information processing style and age often focus on the physiological changes that come with ageing might influence how people process information.
For example, Gell et al. researched people interacting with information-rich technology like email.
They found that the way their participants interacted might change based on barriers such as vision and memory impairments as they grow older~\cite{gell2015patterns}, a finding repeatedly found across the literature (e.g.,~\cite{mcintosh2021evaluating,torrens2020lacking}.
Figure~\ref{fig:ip-by-age} suggests that there was no meaningful difference in this sample of participants' information processing styles across gender, age, or the interaction between them.





% Meyers-Levy \& Loken~\cite{meyers2015infoProcessing} reported research on the information processing style of  men and women, and they detailed the mixed reports where there were both gender differences and none.
% Figure~\ref{fig:ip-by-age} suggests that for this sample of participants, there was no evidence to suggest a difference in their information processing styles across both gender and age.



\textit{Learning style: }
Research investigating people's learning styles and age have measured it with different scales such as the Learning Style Inventory~\cite{admiraal2011learning} or the Myer-Briggs Type Indicator~\cite{li2011exploratory}.
However, both of these found insufficient evidence to suggest an interaction between age and learning style.
Our data suggests something similar (Figure~\ref{fig:learn-by-age}), where the proportion of both process-oriented and tinkering-oriented learners steadily increased across age groups at the same rate.
The women, on average, had 13\% more process-oriented learners than the men did (standard deviation: 2.8\%)
\input{figure/7-mot-learn-trends}



\textit{Motivations: }
Since people interact with technology for a variety of reasons, it is important to capture such motivations and if demographic information such as age plays a role.
For example, van der Groot \& Pilgrim~\cite{van2019exploring} found qualitative differences between their participants' age and their {Motivations} to interact with chatbot technologies.
Further, Gish et al.~\cite{gish2017driving} found in their study of 35 older people driving vehicles with Advanced Vehicle Technologies (AVTs) like lane departure warning three main themes in their data;
participants believed that AVTs could counteract changes in participants' driving performance, that they were devices of convenience, and that AVTs could enhance safe driving, reminiscent of a both task-oriented (changes in performance \& safe driving) AND tech-oriented (devices of convenience) motivations.

Looking at the proportion of participants who had task-oriented motivations (Figure~\ref{fig:mot-by-age}) corroborated such findings about participants' ages factoring in, but it also suggested that gender did too.
For example, across the age axis, the proportion of both women and men with task-oriented motivations increased on average nearly 10\% between consecutive age groups (women's avg.: 9\%; men's avg.: 8\%).
Further, the proportion of women who were task-oriented was 15\% larger than the men on average for each age group (standard deviation: 5.1\%), demonstrating a main effect of gender on motivations.


From the background



% eXplainable AI (XAI) is a resurgent subarea of research, aiming to increase transparency of these algorithms through how it presents information in an interface.
% This in turn might might help people identify and mitigate unfairness and inclusivity issues in AI-powered systems.
% One way to potentially approach this would be if the AI provided explanations, resulting in eXplainable AI (XAI).
% This resurgent subarea of research aims to increase transparency to AI.
% , which in turn helps users form reasonably correct mental models.
% (In the context of user experiences with AI, a mental model is someone's internal representation of how an AI works~\cite{norman1983mental}.)
% For example, Dodge et al.~\cite{dodge-fairness-2019} empirically investigated four different explanations to assist people in identifying unfairness issues in the raw COMPAS dataset, as well as a ``de-biased'' version.

% They found that different explanation types yielded different results, with some seen as ``more'' or ``less'' fair.
% However, explanation types can come in many forms, and they might present different types of \textit{information}.
% One balancing act for designers of AI-powered systems comes from assessing which type of information to convey.
% %presenting such explanations to users is equally challenging.
% For example, Lim \& Dey researched intelligibility types to leverage the information that people asked a system to inform them of what information explanations might contain~\cite{lim2009and,lim2009assessing,lim2012improving}, and Kulesza et al.'s worked on a set of principles of how developers might explain intelligent systems~\cite{kulesza2015principles}.

% Dodge et al. also found that the granularity of explanations mattered too, where local explanations were reported to be more effective at exposing unfairness issues.
% Others have looked at local explanations (explaining specific choices that a system makes~\cite{plumb2018model,guidotti2021evaluating,nguyen2018comparing}), global explanations (how the system reasons about categories of choices~\cite{wu2020towards,mikolajczyk2020global,popordanoska2020machine}), or both~\cite{setzu2021glocalx,hohman2019gamut,lundberg2020local}.

% However, there are also myriad other ways to explain either of these explanation types, such as counterfactual reasoning (showing what needed to have changed to create a different outcome~\cite{goyal2019counterfactual,mothilal2020explaining,Neal_2018_ECCV}), the importance of system inputs~\cite{anderson2020mental,alqaraawi2020evaluating,kenny2021explaining}) or its outputs~\cite{anderson2020mental,van2018contrastive})~\footnote{A full survey of the XAI literature is beyond the scope of this paper, but such surveys exist, like Mueller et al.~\cite{mueller2019explanation}.}.
% % Our work builds upon these by considering people's diversity of thought during HAI interaction.
% % instead measuring diverse people's reactions toward AI systems applying or violating a human-AI guideline.

% \boldify{Most closely related to this paper is work on how well AI serves different populations of stakeholders}

% Some research investigated in a few domains how well AI serves participants with knowledge in those domains.
% For example, Madumal et al. found amongst StarCraft II players that given four possible explanations, there were no differences in trust four possible explanations~\cite{madumal2019RLcausal}.
% Juravle et al. found that medical practitioners trusted AI-assisted diagnoses significantly less than human-assisted diagnoses~\cite{juravle2020trust}.
% Further, Ehsan et al.~\cite{ehsan2021expanding} found that their proposed Critical Technical Practice paradigm assisted sellers and developers of AI-powered systems in calibrating trust in AI systems.
% Our work expands upon these by considering AI-powered systems in the broader domain of productivity software with AI-powered features.


%Further, the display of information (text vs. scatterplot) played a significant role on whether or not participants included a feature, with people preferring text-based explanations over scatterplot.
% However, our work differs because we focus on the user experience of people who the AI is acting upon, whereas their participants were deciding whether (or not) to include outcome variables when they were shaping an AI.

%However, their disaggregation through dimensions such as people's age led to skewed samples (their Figure 3)

%67.1\% of the participants we investigate had either had no computer science experience (26.1\%) or had taken only one computer science course (41.0\%), providing a different perspective on how people might respond to inherent risks in the system.




\subsection{Algorithmic inclusiveness of AI
\draftStatus{2.35}}

\label{sec:fair-ai}

% A significant body of work has investigated increasing recruitment and/or retention across genders in in-person CS education, and these works ...

% Research related to our own broadly fit into two categories: 1) how people have worked on equitable, fair, and inclusive AI {algorithms} (i.e., ``under the hood'' inclusivity), 2) empirical work on human-AI interaction (i.e., ``over the hood'' inclusivity).

\boldify{One branch of research for diversity in artificial intelligence deals with diversifying data, model, and inference in ML models~\cite{Gong2019Diversity}.  }

% One area of research to improve diversity and equitability of the ways designers of AI-powered systems can improve how ethically an AI behaves is to try and ensure it behaves similarly across different populations.
An ``under the hood'' area of research which has seen a surge in publications in the last decade investigates how to make the AI \textit{algorithms} more equitable, fair, and inclusive.
For example, ACM FAccT is an entire conference series devoted to reporting on such issues.
Among the approaches researchers are exploring are the models themselves, diversifying training data, the models by parameter adjustment or training multiple models, or the inferences that the model makes, such as the model predicting a ranked list of possibilities rather than a single classification~\cite{Gong2019Diversity}.
One of the most famous examples of unfairness was the COMPAS data set, which has been used in research to demonstrate negative outcomes like how an algorithm's prediction of people's recidivism risks were different based on their race, even with similar numbers of prior convictions~\cite{propublica-compas}.
Crawford's keynote address~\cite{crawford2017trouble} raised many kinds of negative outcomes%
\footnote{In Crawford's work, she uses the term ``harms'' to capture this.} 
from AI and noted that fairness in AI is a socio-technical problem.
Some of these negative outcomes include differing quality-of-service or allocation of resources, inequitable representation, and more.


\boldify{These harms can show up in a bunch of domains, including student-college matching, voice...}

Researchers have begun investigating such negative outcomes in several domains.
For example, Robertson, Nguyen, and Salehi discussed negative outcomes within the context of matching students to schools, where several barriers arise such as the mismatch between how engineers' modeling assumptions and users' real-world goals and constraints~\cite{robertson2021modeling}.
In the domain of speech captioning, Tatman~\cite{tatman2017gender} found disparities in YouTube's automatic captioning feature between male and female voices, dialects from different areas (e.g., Scottish dialects' error rates were the highest), and the interaction between them.
Disparities like these not only disproportionately affect individuals whose speech the system struggled to understand (e.g., females and Scottish people) but also disproportionately impact members of the Deaf community.
%One approach to solving this issue in voice-recognition focused on proposing new models to try and close this disparity (i.e.,~\cite{livieris2019gender, zvarevashe2018gender}).


\boldify{... for NLP...}

Another domain investigating negative outcomes for particular populations is Natural Language Processing (NLP) algorithms.
For example, Leavy~\cite{leavy2018gender} reported on gender bias in NLP across five different dimensions, like naming (e.g. ``female lawyer'' vs. ``lawyer''), ordering (e.g., having man before woman in ``man/woman''), and biased adjectives (e.g., use of the term ``gossiping'' for women vs. ``affable'' for men).
These highlight potential negative stereotypes, which disparately impact some people over others (in Leavy's case, females).
Sun et al. provide a comprehensive review of under-the-hood bias problems and mitigation strategies for NLP~\cite{sun2019mitigating}.
%--- the need for diversifying training data~\cite{zhao2019gender,zhao2018gender}, the model~\cite{zhang2018mitigating}, and the inference~\cite{lu2020gender,kiritchenko2018examining} .

\boldify{... and for image data.}

Researchers have also investigated negative outcomes in image data for gender, race, and intersections of gender and race.
For example, Buolamwini \& Gebru found that the image classifiers they investigated performed better on male faces than on female faces, and better on lighter faces than darker faces---but performed worst on darker female faces~\cite{buolamwini2018gender}.
Wilson et al. reported self-driving cars detecting the presence of light-skinned pedestrians better than dark-skinned pedestrians~\cite{wilson2019predictive}.
Rose reported on a phenomenon with classifying photographs, where the algorithm mistakenly believed that people of Asian descent were blinking, even though they were smiling for the photo~\cite{rose_2010}.

Guo et al.~\cite{guo2019toward} comprehensively reported on the disparate impacts of speech-, text-, and image-processing systems for people with disabilities.
% Although algorithmic fairness is outside the scope of this paper, it is still an important topic to raise when discussing diversity, equity, and inclusion, and the negative outcomes discussed here are only handful of the research dealing with biases in AI~\cite{nasr2020bidding,yang2020towards}.
Other comprehensive surveys of algorithmic fairness and accountability in AI literature include Mehrabi et al. and Wieringa~\cite{mehrabi2019survey,wieringa2020account}.
However, these works focus on under-the-hood aspects of AI equity.
In contrast, our work investigates the ``over-the-hood'' user experiences of people's interactions with AI.


%OLD INTRO STUFF
No two individuals are alike.
Just as the individual differences among people in our world are myriad and complex, so too are the individual differences among people who interact with AI-powered systems.
However, despite a growing body of literature on how to improve human-AI (HAI) interaction~\cite{amershi2019guidelines,kulesza2015principles,lim2012improving,wang2019designing, shneiderman2020bridging, wickramasinghe2020trustworthy, schneider2020human},
%in areas like medical assistance technology~\cite{gandhi2019intellidoctor,lin2019ten,jacobs2021designing, admiraal2011learning,haboucha2017user,Schneider_AV_modalities,sundaresan2019code},
little is known about how AI designers can design interfaces inclusively for diverse populations during these interactions. 
%\FIXME{MMB@AAA: (1) need cites above to make sure we've covered all the well-known HAI guidelines (2) these will also have to be discussed in the Related Work section}



% \FIXME{MMB: Reader liked the 1st parag, but lost the scent at the 2nd parag: "why am I reading about GenderMag". needs a connection -- the boldif is better than the topic sentence.  Maybe the last sentnce of this parag should instead be the topic sentence?}

\boldify{what implications should user diversity have on HAI? Let's think about that thru the lens of diversity of thought }

Users' diversity should be considered in the design of interactive AI systems, but how can HAI designers choose which diversity dimension(s) to consider: should they strive for inclusive HAI systems across different gender demographics, age demographics, and/or across some other diversity categories?


We believe that it might be possible to cut across demographic diversity categories like age or gender, by focusing instead on an underlying motivator for why companies and institutions strive to support diversity---\textit{diversity of thought}.
%
%\FIXME{MMB@MMB: Must decide whether to keep the current last sentence or cut it. I like the above sentence, but ending on the sentence before is punchier.}
%
%\boldify{here's why care about diversity of thought and what kind we mean }
% Although the motivation of some organizations to support demographic diversity is to gain better reputations as ethical corporate/institutional citizens, other organizations are motivated by the diversity of thought that demographic diversity brings.
%AAA@MMB: The above line was very unclear, and it seemed to assume a lot about organizational motivations. I found myself asking ``how do you know that?''
Diversity of thought has been shown to have many positive effects on organizations, including better ability to innovate and a better ``bottom line'' for businesses~\cite{larkin2020diversity, page2019diversity, phillips2014diversity}.
The type of diversity of thought we consider in this paper is the diverse ways different individuals go about thinking their way through a problem or obstacle to achieve some outcomes or at least some understanding of an outcome.
% Thus, the diversity aspect we consider in this paper is diversity of thought---more specifically, the diverse ways different individuals go about thinking their way through a problem or obstacle to achieve some outcome or at least some understanding of an outcome.  
We will refer to the ways an individual goes about this kind of problem-solving as their ``problem solving style.''


\boldify{we used GenderMag to find out}
To investigate how people's diverse problem solving styles%
\footnote{In GenderMag publications, GenderMag's problem solving styles have also been called ``facets'' or ``problem-solving styles.''} relate to their user experiences with AI systems, we leveraged the problem solving style survey from the Gender-Inclusiveness Magnifier (GenderMag) method~\cite{burnett2016gendermag}.% 
GenderMag is an empirically validated method~\cite{burnett2016gendermag,hill2017gender,padala2020gender,vorvoreanu2019gender} with a dual gender/cognitive focus, and its problem solving style survey is a validated instrument that has been used by industry, open-source communities, and academic organizations~\cite{guizani2022debug,hilderbrand2020engineering, vorvoreanu2019gender}.

\boldify{We performed a secondary analysis on Li et al.'s data. Here's what that means...} 

Fortunately, problem solving style survey data on over 1,000 of participants from a recent HAI investigation was available to us to analyze from a problem solving styles perspective.
In Li et al.'s empirical investigation~\cite{li-MSR-work} into the efficacy of Amershi et al.'s HAI guidelines~\cite{amershi2019guidelines}, the participants self-reported their problem solving styles using the GenderMag problem solving style survey.
The participants were distributed across 18 experiments whose primary collective purpose was to evaluate the effects of applying (or violating) the guidelines for human-AI interaction. 
We used these data in a secondary analysis%
\footnote{A secondary analysis is analysis of data ``which were originally collected for other purposes''~\cite{glaser1963, johnston2014secondaryAnalysis}, enabling the analyst to pursue a research direction that is distinct from that of the original work.}
to investigate what insights could be gleaned by disaggregating participants' data by five problem solving style spectra.

Specifically, our secondary analysis investigated how 
disaggregating by participants' diverse problem solving styles impacted their user experience outcomes with AI systems that applied or violated Amershi et al.'s HAI guidelines.
We also investigated how the resulting problem solving style insights related to two demographic diversity groupings more traditionally used in diversity investigations, namely gender and age.
Thus, our research questions were:



%--------MMB: I commented this out for now -- seems to just duplicate the RQs.
%This paper contributes the following:
%\begin{itemize}[ leftmargin = 8px ]
%    \item Reveals disaggregating 1000+ participants by their problem solving styles yielded new insights into the diverse users' experiences in human-AI contexts.
%    \item Reveals how the 1000 participants' problem solving styles relate to their gender- and age-diversity demographics.
%\end{itemize}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This was the old stuff from the hypothesis version





\boldify{We're beginnning with end users' attitudes toward risk, which we chose because it doesn't take much to consider that AI can be risky.}

Researchers have already identified the growing risks of artificial intelligence (e.g.,~\cite{yigitcanlar2020contributions,boukherouaa2021powering,zanetti2020potential}), creating a natural connection to begin our investigation by considering the ``attitudes toward risk'' problem solving style.
We then generalize our findings 

\boldify{AI is risky, and others have already identified the risks. This led to our first hypothesis.}

This paper reports on the second investigation, which considers whether problem solving style disaggregation uncovers previously unseen insights into HAI data.
As an example of the pertinence of problem solving styles, other research has indicated the growing risks of Artificial Intelligence (e.g.,~\cite{yigitcanlar2020contributions,boukherouaa2021powering,zanetti2020potential}), and one of GenderMag's problem solving style types captures an individual's attitudes toward risks in technology.
Thus, our first hypothesis was:

\FIXME{Remove the term ``hypothesis'' from this paper. They're going back to RQs}

\begin{enumerate}[ label = {}, rightmargin = 30px]

\item \textbf{RQ1:} \textit{How do HAI users' experiences differ between violations/applications of human-AI interaction guidelines when considering their diverse attitudes toward risk?}
\item \textbf{RQ2:} \textit{Do such differences in user experience exist beyond end users' attitudes toward risk into GenderMag's other four problem solving styles?}
\item \textbf{RQ3:} \textit{Beyond these guidelines for human-AI interaction, how can the alignment of end-users' problem solving styles and demographic data help HAI practitioners understand more about their target audience?}
% \item \textbf{H1-CognitiveDiversity-RiskStyle: } \textit{Risk-averse and risk-tolerant HAI users' experiences will exhibit disparities in UX metrics for human-AI interaction.}
\end{enumerate}

\boldify{However, that's supporting just one facet, and other researchers have shown that leveraging all 5 facets uncovers information too.}

Beyond risk, prior research with \textit{non}-AI systems has shown that various technology features can disparately impact people via any one of GenderMag's five problem solving style types.
Our second hypothesis considers this possibility with AI-powered systems:

\begin{enumerate}[ label = {}, rightmargin = 30px]
\item \textbf{H2-CognitiveDiversity-5Styles: } \textit{Insights found in human-AI interaction data by disaggregating participants' data by their attitudes toward risk will also be found in the remaining four GenderMag problem solving style types.}
\end{enumerate}


%\FIXME{AE4\\
%MMB@AAA: fix hyps as per spelling in TODO document (be careful with hyphens -- use as in TODO) \\
%MMB@AAA: Hyp bodies need work. Move motivational stuff OUT of the hyps and have it as text that leads into the hyp.  Also, do subject-verb-object check (eg, are we really proving that "findings...impact users"?), and otherwise trim to what's really the hyp}

\boldify{Lastly, GenderMag can help us understand more about our users, rather than about their experiences, leading to our last hypothesis!}

Last, we hypothesized that if \textbf{H1-CognitiveDiversity-RiskStyle} or \textbf{H2-CognitiveDiversity-5Styles} are supported, then problem solving style disaggregation can also shed light on demographic differences in people's HAI experiences.
The demographics we focused on were gender and  intersectional gender-age:

\begin{enumerate}[ label = {}, rightmargin = 30px]
\item \textbf{H3-Demographics:} \textit{Human-AI interaction participants' problem solving style values will cluster by gender groupings and will cluster by  intersectional groupings of gender and age.}
\end{enumerate}










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Old Methodology stuff below






\clearpage

\FIXED{
\subsection{Experimental Methodology \& Phase One Result Summary
\draftStatus{D2.5}}
\label{sec:li-original-methods}

\boldify{Here's what Li et al. were interested in, and I'll describe the experimental setup in detail.
Each experiment was a 2 x 2 factorial design, where one factor was within-subjects (guideline Application/Violation), and the other was between-subjects (AI-quality).}

The investigation wanted to gauge the efficacy of  Amershi et al.'s~\cite{amershi2019guidelines} guidelines for Human-AI interaction, recruiting 1,043 participants and randomly assigning them to one of 18 experiments, one for each guideline.
Each experiment was a 2 x 2 factorial experiments, and the experimental independent variables were 1) adherence to the guidelines as a within-subjects factor (levels: Guideline Violation \& Guideline Application) and 2) AI-quality as a between-subjects factor (levels: optimal \& sub-optimal).
For example, Experiment~11 was the experiment to gauge the efficacy of Guideline~11.

Like several other human-AI works (e.g.,~\cite{lima2021human,abendschein2021influence,mckee2021understanding,davis2022gender,lee-efficientAnnotations}), each AI system  was represented by a vignette\footnote{All vignettes for both guideline violations and applications can be found in Appendix~\href{https://web.engr.oregonstate.edu/~anderan2/MSR-Appendices/Appendix-Vignettes.pdf}{{\color{blue}B}}};
in a random order, participants saw a vignette which described an interaction with a system that applied the studied guideline (i.e., the \appProduct{}) and a vignette which described an interaction with a system that violated the guideline (i.e., the \vioProduct{}).
All vignettes described systems from productivity software systems: document and slide editors, search engines, email applications, and spreadsheet applications. 

For each vignette, participants answered questions (Table~\ref{table:dependent_variables}) on a 7-point Likert scale from ``Strongly Disagree'' (encoded as a ``1'') to ``Strongly Agree'' (encoded as a ``7''), with an option to reply with ``I don't know''.
After participants saw both vignettes, they were asked to describe the differences between the two products and which of the two products they would prefer (and why).
Finally, they filled out demographic information, including the GenderMag problem solving style survey.

\boldify{Here's what the vignettes looked like, so you have a bit of context for our discussion}

Table~\ref{table:G1-Vignette} provides an example of one experiment's pair of vignettes.
Each vignette had three parts: 
\begin{enumerate}
    \item The \textit{introduction to the product and feature} set up the context for the product, describing what the product did and the AI-powered feature that the participant would interact with.
    \item The \textit{product behavior description} described how the product behaved in the \appProduct{} and the \vioProduct{}, which manipulated the independent variable.
    \item The \textit{AI performance description} described how well the product did its job, which could be optimal (i.e., it worked well most of the time) or sub-optimal (i.e., the product sometimes made mistakes and sometimes worked well).
\end{enumerate}
For (3), the phase one analysis showed that the AI performance factor had a substantial practically significant interaction effect for \textit{only} Guideline 13's (learn from user behavior) experiment.
Therefore, AI optimality was not considered as a factor across all experiments.
We keep this finding in phase two.

%\input{tables/02-F1-Vignette/G1-Vignette}




\boldify{What they found was that for the 16 experiments, applying the set of guidelines was almost always preferred over the violation for both how products were perceived and on the user experience, but there were some exceptions (such as G4 and G13)}

\subsubsection{Investigation One Result Summary}
\label{subsec:investigation-one-results}
The phase one analyses found that for the 16 successful experiments, the \appProduct{} (which applied the guidelines) generally resulted in products being perceived as more useful and better for the user experience.
However, in some instances, participants may perceive that when designers apply some of the guidelines (such as Guideline 4 and Guideline 13), users may find that designs to personalize the system might be limiting.
%End FIXED
}
%---------
\subsection{Investigation Two Analysis Methodology
\draftStatus{2.5}}
\label{sec:anderson-methods}

% \subsubsection{Our subset of Li et al.'s participants}

\boldify{We wanted to perform our concurrent analysis on this data because 1) to our knowledge, it was the only study on human-AI interaction that would incorporate the GenderMag problem solving style survey and 2) It would enable us to uncover additional information like a) when the guidelines are violated, are such violations \textit{worse} for some more than others, b) when the guidelines are applied, are such applications \textit{better} for some more than others.}


Phase two of the analyses on these data seeks to uncover how users with certain problem solving style values may (or may not) have been impacted by violations and applications of Amershi et al.'s guidelines using the GenderMag problem solving style survey.
To the best of our knowledge, this was the first attempt to study the user experience of such cognitively diverse users with such guidelines, seeking to uncover additional information such as:
1) when the guidelines were violated, were such violations \textit{worse} for some users than for others, and
2) when the guidelines were applied, were such applications \textit{better} for some users more than others.



\boldify{First, we needed to make sure everyone had paid attention. From the 1043 participants that Li et al. analyzed from the 16 successful experiments, 27 failed at least one of the 3 checks in the GenderMag survey, giving us 1016 participants. Let's talk about them. NOW HIT THEM OVER THE HEAD WITH SELF-IDENTIFIED GENDER AGAIN.  }


Of the 1,043 participants who passed the experimental attention checks, 27 participants did not pass an attention check in the GenderMag problem solving style survey, leaving a total of 1,016 participants.
They came from all walks of life, from different ages (18---74), educational backgrounds (less than high school to Masters or higher), occupations, and the gender identity/identities they reported to us (Appendix~{\color{blue}~\href{https://web.engr.oregonstate.edu/~anderan2/MSR-Appendices/Appendix-Demographics.pdf}{C}}).

%\input{tables/17-Demographics}


% \FIXME{478 men, 527 women, 12 non-binary, 2 gender-non-conforming, 4 transgendered, 1 intersex, 2 prefer not to answer\\
% \\
% % 125 $\in$ 18 - 24 years old, 422 $\in$ 25 - 34 years old, 259 $\in$ 35 - 44 years old, 138 $\in$ 45 - 54  years old, 58 $\in$ 55 - 64 years old, 14 $\in$ 65 - 74 years old\\
% % \\
% % 5 less than high school, 86 graduated high school, 22 trade/technical school, 199 some college-no degree, 112 associate degrees, 430 bachelors degree, 162 advanced degrees.\\
% % \\
% % 3 unable to work, 6 unemployed and not looking, 12 retired, 26 unemployed and looking, 31 homemakers, 60 students, 106 self-employed, 115 part-time workers ($\leq 39$ hours/week), 657 employed ($> 39$ hours/week)
% }


\subsubsection{Computing Participants' problem solving styles}
\label{sec:get-facets}

\boldify{In the facet survey, different questions relate to different problem solving styles, and here are some examples. Participants had the option to say ``idk''.}

Participants responded to the GenderMag problem solving style survey on 9-point agreement scales for 36 statements, with an option to reply with ``\textit{I don't know}'' if needed.
%
%Each question uncovered information about one of the 5 problem solving styles in Table~\ref{table:personas}.
%For example, people who strongly agree with the statement ``I avoid using new apps or technology before they are well-tested'' are likely to be \colorboxBackgroundForegroundText{AbiOrange}{black}{risk-averse}, relative to their \colorboxBackgroundForegroundText{TimBlue}{black}{risk-tolerant} peers who heavily disagrees with it.
%Further, people who agree with the statement ``My first step in learning new technology is experimenting and tinkering with it'' are likely to have a \colorboxBackgroundForegroundText{TimBlue}{black}{tinkering-oriented} learning style, as opposed to their \colorboxBackgroundForegroundText{AbiOrange}{black}{process-oriented} counterparts.
%
%\input{figure/01-Gender-Insight/04-GM-Scores}






%\input{tables/6-GM-Rules}






%
There are five subsets that partition the 36 survey statements, one subset for each of the five problem solving style types.
We computed participants' problem solving style values twice, once relative to their participant peers in the same experiment (analyzed in Section~\ref{sec:Results-Insights}) and the other relative to participants across \textit{all} experiments (analyzed in Section~\ref{sec:gender}).
To compute participants' problem solving style values for each problem solving style type, we summed up the responses to the questions %(q) 
that were not ``\textit{I don't know}'' to create a score for that problem solving style type.
To account for the ``\textit{I don't know}'' responses, we adjusted each participants' score by dividing it by the percentage of responses they answered.
% the questions they had actually answered for that style.

To illustrate the need for such a correction method, consider that there are seven questions for attitudes toward risk. 
Suppose Participant X answered four of them with ``I don't know'',
but they answered with ``9'' for the other three questions.
This would sum to a ``risk score'' of 27.
Now suppose that Participant Y answered all seven questions with ``4's'', so Participant Y's score would have a score of 28.
Without adjustment, this would create a possibility of both participants being classified as having the same attitude towards risk, despite the average of their answered questions being completely different (9 vs. 4).
Our correction technique took each participants' score (Participant X: 27) and divide it by the percentage of questions they answered (Participant X: 0.429).
Therefore, their adjusted score for attitudes toward risk was $\frac{27}{0.429} \approx 63$.
%Begin FIXED
\FIXED{
In keeping with precedent~\cite{hilderbrand2020engineering,guizani2022debug,kanij2022new}, participants' scores were classified relative to the median of each distribution after the adjustment.
%End FIXED
}
For attitudes toward risk, those who were above the median were categorized as more \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} than their \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} peers whose scores were below the median\footnote{
The classification rules for all five problem solving style types can be found in Appendix{\color{blue}~\href{https://web.engr.oregonstate.edu/~anderan2/MSR-Appendices/Appendix-Facet-Survey-Rules.pdf}{A}}.}.
Specifically to attitudes toward risk, using the median as the classification threshold enables researchers to derive actionable insights, because users can be classified as ``more'' or ``less'' risk-averse than others.

% For example, if participant X answered three of the five Attitudes Toward Risk questions with ``I don't know'', but the sum of the other two questions created a ``score'' of 10, then their score for this problem solving style became 10/0.6 = 16.67.
% To analyze Section~\ref{sec:Results-Insights}, we used the medians in each experiment for each of the five distributions to classify which side of each cognitive spectrum a participant was on relative to their peers in the experiment (Table~\ref{table:personas}).
% To analyze Section~\ref{sec:gender}, we used the grand median across all participants to classify each individual.
%
%\boldify{Here's how we decide who is which style.}
%
%Thus, for each of the 16 independent experiments, participant scores formed 5 different distributions, one for each of the 5 problem solving styles.
%Then, just as Burnett et al. \& Vorvoreanu et al. did~\cite{burnett2016gendermag,vorvoreanu2019gender}, we leveraged the median to decide which participants' scores reflected which problem solving style, and the rules for each problem solving style are reflected in Table~\ref{tab:style_rules}.
%Begin FIXED
\FIXED{
\subsubsection{Statistical Testing Paradigm}
\label{sec:testing-paradigm}



\boldify{Here is our testing paradigm, aimed to reduce the number of tests we ran and to maximize the chances of success.}

Each of the 16 independent experiments had its own pool of data, and we analyzed each independently of the other 15 experiments.
Within each experiment, after plotting the data, we measured the distance between the means of each dependent variable for both the \vioProduct{} and \appProduct{}, and we ran a test if that distance was greater than 0.5.
We validated the t-test's assumption of equal variance by using Levene's test, to decide whether Student's t-test (i.e., Levene's test $p \geq .05$) or Welch's t-test (i.e., Levene's test $p < .05$) was more applicable.
We did not draw inferences from ``marginally significant'' results (i.e., $.05 \leq p < .1$), but we count having ran these tests for correction purposes, and we applied Bonferroni correction for the \appProduct{} or \vioProduct{} separately in each experiment by multiplying each p-value by the number of tests run on that product, in the interest of transparency.
%End FIXED
}
%We used Student's t-test whenever the assumption of equal variance was met (i.e., Levene's test: $p > .05$) and explicitly state when we use Welch's t-test.
%When we instead needed to use a paired t-test or Welch's t-test we state the test explicitly.




%\input{figure/2-Testing-Paradigm}



\FIXME{THE BELOW WAS A CONVERSATION THAT PEGGY AND I HAD}


EQUITY is BETWEEN risk-averse vs risk-tolerant.  So you can't say things like line 93

That's what I had wanted to talk to you about. Cohen's d in the vioProduct does measure the gap between risk-averse and risk-tolerant (same with appProduct).
I'm positing that to measure HOW MUCH the equity gap changed, we can take the ratio between these two numbers. It's a similar concept to the odds ratio that we use to show how much more/les slikely someone was to do something.

Sure, sounds reasonable.  But you still can't word EQUITY things like line 93.  It makes no sense to say "equity gap did reduce for the risk-averse participants".  It only makes sense to say "equity gap did reduce BETWEEN risk-averse and risk-tolerant participants"

However, if you were talking about INCLUSIVITY instead, your wording such as on line 93 would be perfect.
EQUITY is BETWEEN.  INCLUSIVITY is WITHIN.



I'm with you now. Need to have both of them in the sentence, rather than just say the one. Yeah, that's why we have the paired t-test for inclusiveness (inclusivity?inclusion? I need to pick one), and the two-sample t-tests are for equity. Good catch, and I'll adapt. I'm still wrapping my head around all this.

k.  Ready to move forward again?  All answered for now?


Everything answered, ready to onward and upward. Until I see you tomorrow at least.

ok.  BTW, for the next couple of weeks, I have only boring things on my plate.  If you want to entice me into doing something substantive on this paper, tomorrow would be an excellent day to do so.


lovely. I'll try to write enticingly then.


\subsection{User Experience Equity by Attitudes Toward Risk Across 16 Experiments
\draftStatus{MMB thinks...?}} 
\label{subsec:equity-risk}

\FIXME{AAA - THis goes somewhere here

\boldify{What about the change in equity? Well we do see that the equity gap narrowed, but we propose that one way to measure equity is through the ratio of Cohen's d}

There were two differences of note between the \vioProduct{} and the \appProduct{} products.
First, the risk-averse participants still felt significantly less in control of the \appProduct{} (t(61) = -2.0149, p = .048, d = .508) than their risk-tolerant peers, suggesting that the equity gap remained between these two products.
However, the second difference to notice is that this equity gap between the risk-averse and risk-tolerant (i.e., the distance between the averages in both products) \textit{reduced}.
One way to  measure this change is to use the ratio of the measures of practical significance\footnote{Practical significance refers to the effect size. 
Results are practically significant when the difference is large enough to be meaningful in a real life context.~\cite{ramsey2012statistical}.}.
In this instance, consider the ratio of the effect sizes between these two products (i.e., $\frac{\appProduct{}}{\vioProduct{}}$), which would be 0.508/0.644 in this instance.
The result (0.789) is a number less than one, demonstrating that the equity gap reduced between the risk-averse and risk-tolerant participants.
This suggests that although applying Guideline 11 was inclusively beneficial, more work remains to understand how to do so in such a way that further improves equity.
}

\FIXME{C - Improved inclusivity and equity

V - Improved inclusivity but not equity

P - As inclusive and equitable to vio/apply

Report on equity and inclusion, have Elizabeth help me with classifying these}




\subsubsection{Pattern \#1: Applying Guidelines Improved Inclusivity \& Equity}
\label{subsec:category-1}






Stuff from the related works about OCEAN and propensity to stereotype. These don't have anything to do with problem-solving.

% \boldify{...and other works do not tie in at all to the GenderMag facets, and here's some and what they found.
% }

% Other researchers have considered  problem-solving styles that are unrelated to  within the context of artificial intelligence in how diverse people used AI systems.
% For example, Millecamp et al.~\cite{millecamp2020s} considered participants' OCEAN%
% \footnote{OCEAN: \underline{O}penness, \underline{C}onscientiousness, \underline{E}xtraversion, \underline{A}greeableness, \underline{N}euroticism}
% personality traits~\cite{goldberg1990alternative} to investigate whether differences in personalities impact end users' use of AI music recommender systems.
% % In their experiment, they presented participants with two interfaces in a within-subjects design;
% % one of the interfaces had explanations for why the system was recommending a song (e.g., based on the song's danceability, energy, popularity, tempo, etc.), and the other interface did not have an explanation.
% Their results suggested that personality dimensions like participants' Openness could govern whether the participant had an intention to interact with the interface again or not.
% Additionalyl, Giboney et al. considered how propensity to stereotype related to perceived quality of the AI system~\cite{giboney2015user}.
% % For example, Giboney et al.~\cite{giboney2015user} investigated how people's propensities to stereotype aligned with explanations of expert systems.
% % They found that the more that participants’ propensity to stereotype aligned with an explanation’s presentation, the higher the perceived quality of the system.
% % Jiang et al. considered participants’ self-confidence and found that the greater the participants’ self-confidence, the less likely they were to accept the expert system’s proposed solution. 
% %Other researchers in the human-AI space have also started using the term ``problem solving style'' to try and understand human behavior in the human-AI interaction.
% %Felmingham et al.~\cite{felmingham2021importance} hypothesized that one possible explanation for why clinicians interacting with an intelligent algorithm may change their mind may be in part explained by their responses to the Cognitive Reflection Test (CRT) and the Rational-Experiential Inventory (REI).

==> doc/zz-04-Results-aOLD-Inclusivity.tex <==
\section{Results: What participants' problem-solving styles revealed \draftStatus{top is MMB2.4}
}
\label{sec:Results-Insights}

\FIXME{MMB: this was the version of 8/4/23 at noon}

\FIXME{AE-18, AE-20, R4-9, R5-5, R6-26, R6-27}

%\FIXME{MMB for global todo: throughout, I keep changing "that" statements to "whether" statements.  Our investigation is to show WHETHER unfairness exists, not THAT unfairness exists. WHETHER is a research paper; THAT is a soapbox/position paper\\
%update: added to the global TODO's list}

%\FIXME{MMB for global todo: \\
%(1) in results, never use the word "user" or "end user" -- the results are about what the PARICIPANTS did, not what USERS did. \\
%(2) throughout paper, never claim that our participants are/were end users unless you specifically substantiate that claim (eg, in methodology the filters used to recruit them, or by the virtue of the fact that they never see anything except the output so its an end-user perspective. For this, I think it's easier to just say "users" when we're not talking specifically about our participants, since it's not important to us whether they're "end users" or not.\\
%update: added to the global TODO's list}


\boldify{We're going to investigate HAI-UX inclusivity and equity, starting with inclusivity}

We investigate two types human-AI user experience (HAI-UX) unfairness in the context of these AI products: HAI-UX inclusivity and HAI-UX equity.
\textbf{RQ1-Risk} considers whether these kinds of HAI-UX unfairness arise for diverse problem-solvers, where the diversity lies in their different attitudes toward risk.   


%-----------------------------------------------
\subsection{Inclusivity, for risk-diverse problem solvers\draftStatus{top=D2.8}}
\label{subsec:inclusivity-risk}

%\FIXME{
%categories are:\\
%No improvement for either (1) \\
%Improvement for Abi ONLY (2) \\
%Improvement for Tim ONLY (3) \\
%Improvement for Both (4) \\
%(1) happened 44 times \\
%(2) happened 13 times \\
%(3) happened 28 times \\
%(4) happened 75 times
%}



We begin our RQ1-Risk investigation with risk-diverse participants' HAI-UX inclusivity outcomes.
As pointed out in the Introduction, conceptually, inclusivity in HAI-UX means providing every group of people with a high-quality user experience. 

\boldify{We measured inclusivity change as follows.}
In this paper, we measure whether/how applying a guideline to an AI product \textit{changed} the product's inclusivity toward some particular group of participants.
For any user experience dependent variable in an AI product, we will say the HAI-UX is \textit{more (less) inclusive to a group of participants if the Application AI product's result for that variable are significantly higher (lower) than the  Violation AI product's for those participants.}
Recall that, because this inclusivity measure is within-subject, we used paired t-tests to measure HAI-UX in the before (\vioProduct{}) vs. after (\appProduct{}) versions of the AI products.


\boldify{The outcomes could go any of the following 4 ways, and they did (see table). And in every case it was an improvement or neutral, never negative.}
HAI-UX inclusivity could change in only four possible ways: 
(1)~inclusivity changes for both the risk-averse and risk-tolerant participants, 
(2)~inclusivity changes for neither of them, 
(3)~inclusivity changes for the risk-averse only, and 
(4)~inclusivity changes for the risk-tolerant only.
As Table~\ref{tab:Risk-Inclusivity-Frequency} shows, instances of all of these categories occurred.
This table summary reveals our first result: whenever a change in inclusivity occurred, it was a positive change, improving inclusivity for at least some risk-attitude participant group of participants without harming others.
There were no statistically significant negative changes to inclusivity.

\colorbox{red}{MMB: DO NOT ADD ANY WORDS after here}

\input{tables/04-Inclusivity-Frequency-Table}

\FIXME{MMB@AAA: notice: our 1st result is here. (I'm going to try to point all of these out, so that you can find them all later.\\
}
%----------
%END HERE -- above line is our sunset to this section. DO NOT ADD anything after it.

%We define our measure of inclusivity in the following way:
%``\textit{A user experience between two AI products is inclusive if there is a paired, statistically significant difference between participants' average response for the two products.}''
%
%\FIXME{MMB@AAA: **the above defn isn't correct. We aren't measuring the final inclusivity state, we're measuring CHANGE in inclusivity.  But I defined it correctly above, so commented it out here.}







%---------
\subsubsection{Inclusivity changes for both the risk-averse and the risk-tolerant\draftStatus{MMB:2? down to 6-example table, then needs a different example}}
\label{subsubsec:both-inclusivity}

\boldify{This category happened a lot. }

As Table~\ref{tab:Risk-Inclusivity-Frequency} showed, 
applying the guidelines improved HAI-UX experiences of both the risk-averse and the risk-tolerant 75 times.
These outcomes occurred in 12 of the 16 experiments. 
%In every case, the \appProduct{} was the AI product with the higher inclusivity; thus these inclusivity changes were always inclusivity improvements. %MMB: don't need this, we've already said it twice above.
For some experiments, the inclusivity results by risk largely mirror Investigation One's overall results---G6 is a case in point.
However, in other experiments, they reveal which attitudes toward risk need much more support, as we will discuss in upcoming sections.


\boldify{What does an inclusivity improvement look like? let's look at an example...} 
For a close-up view of what an inclusivity improvement looks like in these data, we begin with a small example: 
a \textit{single} dependent variable from a \textit{single} guideline experiment  (Table~\ref{fig:G8-inclusivity-illustrative-example}).
The dependent variable was participants' responses to ``I would not be suspicious''
and the experimental setting was the Guideline~8 experiment.%
%     start ftnote
\footnote{Appendix~{\color{blue}\href{https://web.engr.oregonstate.edu/~anderan2/MSR-Appendices/Appendix-Boxplots.pdf}{D}} provides boxplots of results for \textit{all} dependent variables in \textit{all} guidelines. 
}        %end ftnote

In this experiment, the AI-powered feature was a design helper to automatically provide design suggestions for alternative layouts in a presentation application.
In the \vioProduct{}'s vignette, the feature's behavior was:
\textit{``You are working on a slide and Design Helper pops up, showing you some design suggestions. You do not need any design help at this time, but there is no way to hide the design suggestions.''} 
In contrast, the \appProduct{}'s vignette started out the same, but its last sentence was: \textit{``You do not need any design help at this time, so you click on a button visible on screen to hide the design suggestions.''}

The \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} participants, shown in Table~\ref{fig:G8-inclusivity-illustrative-example}'s \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{left hatched boxplot}, were fairly evenly dispersed above and below neutral in their suspicions of the \vioProduct{}, but the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{same participants} were significantly less suspicious%
\footnote{Recall from Table~\ref{table:step1-dependent_variables} that the ``suspicious'' dependent variable was on of the variables that reverse-coded for presentation clarity, so that more positive outcomes were always higher on the scales.} %end ftnote
with the \appProduct{}, as shown in the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{left clear boxplot}
\tTestResult{25}{3.2354}{.003}{.648}.
The \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants also were significantly less suspicious of the \appProduct{} \tTestResult{34}{3.0020}{.005}{.507}, as shown in the \colorboxBackgroundForegroundText{TimBlueQuote}{black}{right boxplots}.

\input{tables/03-Inclusivity-Risk-Walkthrough}
\input{tables/04-Inclusivity-Improved-Both}



Table~\ref{tab:inclusivity-change-both} provides additional examples in this category, selected to give an idea the category's broad span. 
The 75 instances of this category spanned all %10 DVs
dependent variables, each of which measures a different aspect of HAI-UX.%, and in 12 of the 16 experiments.


\FIXME{MMB: above parag and table seem unneeded now?  should we skip entirely, or save some words somehow, or reduce table, or ...??? }

\boldify{where did these risk-related inclusivity gains come from? Let's look at G13.}

\FIXME{MMB: Sigh, now that I look at the table of results, I can see that G13 is not a good choice for this section.  It needs either something in G6-G11 or in G14-G17.}

**MMB says: here are some useful Abi quotes from G10:
G10-583-risk-averse: I prefer to be prompted to clarify the word rather than have it assumed potentially incorrectly from what I'm intending.
G10-593-risk-averse: I would be afraid with Kelso that i would miss the incorrect words that were auto corrected and with Ione i have more control by picking from a list of options.
G10-647-risk-averse: Sometimes the auto-correct is really annoying, and fixing it might take multiple attempts.

and some useful Tim quotes from G10:

G10-2408-risk-tolerant: I mistype things a LOT! I would wind up going back to correct Kelso all the time, pretty much making that application useless. Unless it has machine learning and will start to make the changes based on your history, I can't see how this would be useful for anyone.

G10-1969-risk-tolerant: I like having a choice of similar words in case the word the program chooses isn't correct

G10-1916-risk-tolerant: MS Word my spelling/grammar checker of preference gives me the options like Kelso so I am use to such a system already.

G10-1926-risk-tolerant: I'd rather be able to chose from a list so that i had more options.  If you use Ione chances are you would have at least some wrong words because of the auto replacement.

G10-1524-risk-tolerant: I would prefer the speed of which I can click on the word to avoid having to type the whole word myself. Ione would confuse me and make me sad.

To understand how these inclusivity gains worked for participants with different attitudes toward risk, consider Guideline 13 (Table~\ref{tab:inclusivity-change-both}).
Guideline 13's \vioProduct{} vignette explained that \textit{...You usually pick designs that feature the color blue. After using [Violation AI product] a few times, you notice it has not learned your preferences, and blue designs appear in the same place among the suggested designs as the first time you used it.}
In contrast, in the \appProduct{}, \textit{``...You usually pick designs that feature the color blue. After using [Application AI product] a few times, you notice it has learned your preferences and not features blue designs prominently.''}.

\boldify{Participants' reasoning often had to do with their risk attitude.}
Participants' reasons for rating the \appProduct{} higher than the \vioProduct{} varied according their attitude toward risk.  
The risk facet is nuanced---it includes not only aversion/tolerance of privacy/security risks, but also of producing inadequate work, of wasting time on trivial details, and of having trouble with the product. 
Participants' comments included all of these types of risk.
For example, 39\% (11/28) of this experiment's risk-averse participants appreciated the \appProduct{} because of less wasted time, less trouble, less unpredictability, such as:

%------quote template:
%\quotateInset{**desired quote**.}
%{}
%{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{**id**}}
%{Whole quote - **whole quote.}
%-------end quote template

\quotateInset{The more familiarity with a product [possibly referring to the stable placement of the blue designs], the better...}
{}
{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G13-1364-risk-averse **wrong PID**}}
{Whole quote - The more familiarity with a product, the better it usually is.}

%\quotateInset{It learned my preferences quicker which in time will save me time and trouble.}
%{}
%{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G13-959-risk-averse}}
%{Whole quote - It learned my preferences quicker which in time will save me time and trouble.}

\quotateInset{With [\vioProduct{}], I will have to scroll down to pick my preference each time...}
%{}
{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G13-153-risk-averse**wrong PID**}}
{Whole quote - With Kelso, I will have to scroll down to pick my preference each time (if I pick any).  With Ione, I might save some time.}

%G13-1177-risk-averse: I feel that if I favor something enough for it to be recognized then I would prefer for that to be most prominent in my choices. That way I do not have to make specific choices for everything as some things will already be done for me. 


\quotateInset{It would be nice for the program to take my preferences to use as default so that I don't have to search for the color and design I want every time.}
{}
{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G13-2212-risk-averse**wrong PID**}}
{Whole quote - It would be nice for the program to take my preferences to use as default so that I don't have to search for the color and design I want every time.}

Of course, some (29\%) of the risk-tolerant participants liked time-savings as well.
Still, 45\% of their comments expressed a risk-tolerant interest in applying more automation or automating in ways they had not experienced before:

\quotateInset{... [\appProduct{}] learns my needs and preferences, this is pretty crucial in this kind of application...}
{}
{\colorboxBackgroundForegroundText{TimBlueQuote}{black}{G13-1005-risk-tolerant**wrong PID**}}
{Whole quote - I like that Kelso learns my needs and preferences, this is pretty crucial in this kind of application for me}

\quotateInset{I would be interested to see what a program can learn about me... and what the quality of those suggestions would be.}
{}{\colorboxBackgroundForegroundText{TimBlueQuote}{black}
{G13-1085-risk-tolerant**wrong PID**}}
{Whole quote - I would be interested to see what a program can learn about me, from my own input and behaviors, and what the quality of those suggestions would be.}

\quotateInset{I like how it learns my preferences and auto applies them.}
{}
{\colorboxBackgroundForegroundText{TimBlueQuote}{black}{G13-751-risk-tolerant**wrong PID**}}
{Whole quote - I like how it learns my preferences and auto applies them.}






%-----------
\subsubsection{Inclusivity improvements for neither the risk-averse nor the risk-tolerant \draftStatus{MMB: d1.5}}
\label{subsubsec:none-inclusivity}
\boldify{The second-most prevalent category was where nobody's inclusivity got better.}

However, not all the results were as positive for diversity. %MMB to AAA: I reverted this sentence, please keep as is.  (Relax, Mickey will be fine with it.)
Some changes did not change inclusivity outcomes for either of the two groups, defined in this paper as  no significant difference in HAI-UX inclusivity for either the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} or the \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants between the \vioProduct{} and \appProduct{}.
This was the second-most prevalent category, occurring 44 times across 10 experiments.
% Thus, neither the risk-averse nor risk-tolerant participants had significantly different experiences between the \vioProduct{} and the \appProduct{}.

\boldify{For example...}
Table~\ref{tab:no-inclusivity-change-general} shows six examples from this category.
For example, the first two rows are both from Guideline 1's experiment.
The AI-powered feature in that experiment was a capability called Presenter Coach to help participants practice and improve their presentations.
The \vioProduct{} violated the guideline by providing vague information about Presenter Coach's capabilities: \textit{``We will help you improve your presentation style.''}
In contrast, the \appProduct{} provided more detailed information about Presented Coach's capabilities: \textit{``As you practice your presentation, we will give you feedback about your presentation style: how fast you speak, use of filler words (such as `um' and `like'), use of inappropriate words (such as `damn').''}
As the table shows, the way Guideline 1 was applied in this \appProduct{}made no significant difference to either the risk-averse or the risk-tolerant participants---and this was the case for almost all of Guideline 1's dependent variables.


\input{tables/04-Inclusivity-No-Change-General}


%\FIXME{MMB@AAA: To here it's D1.5ish, but at this point it deviates from our paper's meta-story and never comes back. (See the AUDIT in the todo list.) By this I mean, it does the comparisons, but then talks about some other undefined HAI-UX response change and a bunch more comparisons and quotes, but much of it seems to contradict our meta-story. The bottom line seems to be that looking at risk doesn't help our understanding at all.\\
%FIX idea \#1: If we don't really have anything to say except that it happened a lot, maybe we just drastically shorten this subsection to say only that (with a table of some results).\\
%FIX idea \#2: We do have something, that participants with diverse attitudes toward risk preferred the \appProduct{} but for entirely different reasons! It enhances our understanding of \textit{why} they preferred it, even when we don't find anything in their HAI-UX inclusivity.}


\input{tables/04-G4-Inclusivity-No-Change}


\boldify{But why? Well, turns out participants with both attitudes toward risk had privacy and security concerns from a different data source}

% \FIXME{AAA - Put something like ``we were surprised'' and never say ``surprisingly''. The first is a reflection on how we felt and doesn't assume how the reviewer should feel. 

% I'm also starting to think that we should END this part with G4. We need to talk about the overwhelming majorities preferring the appProducts, and that sets up the surprise for Guideline 4. Yes, this is the way.}

When participants selected that they preferred the \vioProduct{}, their explanation for why they preferred it provided a possible explanation for this HAI-UX inclusivity phenomenon.
For example, sometimes both the risk-averse and risk-tolerant participants had shared concerns about the \appProduct{}, such as privacy/security concerns:

\quotateInset{I would prefer to use [\vioProduct{}] because [\appProduct{}] feels a bit more intrusive. I would be nervous that [it] is pulling data from things like my other software and my browsing history.}
{}
{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G4-3905-risk-averse**chkPID**}}
{Whole quote - I would prefer to use Ione because Kelso feels a bit more intrusive. I would be nervous that it is pulling data from things like my other software and my browsing history. This would be unacceptable since I work with sensitive PII.}

% \quotateInset{I feel more secure with my information using [\vioProduct{}].}
% {}
% {\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G4-4045-risk-averse**chkPID**}}
% {Whole quote - I feel more secure with my information using Kelso.}

% \quotateInset{Whenever possible, I try to avoid giving more apps and services permission to access and use my data, and I assume [\appProduct{}] would need that permission in order to provide its service. }
% {}
% {\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G4-3931-risk-averse**chkPID**}}
% {Whole quote - Whenever possible, I try to avoid giving more apps and services permission to access and use my data, and I assume Ione would need that permission in order to provide its service. }




\quotateInset{I don't like the idea of [\appProduct{}] taking definitions from my workplace. 
It makes me worry I'm being listened to, or that my network is being monitored, etc.}
{}
{\colorboxBackgroundForegroundText{TimBlueQuote}{black}{G4-3947-risk-tolerant**chkPID**}}
{Whole quote -I don't like the idea of Ione taking definitions from my workplace. 
It makes me worry I'm being listened to, or that my network is being monitored, etc.}

\boldify{Risk-averse participants also had smatterings of concerns that tie with attitudes toward risk, such as how easily mistakes could be identified (over-reliance?) or having control of the system. }

However, the risk-averse participants also raised other concerns that the risk-tolerant did not, such as how easily they may be able to identify mistakes...

\quotateInset{[\vioProduct{}] may make mistakes in context,  but its use of a generic dictionary makes it easier to recognize mistakes,  I'll know that it isn't identifying workplace-specific acronyms.  With [\appProduct{}],  I would be more likely to miss mistakes.}
{}
{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G4-3936-risk-averse**chkPID**}}
{Whole quote -Kelso may make mistakes in context,  but its use of a generic dictionary makes it easier to recognize mistakes,  I'll know that it isn't identifying workplace-specific acronyms.  With Ione,  I would be more likely to miss mistakes.  }

...or that when mistakes may occur, some of the risk-averse participants stated that they would prefer the \vioProduct{} because they would have more control over the system's output:

\quotateInset{[\appProduct{}] would be easier but if [it] were to make a mistake on me, I would have a hard time trusting it because I did not make any part of the decision.}{}{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G4-3799-risk-averse**chkPID**}}{I would rather use Kelso because Kelso gives me the choice of choosing which definition I would want to go by. Ione would be easier but if Ione were to make a mistake on me, I would have a hard time trusting it because I did not make any part of the decision.}

\quotateInset{With [\vioProduct{}], I can rely on my own expertise to choose the correct acronym definition.  I feel I have more control/responsibility with [\vioProduct{}].}{}{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G4-3799-risk-averse**chkPID**}}{Whole quote - With Ione, I can rely on my own expertise to choose the correct acronym definition.  So if there is a mistake, it would be me making the mistake, not Ione.  I feel I have more control/responsibility with Ione.  With Kelso, if I relied on it too much and it make a mistake, of course I would be the one held responsible, not the document program.  I would feel safer relying on my own expertise and using Ione. }

\boldify{What does this all mean for the HAI community? Well primarily that we should definitely be considering \textit{how} to apply these guidelines.}



For the HAI community, these findings suggest that considering participants' quantitative and qualitative responses through the lens of their diverse attitudes toward risk can provide additional insights behind something seemingly uninteresting (i.e., no change in HAI-UX inclusivity).
Additionally, for Guideline 4, these findings suggests that in order to adequately meet the needs of such diverse people, the community should consider carefully \textit{how} to apply these guidelines.




%-------------
\subsubsection{Inclusivity improvements, but for the risk-averse only \draftstatus{MMB1.5?}}
\label{subsubsec:abi-inclusivity}

\boldify{The third category of HAI-UX inclusivity change was when \textit{only} the risk-averse were helped by the changes in the product, which occurred 13 times in 8 experiments}

The third category of HAI-UX inclusivity change occurred when the change between the \vioProduct{} and \appProduct{} was statistically significant for the risk-averse participants \textit{only}.
%\textit{only} the risk-averse participants were inclusively supported between the \vioProduct{} and \appProduct{}.
%the app product improved inclusivity for the risk-averse participants only.
This category arose 13 times across 8 of the independent experiments, and Table~\ref{**FIXME**} provides some examples of this category.

\boldify{For example, G14 (this one particularly helped the Abi's}
One example was Guideline 14 (top row).
In this experiment, the products were document editing apps, and the AI-powered feature suggested functionality that it thought the user may need next.
The \vioProduct{} automatically changed the entire menu bar at the top based on the functionality it thinks a user needs next.
In contrast, the \appProduct{}'s display changes, which were also based on functionality, affected only a dedicated part of the menu in the top-right, leaving the rest of the menu the same.

The \appProduct{}'s display improvement was well-received by both the risk-averse and the risk-tolerant for five of the dependent variables.
But in addition, it particularly influenced the risk-averse in three more dependent variables: 
their reportings of their own adequacy with the product (**FIXME stats**), their sense of the product's reliability (\tTestResult{30}{3.4366}{0.002}{**FIXME**}), and their trust in the product \tTestResult{29}{2.8499}{.008}{**FIXME**}.

\FIXME{MMB@AAA: before, you wrote only the following (2 DVs), but the new table shows significance in 3 (above parag).  One of them is wrong, please fix. Here's what you wrote before:\\
not only did they find the \appProduct{} significantly more reliable than the had the \vioProduct{} \tTestResult{30}{3.4366}{0.002}{**FIXME**}, but they also felt that they would trust the \appProduct{} significantly more \tTestResult{29}{2.8499}{.008}{**FIXME**}.
}

\boldify{This seemingly small change was a big deal for risk-averse participants, who commented on how they would think the \vioProduct{} was disruptive }

One reason to explain this is that some of \textit{only} the risk-averse participants mentioned how disruptive the \vioProduct{} would be: 

\quotateInset{I feel like [\vioProduct{}] would constantly change the entire menu bar and these changes would be disruptive or distracting to me as I tried to work. Kelso would be less intrusive.}
{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G14-3935-risk-averse**chkPID**}}{}
{Whole quote - I feel like Ione would constantly change the entire menu bar and these changes would be disruptive or distracting to me as I tried to work. Kelso would be less intrusive.}

\quotateInset{I would be worried that I'd get confused or frustrated if [\vioProduct{}] changed too many things too often and I had to look for them each time I needed something.}
{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G14-3978-risk-averse**chkPID**}}{}
{Whole quote - I would find a small change to the menu less disruptive. I would be worried that I'd get confused or frustrated if Ione changed too many things too often and I had to look for them each time I needed something.}

\quotateInset{Changing the entire menu bar [in the \vioProduct{}] continuously would be confusing and distracting.  When only a portion updates [in the Application AI product], you may not be distracted.}
{\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{G14-4029-risk-averse**chkPID**}}{}
{Whole quote - Changing the entire menu bar continuously would be confusing and distracting.  When only a portion updates, you may not be distracted.}

It makes sense why the risk-averse were the only ones who brought this up, because in the literature, people who are more risk-averse while using technology tend to perform technology tasks using familiar features, because the risk-averse find the value they derive from such features more predictable and can gauge how much time using these features will take.
As such, it makes sense why a menu that constantly updates would frustrate someone who is more risk-averse when using technology.


% \FIXME{MMB@AAA: I took "disruptively" out of our description of the vioproduct, because I'd like the participants to tell us that.  ie, I'd like to surprise the reader that this seemingly small/innocuous UI difference could have such an effect, and then have the participants explain why.\\
% So...don't we have any quotes showing that a risk-averse participant thought the vio's changes disruptive/disorienting/etc?
% }



%-------------
\subsubsection{Inclusivity improvements, but for the risk-tolerant only\draftstatus{MMB1.??}}
\label{subsubsec:tim-inclusivity}


\boldify{The last category of HAI-UX inclusivity change was when \textit{only} the risk-tolerant were supported by the changes in the product, which occurred 28 times in 13 experiments.}

The last category was inclusivity changes between the \vioProduct{} and \appProduct{} for the risk-tolerant participants only.
This category arose 28 times across 13 of the independent experiments.
Table~\ref{**FIXME**} provides some examples to demonstrate the range.

\FIXME{MMB: G5 is a bad choice -- it only helped Tim in one DV.  We need G3, G13, or G18 here.}
For example, Guideline 5's product was a document editing app with an AI-powered feature that made suggestions to improve writing style.
In the \vioProduct{}, the product's suggestions were imperative, with language like: \textit{``You made a mistake. Replace with...''}, whereas the \appProduct{} matched relevant social norms via language that was phrased more like a suggestion: \textit{``Consider using...''}
The risk-tolerant participants derived a statistically perceptible HAI-UX inclusivity benefit from this design change;
their feelings of adequacy significantly improved \tTestResult{36}{2.8505}{.007}{**FIXME**} between the \vioProduct{} and \appProduct{}.

\FIXME{***here's G3: previously was in BOTH section, then removed this G3 example because it doesn't seem to add anything new. (If we add it here, need to reword where it's going and then find quotes.)\\
\\
For example, in Guideline 3's experiment (first row of the table), the participants were told that the \vioProduct{} sent email notifications whenever a new email arrived, regardless of what the participants were doing.
However, the participants were told that the \appProduct{} muted  notifications when the participants were busy. 
This change between the two products resulted in the risk-averse participants feeling that the \vioProduct{} would be significantly less reliable than the \appProduct{} would be \tTestResult{29}{2.9844}{.0057}{**FIXME**} would be, and the risk-tolerant participants also felt this way \tTestResult{36}{2.7778}{.0086}{**FIXME**}.\\
**insert quotes here\\
** ***---end of G3 removed }

\FIXME{MMB@AAA: need something more here.  There's a comparison, but readers didn't learn anything.\\  
Idea \#1: (counter to what I usually suggest in the Inclusivity sections): Perhaps there's a quote that helps us figure out why the Abi's DIDN'T improve?\\
Idea \#2: We can pick a different guideline and write about that. Basically everyone said in G5, whether risk-averse or risk-tolerant, turned round and said ``I like being asked/requested, rather than told''. 
We stand a better change of finding a quote from there. \\
Idea \#3: Combine the ABi and Tim sections, so now they're learning that sometimes it was Abi and other times Tim?}


% \boldify{Speculatively, the risk-tolerant may have derived this significant benefit because...}

% \FIXME{AAA@MMB: I have no earthly idea. Nothing is telling me why, not their quotes, their preference selection, or their HAI-UX responses. These are people who are not historically disadvantaged by technology! Grrr}

% \FIXME{MMB@AAA: maybe move the "summary" text below elsewhere, because I have some nice glue at the beginning of 4.2-equity that might work fine with an abrupt ending to 4.1-inclusivity.  See what you think. \\
% AAA@MMB: I like the text you have, and I've moved the summary text to the conclusion. I realised that it actually would work quite well there.}



% \boldify{Another way that HAI-UX inclusivity could change between the \vioProduct{} and \appProduct{} was that it changed for \textit{only} one of the two kinds of participants. What you should notice here is that the \appProduct{} worked well for the risk-averse sometimes and the risk-tolerant in others.}

% For example, in Guideline 1's experiment (Table~\ref{**FIXME**}, top row), the risk-averse participants' average feelings of productivity significantly improved between the \vioProduct{} and the \appProduct{} (t(25) = 2.6093, \textit{p} = .015, \textit{d} = .512).
% However, although the risk-tolerant participants' average feelings of productivity increased, it did not do so in such a way that was statistically perceptible (t(29) = .6679, \textit{p} = .5094, \textit{d} = .122).











==> doc/zz-04-Results-b-Equity.tex <==
%----------------------------------------------
\subsection{Equity between Attitudes toward Risk\draftStatus{**}}
%\subsection{Participants' risk attitudes mattered  \draftStatus{3}{}
\label{subsec:equity-risk}

\boldify{The above section measured CHANGE in inclusivity -- but how much is enough?  For this, we need equity.}

Our measure of inclusivity measured changes, which were usually**FIXME?** improvements, in the inclusivity that risk-diverse groups of participants experienced with these HAI products.
But how much more change is needed to these products---i.e., how much inclusivity is ``enough''?  

\FIXME{MMB@AAA: do you know why it says "usually" above?  Elsewhere we wrote "always".  Perhaps "usually" is a holdover/obsolete? Or did you change it for some reason?\\
AAA@MMB: Not my word; I left your words as-is, I promise. Perhaps you had been waiting to see if anyone moved in a significantly \textit{negative} direction? }

One answer to this question lies with the concept of equity.
For example, suppose risk-averse participants' user experiences are worse than those of risk-tolerant participants with a particular AI product.
For that product, we will say that the product needs enough additional inclusivity progress to bring these two groups of participants to have equitable user experiences by our measures.  

\boldify{To measure equity, we...}
Recall from the Introduction that equity, when applied to AI products, is the quality of all groups' user experiences being of the same quality.  
We can thus measure HAI-UX equity in the following way:
``\textit{The outcomes of participants' responses will be considered equitable if the two groups have no statistically significant difference between the groups' outcomes}''
As such, significant differences in the \vioProduct{} or the \appProduct{} indicate the presence of user experience inequity~
\footnote{Two-sample t-tests used to test differences between diverse participants' averages in the \vioProduct{} and \appProduct{} independently.}. %end ftnote
There were four trends for HAI-UX equity between the two products for participants with diverse attitudes toward risk: 
\begin{enumerate}
    \item both the \vioProduct{} and \appProduct{} were equitable for these two groups.
    \item both the \vioProduct{} and \appProduct{} were \textit{in}equitable for these two groups.
    \item the \vioProduct{} was inequitable, but the \appProduct{} fixed this inequity.
    \item the \vioProduct{} was equitable, but the \appProduct{} was \textit{in}equitable.
\end{enumerate}


\FIXME{AAA@ALL: Up to this point, we have talked about, in order: G8, G4, G14, G5. I don't want to revisit them in Equity section unless ABSOLUTELY necessary}

% Throughout this paper, we begin every discussion  of equity with the \vioProduct{} because although violating a guideline is obviously bad, the research community knows little about whether and how such violations are \textit{equitably} bad and for whom.

\FIXME{Equity 1 - Equity improved (5 times)

Equity 2 - Inequitable in \textit{both} (13 times)

Equity 3 - Equity declined (18 times)

Equity 4 - Equitable in \textit{both} (124 times)}

\boldify{To re-orient you, take a look at Guideline 8's example. Notice that we're now focusing on comparing BETWEEN Abis and Tims for each product individually. We'll briefly discuss the most frequent of the four categories, where both the \vioProduct{} and the \appProduct{} were equitable (PUNT to Discussion).}

Table~\ref{tab:equity-no-change-example} illustrates how HAI practitioners can leverage participants' attitudes toward risk to uncover insights about the equity between AI products.


\subsubsection{Both products equitable}

The first of the four HAI-UX equity categories for participants with diverse attitudes toward risk was defined by \textit{no} statistically significant difference between the risk-averse and risk-tolerant participants in either the \vioProduct{} or the \appProduct{}.


% Throughout this paper, we begin every discussion  of equity with the \vioProduct{} because although violating a guideline is obviously bad, the research community knows little about whether and how such violations are \textit{equitably} bad and for whom.

\boldify{Here's the guideline products and AI-features, for context...}

In Guideline 10's experiment, the products were document editing applications, and the AI-powered feature was a spelling assistant that could automatically detect typos.
In the \vioProduct{}, participants were told that the spelling assistant automatically replaced typos, even when there may be other options that made sense too;
in the \appProduct{}, on the other hand, participants were told that the spelling assistant would provide multiple options for the participant to select from.

\boldify{and here's what we found, a big resounding zilch. We'll be punting this to the discussion because we think there are interesting things to discuss between inclusivity and equity.}

The middle column of Table~\ref{tab:equity-no-change-example} shows the risk-averse (top box) and risk-tolerant (bottom box) participants' feelings of certainty with the \vioProduct{}, and there was no statistical difference between their responses \tTestResult{62}{0.8356}{.407}{.209}.
This was also true when these participants saw the \appProduct{} (Table~\ref{fig:G8-illustrative-example}, right), with no statistically significant difference between the two groups' feelings of certainty \tTestResult{63}{0.6264}{.533}{.157}.
In total, this first HAI-UX equity category occurred 124 times across the 16 experiments, and we return to \textit{why} this category may have occurred so frequently in Section~\ref{subsec:equity-inclusiveness-discussion}.

\input{tables/04-Equity-Risk-Walkthrough}


\subsubsection{Neither product was equitable}
\boldify{The second  HAI-UX equity category occurred when there were inequities in both the \vioProduct{} and \appProduct{}. This was the most prevalent category in Guideline 4, so we use that as our example.}

Similarly to Section~\ref{subsec:inclusivity-risk}, investigating human data from HAI experiments by their attitudes toward risk uncovered a category that was not the most positive.
This second HAI-UX equity category occurred 13 times and was defined by a statistically significant HAI-UX equity gap between the risk-averse and risk-tolerant participants in \textit{both} the \vioProduct{} and \appProduct{}.


\input{tables/16-Inequities-Remain}

\boldify{Consider participants' responses to the ``I would feel secure'' DV. Notice that the risk-averse participants felt significantly less secure with the \vioProduct{}? It remained in the \appProduct{}}


Additionally, studying attitudes toward risk helped to uncover \textit{which} of the risk-averse and risk-tolerant participants were disadvantaged by these persistent HAI-UX equity gaps.
For example, \textit{seven} of the instances of this category arose in Guideline 4's experiment (Table~\ref{tab:no-equity-change-G4}).
Recall from Section~\ref{subsubsec:none-inclusivity} that in this experiment, the \vioProduct{} showed only a standard list of possible definitions taken from a popular acronym dictionary, and the \vioProduct{} showed a contextually relevant list from the workplace.
In each of these seven dependent variables, the risk-averse participants were \textit{always} significantly disadvantaged in both products, such as feeling significantly less secure \tTestResult{62}{-2.3006}{.025}{.575} and less adequate \tTestResult{61}{-2.9179}{.005}{.743} than the risk-tolerant peers.
Although the \appProduct{} did provide the workplace definitions, the design changes did not change user experience inequity change;
the risk-averse participants \textit{still} felt significantly less secure \tTestResult{61}{-3.1984}{.002}{.814} and adequate \tTestResult{62}{-2.4955}{.015}{.629} than the risk-tolerant participants.

\boldify{We do note that our measure may not capture some nuances of what it means to ``improve''.
For example, a gap reduction from 0.7 $\rightarrow$ 0.4 \textit{is} improvement, but the statistical tests themselves may just not pick these differences up. We speculatively look at a measurement comparing Cohen's d values (app-Cohen)/(vio-Cohen). This could help us detect these changes.}

We noticed during the course of our analyses that our measurement may not capture nuances in what it meant for participants' HAI-UX equity to ``improve''.
For example, as Figure~\ref{**FIXME**} 
%We're going to need an additional example because G4 is a terrible way to say ``hey things improve'' when they really didn't. In fact, they got worse! Not the message we want to send.
illustrates, participants' feelings of certainty in Guideline 11's experiment followed the definition of this category.
When they saw the \vioProduct{}, the risk-averse participants felt significantly less in control \tTestResult{61}{-2.5538}{.013}{.644} than their risk-tolerant peers, and the \appProduct{} did not resolve this HAI-UX inequity \tTestResult{61}{-2.0149}{.048}{.508}.
Although this fits the definition of the second HAI-UX equity category, it is notable that the distance between the averages did reduce from 0.946 to 0.749, so what can help HAI practitioners gauge improvements?
We draw inspiration from proportions, odds, and odds ratios\footnote{In statistics, proportions ($\hat{\pi}$) are calculated in binarized outcomes by the number of observed ``successes'', divided by the number of observations.
From this, the odds ($\hat{\omega}$) for any group can be calculated to gauge how much more/less likely an event was to occur through $\hat{\omega} = \frac{\hat{\pi}}{1-\hat{\pi}}$.
Between two groups, A \& B, calculating the odds ratio ($\hat{\phi}$) can help determine how much more/less likely one group was to ``succeed'' over another through $\hat{\phi} = \frac{\hat{\omega}_A}{\hat{\omega}_B}$.}%
~\cite{ramsey2012statistical} and speculatively propose leveraging the measures of effect size in a similar way, using the formula $\frac{(Cohen's-d)_{App}}{(Cohen's-d)_{Vio}}$.
A resulting number less than 1 indicates that the effect size for the \vioProduct{} is greater than the effect size for the \appProduct{}---an indication of progress for HAI-UX equity.
In this example, the resulting number is 0.789, which \textit{does} demonstrate that equity improved, even though the statistical tests did not pick this up.

\subsubsection{Inequities in the Violation Product that were resolved by the Application Product}

\boldify{The third HAI-UX equity category occurred when there was inequities in the \vioProduct{}, but that DV was equitable in the \appProduct{}}

A third HAI-UX equity category occurred 5 times across 5 experiments for 5 different dependent variables.
For example, in  Guideline 6's experiment (top row), the products were search engines, being used to search for images of CEOs and doctors.
The participants were told that the \vioProduct{} did not show any images of women or people of color, whereas the \appProduct{} showed images of different types of people in terms of gender and skin tone, including people who looked like the participants.
The lack of representation in the \vioProduct{} caused an inequity in the HAI-UX;
the risk-averse participants felt significantly less adequate \tTestResult{62}{-2.9429}{.005}{.736} than their risk-tolerant peers.
Fitting the definition of this category, the HAI-UX equity gap between these participants with diverse attitudes toward risk no longer existed in the \appProduct{} \tTestResult{62}{-1.0586}{.294}{.265}.
Using the proposed measure of a change in equity, the resulting number is 0.36, suggesting a remarkable improvement in equity.
This HAI-UX equity category demonstrates two things: (1) it highlights for practitioners that violating some of these guidelines are not just bad---violating them are \textit{inequitably} bad for some of those with certain attitudes toward risk (in Guideline 6's case, the risk-averse).
(2) it also highlights the benefits that practitioners derive by applying these guidelines, that such applications are equitably \textit{good} for those with diverse attitudes toward risk

\boldify{Notably, one of these inequities disadvantaged the risk-\textit{tolerant} participants, a rare result but one that cannot be dismissed}

Notably, it was not \textit{always} the risk-averse who were disadvantaged by HAI-UX equity gaps.
For example, the third row of Table~\ref{tab:equity-improved-general} shows results from Guideline 7's experiment.
In this experiment, the products were presentation applications with an AI-powered feature called Design Helper to assist its users with design ideas to add text or images.
The participants were told that the \vioProduct{}, Design Helper had not automatically popped up with design suggestions, and there was no visible button for participants to request suggestions from Design Helper.
The \appProduct{} made such a button visible to request suggestions, which then appear on a side bar.
In this case, the risk-averse felt significantly \textit{more} in control \tTestResult{56}{2.7881}{.007}{.732} than their risk-tolerant peers with the \vioProduct{}, yet the \appProduct{} resolved this HAI-UX equity gap \tTestResult{56}{1.2730}{.208}{.334}
This was the only time this category arose where the HAI-UX equity gap in the \vioProduct{} disadvantaged the risk-tolerant.
With so little data, it remains an open question on what the risk-tolerant may need to close HAI-UX equity gaps between them and the risk-averse when some guidelines are violated.
However, the non-zero amount of times that results like these occurred indicates for the HAI community that the focus cannot be \textit{solely} on the risk-averse participants but rather on considering the needs of both the risk-averse \textit{and} risk-tolerant.

\input{tables/05-Equity-Improved}

%G8, G1, G4, G14, G5, G10, G6

%Options to talk about: G1,  G4, G9, G10, G11, G13, G14, G18


\subsubsection{An equitable Violation Product but an inequitable Application Product}

\boldify{The fourth and last HAI-UX equity category was susprisingly where equity seemed to \textit{decline}. In these cases, the \vioProduct{} contained no evidence of an equity gap, but the \appProduct{} did. This is counter-intuitive because the \appProduct{} is supposed to be the ``gold standard'' for us.}

The last category that studying participants' attitudes toward risk revealed was the most confusing to us, instances where applying the guidelines seemed to \textit{reduce} HAI-UX equity.
For example, Table~\ref{tab:no-equity-declined} highlights the dependent variables from Guideline 18's experiment which exhibited this category.
In this experiment, the products were email applications, and the AI-powered feature could automatically sort email into \textit{important} and \textit{other} categories.
The participants were told that with the \vioProduct{}, they would have to notice that some emails were not making their way into the \textit{important} category, like emails from their boss or from mailing lists.
The \appProduct{} did notify users with a message saying: ``from now on, emails from your boss will always appear in the important category and emails from some mailing lists will no longer appear in the important category.''

\input{tables/04-Equity-Declined}

For example, when participants saw the \vioProduct{}, there was no sign of a HAI-UX equity gap between the risk-averse and risk-tolerant participants' feelings of certainty \tTestResult{65}{-1.7493}{.085}{.428} or productivity \tTestResult{64}{-1.3344}{.187}{.329}.
However, when the participants saw the \appProduct{}, we were surprised to see that the risk-averse participants felt significantly less certain \tTestResult{65}{-2.1207}{.038}{.518} and less productive \tTestResult{64}{-2.2020}{.033}{.5423}.
Our proposed Cohen's d ratio measurement also suggested this;
both of these results were numbers larger than 1, suggesting that the effect size \textit{increased} between the \vioProduct{} and the \appProduct{}.

\boldify{Throughout Sections~\ref{subsec:inclusivity-risk} \&~\ref{subsec:equity-risk}, we empirically showed that considering problem-solving styles can tell us additional information like \textit{how inclusive} applying these guidelines were, along with how equitable they were, and for the most part, it was great}

Sections~\ref{subsec:inclusivity-risk} and~\ref{subsec:equity-risk} provided empirical evidence to support considering participants' diverse problem-solving styles to uncover and understand more about HAI-UX inclusivity and HAI-UX equity when 16 guidelines for human-AI interaction were violated and applied.
These findings suggest that applying these guidelines helped a large number of people with diverse attitudes toward risk, far and away the most prevalent category of HAI-UX inclusivity insight in these data (75/160).


\boldify{The two most prevalent categories in Section~\ref{subsec:equity-risk} were sorta head scratchers, where HAI-UX equity was not significantly different in both the \vioProduct{} and \appProduct{} and where HAI-UX equity seemed to \textit{decrease} by applying the guidelines.}

When it came to HAI-UX equity, we were a little more perplexed by the results.
The most prevalent insight from these data was that both the \vioProduct{} and the \appProduct{} were equitable for these participants with diverse attitudes toward risk.
Additionally, the next-most-prevalent insight arose when HAI-UX equity seemed to decrease between the two products.
One thing we suspect is that a relationship between the HAI-UX inclusivity and HAI-UX equity results can help explain such phenomena, which we turn to next by way of a discussion.

\input{tables/04-Risk-Equity-Frequency-Table}




==> doc/zz-G6_Leftovers.tex <==
\boldify{Guideline 6 provided particularly compelling qualitative data.}
%



% \FIXME{EVERYTHING ABOVE -  Attitude Towards Risk where people are biased against the violation in two ways that isn't personal: (1) they think it doesn't reflect their values, (2) they think it's not accurate, e.g. in real life they work with women/POC CEO's, so the violation isn't accurate in showing just white men. 
% The history of bias in machine learning has been a well-documented theme when the algorithms are making decisions~\cite{mehrabi2019survey}.\\
% EVERYTHING BELOW - How people's PERSONAL identities are biased against, and how they would feel disproportionately impacted.}

\FIXME{Breakup of people questioning Appl Vignette: Total (5) // Preferred Appl -- Abi/Woman (1), Tim/Man (2) // Preferred Violation -- Tim/Woman (1), Tim/Man (1)}

\boldify{However, some people who preferred Application were  suspicious of the way it represented diversity}



\boldify{Additionally, our data suggests that the people who preferred the violation were also suspicious of how diversity was illustrated in the application vignette}




\boldify{Although the people above factored Gender Identity/Race into their opinions about the vignettes, they weren't necessarily directly impacted by these factors. Here are participants who explicitly mentioned how their gender or race/ethnicity would be particularly impacted by the Violation vignette...}

Here are the people who explicitly mentioned how their gender or race/ethnicity would be particularly impacted by the Violation vignette:





%----------------------------------------
\subsubsection{Why the risk-averse and risk-tolerant alike preferred the Application version of G6}

\FIXME{MMB to AAA: Just FYI -- I moved the "why all the risk people liked Application G6" to Leftovers.  Why: it's not at all about risk, and also is specific to G6.  So it's not contributing anything to the plot.}


% G6 quant results reveal: risk averse felt less adequate when guideline was violated
% G6 Scenario: use search engine to search for CEO + doctors. application search results show diverse range of people, violation leaves out POC and women

% \FIXME{RD: Qual differences in G7/G8 are different than G6 -- include in boldify after if needed..}


\boldify{95.3\% of all people in Guideline 6 preferred the Application vignette, and qualitative data from both the risk-tolerant and risk-averse provided compelling evidence about why they preferred the Application vignette.}

In fact, in Guideline 6's experiment (mitigate social biases), the risk-averse and risk-tolerant alike---in fact, almost all of the participants (61 out of 64) preferred the Application.
That experiment's vignette was using a search engine to search for images of CEOs and doctors. 
The Application vignette said that it included diverse people on the first result page, whereas the Violation vignette said that it included no women and no people of color on the first result page.



and participants on both end of the cognitive spectrum tended to have similar reasoning to why they liked the Application vignette, such as it reflecting their personal values towards inclusiveness:



% woman - White/Caucasian/European_Ancestry_(nonHispanic_NonMENA)
\quotateInset{The search results ... [in Application] are more inclusive and represent the values that are important to me...
when it comes to equality and respect. [Violation] encourages negative stereotypes, that women and minorities aren't capable or intelligent enough to be holding these positions and that goes against everything I believe.}
{}{\colorboxBackgroundForegroundText{AbiOrange}{black}{G6-1162-risk-averse}}{
Kelso obviously doesn't think that women and people of color can hold highly-regarded, high-paying, and/or highly-educated positions. The search results I've landed upon on Ione are more inclusive and represent the values that are important to me...the values that are held by (I believe) the majority of people share when it comes to equality and respect. Kelso sounds like it was created by a group of individuals who believe in white supremcy and don't think women are capable of being in these positions. Kelso encourages negative stereotypes, that women and minorities aren't capable or intelligent enough to be holding these positions and that goes against everything I believe.
}

% man - White/Caucasian/European_Ancestry_(nonHispanic_NonMENA)
\quotateInset{A search engine which doesn't show women or people of color seems to have an agenda which I would want no part of.}
{}{\colorboxBackgroundForegroundText{TimBlue}{black}{G6-1236-risk-tolerant}}{
A search engine which doesn't show women or people of color seems to have an agenda which I would want no part of.
}

% woman - White/Caucasian/European_Ancestry_(nonHispanic_NonMENA)
\quotateInset{I prefer to see representation, and it's not like it's female and POC docs and CEOs don't exist. At least Ione promotes realistic diversity.}
{}{\colorboxBackgroundForegroundText{TimBlue}{black}{G6-2651-risk-tolerant}}{
I prefer to see representation, and it's not like it's female and POC docs and CEOs don't exist. At least Ione promotes realistic diversity.
}


\boldify{However, some participants who preferred the application were suspicious of possible biases in the way it represented diversity}

However, some participants who preferred the Application were still suspicious of the vignette's potential to reflect possible biases:

% man - White/Caucasian/European_Ancestry_(nonHispanic_NonMENA)
\quotateInset{I am a little suspicious of [Violation], but maybe [Application] is pushing diverse candidates even if they aren't best for search. I guess I picked [Application] as it seemed sketchy that [Violation] had zero diversity.
}
{}{\colorboxBackgroundForegroundText{TimBlue}{black}{G6-656-risk-tolerant}}{
Maybe there are just a lot of white male CEOs and doctors and I don't know how many results are shown by page. I am a little suspicious of Ione, but maybe Kelso is pushing diverse candidates even if they aren't best for search. I guess I picked Kelso as it seemed sketchy that Ione had zero diversity.
}

% man - White/Caucasian/European_Ancestry_(nonHispanic_NonMENA)
\quotateInset{Even though I cannot confirm that [Violation] is legitimately biased, [Violation] has a negative reputation, and [Application] does not...I would choose the search engine that would not be shrouded in controversy. 
}
{}{\colorboxBackgroundForegroundText{TimBlue}{black}{G6-2546-risk-tolerant}}{
Even though I cannot confirm that Kelso is legitimately biased, Kelso has a negative reputation, and lone does not. If each search engine functions the same otherwise, I would choose the search engine that would not be shrouded in controversy. 
}

% woman - White/Caucasian/European_Ancestry_(nonHispanic_NonMENA)
\quotateInset{The thing is while I am biased towards [Application] and the representation... I understand this itself can be a manipulation if such statistics are not true... I still wouldn't feel in control or completely trust intentions when I do not have more information other than the sheer diversity presented on a single page.
}
{}{\colorboxBackgroundForegroundText{AbiOrange}{black}{G6-493-risk-averse}}{
The thing is while I am biased towards Ione and the representation of a diverse population of leaders, I understand this itself can be a manipulation if such statistics are not true. That is why I answered I still wouldn't feel in control or completely trust intentions when I do not have more information other than the sheer diversity presented on a single page. However, I would personally rather see the diversity than not and would naturally feel more positive.
}

% \FIXME{RD: the "limited results" theme I found here is similar to what we found in the CHI paper - in that study, some participants also recognized that the explanation was incomplete.. }

Broadly, two possible themes arose from the data of participants who preferred the Application: need for explanation and the implications of bias in machine learning. 
% For instance, Participants 656 and 493 mentioned they felt suspicious and not entirely sure about the application's output due to not seeing other information on other pages, suggesting that they think something in the presented information is incomplete, which Kulesza et al. found could impact how people perceive a system~\cite{kulesza2013too,kulesza2015principles}. 
For instance, participants \colorboxBackgroundForegroundText{TimBlue}{black}{G6-656-risk-tolerant } and \colorboxBackgroundForegroundText{TimBlue}{black}{G6-2546-risk-tolerant} both mention suspicions in either how the AI makes its selection (G6-656) or the inability to confirm potential biases (G6-2546),  concerns that might have been addressed through an algorithmic audit, but this method has many barriers, which Rader et al. identified~\cite{rader2018explanations}, and not having formal AI knowledge may raise such barriers higher.
However, the authors also suggest that explanations might be another tool to understand these decisions, which may have allowed these participants to confirm (or refute) their suspicions.

\colorboxBackgroundForegroundText{TimBlue}{black}{G6-656-risk-tolerant}'s last sentence brings into sharp relief the impacts of not addressing potential bias in machine learning~\cite{suresh2019framework}, where this participant deliberately avoided the vignette that had a lack of diversity. 
In fact, even if they could not confirm \textit{why} there were differences between the application and violation vignettes, these participants would ``personally rather see diversity'' or ``would choose the search engine that would not be shrouded in controversy''. 


\boldify{While there were participants who were suspicious of the application, a few participants were actively against the way it represented diversity and preferred the violation.}

As noted above, not everyone preferred the guideline Application vignette.
1 of the 3 participants who preferred the Violation vignette felt that it was the \textit{violation} that mitigated biases:
\quotateInset{I believe the [Violation] search engine mitigates undesirable and unfair stereotypes and biases. Every individual deserves to be treated equally. I understand that we all have preference..., but through [Violation] system, every individual may have the chance to excel better than before.
}
{}{\colorboxBackgroundForegroundText{AbiOrange}{black}{G6-1217-risk-averse}}{
I believe the lone search engine mitigates undesirable and unfair stereotypes and biases. Every individual deserves to be treated equally. I understand that we all have preference in choosing which person we feel we are comfortable to communicate with, but through lone system, every individual may have the chance to excel better than before.
}
The other two participants raised differing viewpoints, where they perceived that the AI was reducing classification of people to their color or genitalia:
% woman - White/Caucasian/European_Ancestry_(nonHispanic_NonMENA)
\quotateInset{Going under the assumption the listings are not racially and sexually generated. I don't want people classified by genitalia and color; I'm seeking professional contacts and not catalog models or actors.
}
{}{\colorboxBackgroundForegroundText{TimBlue}{black}{G6-1939-risk-tolerant}}{
Going under the assumption the listings are not racially and sexually generated. I don't want people classified by genitalia and color; I'm seeking professional contacts and not catalog models or actors.
}
or that the AI was somehow ``forcing'' an agenda of inclusivity because the output did not align with their observations of the world:
% man - White/Caucasian/European_Ancestry_(nonHispanic_NonMENA);East_Asian_(China_Hong_Kong_Japan_Macau_Mongolia_North_Korea_South_KoreaTaiwan)
\quotateInset{Most CEOs and doctors are white males. I feel like the first one is forcing its agenda of being inclusive.
}
{}{\colorboxBackgroundForegroundText{TimBlue}{black}{G6-2796-risk-tolerant}}{
Most CEOs and doctors are white males. I feel like the first one is forcing its agenda of being inclusive
}


However, observations like \colorboxBackgroundForegroundText{TimBlue}{black}{G6-2796-risk-tolerant}'s might not necessarily consider the perspectives of those who identified with the disproportionately impacted communities from the Violation vignette, such as:
% 1903 :: woman - Black/African_American/African_Ancestry
\quotateInset{I am a woman and person of color and would expect differently from [Violation]...these type of situations are reality and based on the past and what America was built on, the fact that acknowledgement of minorities and women are still irrelevant is absolutely crazy.
}
{}{\colorboxBackgroundForegroundText{AbiOrange}{black}{1903-risk-averse}}{
I am a woman and person of color and would expect differently from Kelso.  It is 2019 isn't it, yet these type of situations are reality and based on the past and what America was built on, the fact that acknowledgement of minorities and women are still irrelevant is absolutely crazy.
}

\FIXME{participant number above needs Gnumber}
% whose words suggest that failing to apply these guidelines in the interfaces for human-AI interaction might still have real-world consequences, even if the AI does not make decisions about that person.



==> figure/01-G1/0-F3.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.92\columnwidth]{assets/01-G1/G1-All}
    \caption{\textbf{(A):} Distribution of scores for Guideline 1 participants' F3 --- Feeling Adequate.\\
    \textbf{(B):} The same data, disaggregated by people's self-reported gender; notice how this showed no real difference.\\
    \textbf{(C) \& (D):} The same participants as \textbf{(A)}, but disaggregated by Self-Efficacy \textbf{(C)} and Information-Processing style \textbf{(D)}; notice how the colors (same as Table~\ref{table:personas}) switch position.
    .}
    \label{fig:G1-All}
    % \begin{minipage}[t]{0.67\textwidth}
    %     \centering
    %   % \includegraphics[width=0.92\columnwidth]{assets/01-G1/G1-F3-Swap.pdf}
        
    %     \caption{Distributions for Guideline 1's F3 --- Feeling Adequate --- for the aggregate of participants in (A) and disaggregating by 2 different cognitive dimensions: Self-Efficacy (SE) and Information-Processing (IP) in (B) and (C) respectively.
    %     Notice that disaggregation revealed opposing effects between IP and SE, suggesting the importance of considering multiple facets.}
    %     \label{fig:R-F3-Swap}
    %     \end{minipage}\hfill
    %     \begin{minipage}[t]{0.31\textwidth}
    %     \centering
    %     %\includegraphics[width=.83\columnwidth]{assets/01-G1/G1-Gender.pdf}
        
    %     \caption{The F3 distributions for Guideline 1 under IP (Fig.~\ref{fig:R-F3-Swap}) and gender identity.
    %     Historically used confounding factors (like gender identity) did not yield additional information, but cognitive diversity (like IP) did.}
    %     \label{fig:R-F3-Gender}
    %     \end{minipage}\hfill

    % % \label{fig:overall-precision-recall}
    %         \Description{FIXME} 

\FIXME{MMB: Every figure caption needs to mention which guideline and which dependent variables, and which facets. }

\FIXME{MMB: update this when audits done for this figure (see global TODO for audit type numberings: \\
    Audit1 (status: not done; by: nobody yet\\
    Audit2 (status: not done; by: nobody yet\\
    Audit3 (status: not done; by: nobody yet}

\end{figure}



==> figure/01-G1/1-F3.tex <==
\begin{figure}[h]
    \centering
    \begin{minipage}[t]{0.31\textwidth}
        \centering
        \includegraphics[width=0.92\columnwidth]{assets/01-G1/G1-F3.pdf}
        
        \caption{Distributions for Guideline 1's F3 --- Feeling Adequate --- for 2 different cognitive dimensions: Self-Efficacy (SE) and Information-Processing (IP).
        Notice that disaggregation revealed opposing effects between IP and SE, suggesting the importance of considering multiple facets.}
        \label{fig:R-F3-Swap}
        \end{minipage}\hfill
        \begin{minipage}[t]{0.31\textwidth}
        \centering
        \includegraphics[width=0.745\columnwidth]{assets/01-G1/G1-F3-OtherConfounds.pdf}
        
        \caption{The F3 distributions for Guideline 1 under IP (Fig.~\ref{fig:R-F3-Swap}) and gender identity.
        Historically used confounding factors (like gender identity) did not yield additional information, but cognitive diversity (like IP) did.}
        \label{fig:R-F3-Gender}
        \end{minipage}\hfill
        \begin{minipage}[t]{0.31\textwidth}
        \centering
        \includegraphics[width=0.65\columnwidth]{assets/01-G1/G1-F5.pdf}
        \caption{Distributions for F5 --- Feeling Productive --- for people's attitude towards risk.
        The risk-averse people drove the significance in the aggregate.}
       \label{fig:R-F5}
    \end{minipage}\hfill
    % \label{fig:overall-precision-recall}
            \Description{FIXME} 

\FIXME{MMB: Every single figure caption needs to mention which guideline and which dependent variables, and which facets. }

\FIXME{MMB: update this when audits done for this figure (see global TODO for audit type numberings: \\
    Audit1 (status: not done; by: nobody yet\\
    Audit2 (status: not done; by: nobody yet\\
    Audit3 (status: not done; by: nobody yet}

\end{figure}

==> figure/01-Gender-Insight/02-Age-Distributions.tex <==
% \begin{figure}[b!]
% 	\includegraphics[width = 0.8\linewidth]{assets/02-Results-Gender-Facets/Age-Distributions.pdf}
% 	\caption{ Distributions participants' ages for all 16 experiments.
% 	To what extent does someone's age influence their problem solving styles?
%     }%
% 	\label{fig:Age-Distribution}

% \FIXME{MMB: update this when audits done for this figure (see global TODO for audit type numberings: \\
%     Audit1 (status: )\\
%     Audit2 (status: \\
%     Audit3 (status: }
    
% \end{figure}

\begin{figure}[h]
    \centering

        
        \centering
        \includegraphics[width= 0.65\linewidth]{assets/02-Results-Gender-Facets/Age-Distributions.pdf}
        
        % \caption{New caption here}
        % \label{fig:Age-Distribution}
        
            \Description{FIXME} 
    
    \caption{ The counts of women (orange) and men (blue) for each of the age groups.
    These proportions of women and men in each age group was fairly even, so the differences in Figure~\ref{fig:Age-Facet-Distribution} were not due to one gender's sample size dominating the other.
     }%
     \label{fig:Age-Distribution}

\end{figure}


==> figure/01-Gender-Insight/1-Gender.tex <==
\begin{figure}[h]
	\includegraphics[width = \linewidth]{assets/G4-Gender.pdf}
	\caption{ Distributions of all Guideline 4 participants' scores for the 10 dependent variables, both in the aggregate and disaggregated by people's self-reported gender (legend in the top-left).
	Notice that from a visual scan of the dependent variables, there is no information that tells designers what they should do to show contextually relevant information to better support specific people.
    }%
	\label{fig:Gender-Insights}

\FIXME{MMB: update this when audits done for this figure (see global TODO for audit type numberings: \\
    Audit1 (status: needs to be done\\
    Audit2 (status: needs to be done \\
    Audit3 (status: needs to be done}



% \FIXME{AAA - MV says that Figures~\ref{fig:Risk-G4-All} and~\ref{fig:Risk-G4-Diff} would make a stronger statement if they were one figure geared towards comparison.}

\end{figure}


==> figure/01-Results-1/01-Normal-Disagg.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\columnwidth]{assets/001-Results-1/G1-Disagg.pdf}
    \caption{\textbf{(A):} Distribution of scores for Guideline 1 participants' F3 --- Feeling Adequate.
    \textbf{(B):} Although gender is a diverse spectrum, in this experiment, people reported their gender as either ``man'' or ``woman''.
    These plots show the same data by their self-reported gender; notice how this showed no real difference.\\}
    \label{fig:Normal-Disagg}
    
\FIXME{\st{The 2-gender picture could raise red flags, despite what you say in the text.  Would help to add a caveat to the caption like "(only 2 genders were present in this experiment)"}}
    
\FIXME{MMB: update this when audits done for this figure (see global TODO for audit type numberings: \\
    Audit1 (status: not done; by: nobody yet\\
    Audit2 (status: not done; by: nobody yet\\
    Audit3 (status: not done; by: nobody yet}

\end{figure}



==> figure/01-Results-1/02-Diversity-Disagg.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\columnwidth]{assets/001-Results-1/G1-Diversity-Disagg.pdf}
    \caption{\textbf{(A):} The aggregate distribution from Figure~\ref{fig:Normal-Disagg}.
    However, \textbf{(B)} \& \textbf{(C)} show that disaggregating by diversity dimensions (self-efficacy and information processing style respectively) provide actionable insights on what to do to support people.\\}
    \label{fig:Diverse-Disagg}

\FIXME{MMB: Every figure caption needs to explicitly say (1) which guideline (2) which dependent variables and (3) which facets. (I've also added this to the global todo list)}

\FIXME{MMB: update this when audits done for this figure (see global TODO for audit type numberings: \\
    Audit1 (status: not done; by: nobody yet\\
    Audit2 (status: not done; by: nobody yet\\
    Audit3 (status: not done; by: nobody yet}


\end{figure}



==> figure/01-Results-1/03-G1.tex <==
\begin{figure}[h]
    \centering

        \begin{minipage}[t]{0.43\textwidth}
        \centering
        %\includegraphics[width=0.9\columnwidth]{assets/01-HERE-Insight-1/R-G9.pdf}
        
        \includegraphics[width = 0.4\columnwidth]{assets/05-All-BoxPlots/08-G9/Risk/G9-Feel-Productive-RISK.png}
        \hspace{5mm}
        \includegraphics[width = 0.4\columnwidth]{assets/05-All-BoxPlots/08-G9/Risk/G9-Perceived-Useful-RISK.png}
        
        \caption{Guideline 9 (support efficient correction) -- Participants' scores by attitude toward risk for two dependent variables. 
        The \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants felt significantly more productive and thought the system would be significantly more useful when the guideline was applied.}
        \label{fig:R-G9-F5-PU}
        
        \end{minipage}
        \hspace{5mm}
        \begin{minipage}[t]{0.43\textwidth}
        \centering
        
       % \includegraphics[width=0.92\columnwidth]{assets/01-HERE-Insight-1/R-G10png.pdf}
        \includegraphics[width = 0.4\columnwidth]{assets/05-All-BoxPlots/09-G10/Risk/G10-Perceived-Useful-RISK.png}
        \hspace{5mm}
        \includegraphics[width = 0.4\columnwidth]{assets/05-All-BoxPlots/09-G10/Risk/G10-Product-Reliable-RISK.png}
        
        \caption{Guideline 10 (scope services when in doubt) -- Participants' scores by attitude toward risk for two dependent variables. 
        In contrast to Fig.~\ref{fig:R-G9-F5-PU}, in this experiment, it was the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} participants who  thought the system would be significantly more useful and reliable when the guideline was applied.}
       \label{fig:G10-PU-T3}
    \end{minipage}
    % \label{fig:overall-precision-recall}
            \Description{FIXME} 

%\FIXME{MMB: See audit for boxplots in to-do. }


\end{figure}

==> figure/01-Results-1/04-Risk-G6-G7-G8.tex <==
\begin{figure}[h]
    \centering
    
    \includegraphics[width = 0.22\linewidth]{assets/05-All-BoxPlots/00-Legends/Risk-Legend.pdf}
    \hspace{5mm}
   % \includegraphics[width = 0.18\linewidth]{assets/05-All-BoxPlots/05-G6/Risk/G6-Feel-Adequate-RISK.png}
    \hspace{5mm}
    \includegraphics[width = 0.18\linewidth]{assets/05-All-BoxPlots/06-G7/Risk/G7-Feel-In-Control-RISK.png}
    \hspace{5mm}
    \includegraphics[width = 0.18\linewidth]{assets/05-All-BoxPlots/07-G8/Risk/G8-Not-Suspicious-RISK.png}
    \hspace{5mm}
    \includegraphics[width = 0.18\linewidth]{assets/05-All-BoxPlots/10-G11/Risk/G11-Feel-In-Control-RISK.png}
    
    
    
    %\includegraphics[width= 0.8\columnwidth]{assets/Risk-G6-7-8/R-G6-G7-G8-Combined.pdf}
    \caption{Guidelines 7, 8, \& 11 sample risk outcomes.
   The top boxplots group is the distributions of ratings for the Violation vignettes, both without disaggregation (white) and disaggregating by attitudes toward risk (\colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} vs. \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant}).
    Dashes (~{\large \rotatebox{90}{\Kutline}}) = medians, dots (.) = means.
    The bottom boxplots group is the ratings for the Application vignettes. \\
    \textbf{(Left)} When Guideline 7 (support efficient invocation) was violated,  \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} felt significantly more in control than the \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant}.
    \textbf{(Center:)} However, when Guideline 8 (support efficient dismissal) was violated, \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} participants felt significantly more suspicious.
    \textbf{(Right:)} When Guideline 11 (make clear why the system did what it did) was violated,  \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} participants felt significantly less in control.
    }
    \label{fig:Risk-G6-G7-G8-Combined}



\end{figure}


==> figure/01-Results-1/05-Risk-G1-G3-Drive.tex <==
\begin{figure}[h]
    \centering

        \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=.7\columnwidth]{assets/05-All-BoxPlots/01-G1/Risk/G1-Feel-Productive-RISK.png}
        
        \caption{Guideline 1 -- participants' attitude towards risk for feeling productive.
        Notice that the \colorboxBackgroundForegroundText{AbiOrange}{black}{risk-averse} people drove the significance observed in the aggregate. }
        \label{fig:R-G1-Productive}
        
        \end{minipage}\hfill
        \begin{minipage}[t]{0.66\textwidth}
        \centering

       \includegraphics[width = 0.32\columnwidth]{assets/05-All-BoxPlots/02-G3/Risk/G3-Feel-Adequate-RISK.png}
       \includegraphics[width = 0.32\columnwidth]{assets/05-All-BoxPlots/02-G3/Risk/G3-Trust-Product-RISK.png}
        \caption{Guideline 3 distributions for participants' feeling adequate and trusting the product through the lens of their attitude towards risk. 
        Notice that unlike in Figure~\ref{fig:R-G1-Productive}, it was the \colorboxBackgroundForegroundText{TimBlue}{black}{risk-tolerant} people drove the significance seen in the aggregate.}
       \label{fig:R-G3-F3-T4}
    \end{minipage}\hfill
    % \label{fig:overall-precision-recall}
            \Description{FIXME} 

\FIXME{MMB: See audit for boxplots in to-do. }


\end{figure}

==> figure/01-Results-1/06-Mot-G5-Learn-G18.tex <==
\begin{figure}[h]
    \centering

        % \begin{minipage}[t]{0.35\textwidth}
        % \centering
        % %\includegraphics[width=0.9\columnwidth]{assets/01-HERE-Insight-1/R-G9.pdf}
        
        % \includegraphics[width = 0.45\columnwidth]{assets/05-All-BoxPlots/16-G18/Motiv/G18-Trust-Product-MOTIV.png}

        
        % \caption{Guideline 5: Match relevant social norms -- Looking at the data through participants' motivations for using technology. 
        % When the guideline was violated, \colorboxBackgroundForegroundText{AbiOrange}{black}{task-oriented} people trusted the system significantly less than the \colorboxBackgroundForegroundText{TimBlue}{black}{tech-oriented}.}
        % \label{fig:M-G5}
        
        % \end{minipage}
        % \hspace{5mm}
        % \begin{minipage}[t]{0.51\textwidth}
        \centering
        
       % \includegraphics[width=0.92\columnwidth]{assets/01-HERE-Insight-1/R-G10png.pdf}
        \includegraphics[width = 0.2\columnwidth]{assets/05-All-BoxPlots/16-G18/Learn/G18-Feel-Certain-LEARN.png}
        \hspace{5mm}
        \includegraphics[width = 0.2\columnwidth]{assets/05-All-BoxPlots/16-G18/Learn/G18-Not-Suspicious-LEARN.png}
        \hspace{5mm}
        \includegraphics[width = 0.2\columnwidth]{assets/05-All-BoxPlots/16-G18/Learn/G18-Not-Harmful-LEARN.png}
        
        \caption{Guideline 18 (Notify users about changes) disaggregated by Learning Style: by Process vs. by Tinkering.
        In this experiment, when the guideline was violated, people who prefer to \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{learn by process} felt significantly less certain and adequate using the Violation than those who prefer to \colorboxBackgroundForegroundText{TimBlueQuote}{black}{learn by tinkering}.}
       \label{fig:L-G18}
    % \end{minipage}
    % \label{fig:overall-precision-recall}
            \Description{FIXME} 

\vspace{-10pt}
\end{figure}



==> figure/07-All-Boxes/Risk/03-G4.tex <==
\begin{figure}[h]
\footnotesize
    \centering
    
    \begin{tabular}{ll|ll|ll|ll|ll|ll}


        \multicolumn{2}{l|}{t(62) = -2.3006} & 
        \multicolumn{2}{l|}{t(61) = -2.9179} & 
         \multicolumn{2}{l|}{t(62) = -3.6258} & 
         \multicolumn{2}{l|}{t(34) = -4.8630} & 
         \multicolumn{2}{l|}{t(39) = -2.8694} &
         \multicolumn{2}{l}{t(63) = -2.6615}\\
         \textit{p}: .0248 & \textit{d}: .580 &
         \textit{p}: .0049 & \textit{d}: .743 &
         \textit{p}: .0005 & \textit{d}: .910 &
         \textit{p}: $<$.0001 & \textit{d}: 1.337 &
         \textit{p}: .0066  & \textit{d}: .763 &
         \textit{p}: .0100 & \textit{d}: .664 \\
        
        \multicolumn{2}{l|}{\includegraphics[width = 0.125\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Feel-Secure-RISK.png}}
         &
         \multicolumn{2}{l|}{\includegraphics[width = 0.125\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Feel-Adequate-RISK.png}}
         &
         \multicolumn{2}{l|}{\includegraphics[width = 0.125\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Feel-Certain-RISK.png}}
         &
         \multicolumn{2}{l|}{\includegraphics[width = 0.125\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Not-Suspicious-RISK.png}}
         
         &
         
         \multicolumn{2}{l|}{\includegraphics[width = 0.125\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Not-Harmful-RISK.png}}
         
         &
         
         \multicolumn{2}{l}{\includegraphics[width = 0.125\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Trust-Product-RISK.png}}\\

        \multicolumn{2}{l|}{t(61) = -3.1984} & 
        \multicolumn{2}{l|}{t(62) = -2.4955} & 
         \multicolumn{2}{l|}{t(63) = -4.7513} & 
         \multicolumn{2}{l|}{t(42) = -5.1692} & 
         \multicolumn{2}{l|}{t(44) = -3.1328} &
         \multicolumn{2}{l}{t(62) = -2.6615}\\
         \textit{p}: .0022 & \textit{d}: .814 &
         \textit{p}: .0153 & \textit{d}: .629 &
         \textit{p}: $<$.0001 & \textit{d}: 1.186 &
         \textit{p}: $<$.0001 & \textit{d}: 1.364 &
         \textit{p}: .0031  & \textit{d}: .821 &
         \textit{p}: .0004 & \textit{d}: .937 \\
         
         
         
    \end{tabular}
    \caption{Guideline 4 had six instances of  Pattern~\#3, inclusivity gaps in {both} \violationBox{dashed} and \applicationBox{solid} boxes.
    Notice that in all six instances, the risk-averse \textit{always} had the significantly lower average in both the \vioProduct{} and the \appProduct{}}
    \label{fig:third-category-guideline-4}
    \vspace{0pt}
\end{figure}

% \begin{figure}[]
%     \centering
%     \begin{tabular}{cc|cc|cc|cc|cc}
%     \multicolumn{2}{c|}{\includegraphics[width = 0.16\columnwidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Feel-In-Control-RISK.png}} 
%     &
%     \multicolumn{2}{c|}{\includegraphics[width = 0.16\columnwidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Feel-Secure-RISK.png}} 
%     &
%     \multicolumn{2}{c|}{\includegraphics[width = 0.16\columnwidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Feel-Adequate-RISK.png}} 
%     &
%     \multicolumn{2}{c|}{\includegraphics[width = 0.16\columnwidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Feel-Certain-RISK.png}} 
%     &
%     \multicolumn{2}{c}{\includegraphics[width = 0.16\columnwidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Feel-Productive-RISK.png}}
%     \\
%     \hline
%     \multicolumn{2}{c|}{\includegraphics[width = 0.16\columnwidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Perceived-Useful-RISK.png}} &
%     \multicolumn{2}{c|}{\includegraphics[width = 0.16\columnwidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Not-Suspicious-RISK.png}} &
%     \multicolumn{2}{c|}{\includegraphics[width = 0.16\columnwidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Not-Harmful-RISK.png}} &
%     \multicolumn{2}{c|}{\includegraphics[width = 0.16\columnwidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Product-Reliable-RISK.png}} &
%     \multicolumn{2}{c}{\includegraphics[width = 0.16\columnwidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Trust-Product-RISK.png}}
%     \end{tabular}
    
%     \caption{Guideline 4 participants' ratings for all dependent variables, disaggregated by participants' attitudes toward risk.
%     Guideline 4 demonstrated all 3 categories of insight, closing gaps category (dashed red box \textit{only}), creating gaps category (solid red box \textit{only}), and pervasive gaps category ({both} dashed \textit{and} solid red boxes).
% 	%For the disaggregated data, notice how large the distances between the average rating are when the guideline is applied.
% 	Table~\ref{tab:G4-Stats} below provides the statistics.
% }
%     \label{fig:Risk-G4-All}
% \end{figure}

% \begin{figure}[t]
% 	\includegraphics[width = \linewidth]{assets/Appendices/03-G4/RISK-G4-All.pdf}
% 	%\includegraphics[width = .25\linewidth]{assets/figure.png}
% 	\caption{ Guideline 4 participants' ratings for the 10 dependent variables, both in the aggregate (black and white) and disaggregated by the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} and \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant}.
% 	For the disaggregated data, notice how large the distances between the average rating are when the guideline is applied.
% 	Table~\ref{tab:G4-Stats} below provides the statistics.
%     }%
% 	\label{fig:Risk-G4-All}

% \end{figure}

==> figure/G11-In-Control-Data-disagg.tex <==
\begin{figure}
        \centering
        \includegraphics[width = 0.78\linewidth]{assets/G11-In-Control-Data-disagg.pdf} 
        \caption{Guideline 11: Figure~\ref{fig:G11-In-Control-Data}'s data, now disaggregated by participants' attitudes toward risk.
        \textbf{(a)}: Legend for all figures in Sections~\ref{subsec:why-disaggregate} \&~\ref{subsec:3-categories}. 
        \textbf{(b)}\vioProduct{}: reveals that Figure~\ref{fig:G11-In-Control-Data}(b)'s bimodal peaks cluster by participants' attitudes toward risk:
        most \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} participants felt a lack of control, but most \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} felt in control.
        % \textbf{(c)}: Disaggregating by participants' attitudes toward risk showed that the two peaks clustered by participants' attitudes toward risk;
        \textbf{({c})}: \appProduct{}: Although about half the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} and about 2/3 of the \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants felt more in control than with \vioProduct{}, almost all those who did not were the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} participants.
        % \textbf{(e)} Disaggregating: both risk attitudes benefited, but risk-averse users may still need additional support.
        %61.3\% of the risk-averse participants agreed, and 87.5\% of the risk-tolerant participants did the same.
        % \textbf{(f)}: To assess the distance between averages ($\times$s) and spread of the data for statistical inferences, we visualized all data with box plots.
        % For all figures, each box from top-to bottom is as follows: Violation AI-product (overall, risk-averse, risk-tolerant), Application AI-product (overall, risk-averse, risk-tolerant).
        }
        \label{fig:G11-In-Control-Data-disagg}
\end{figure}

==> figure/G11-In-Control-Data-non.tex <==
\begin{figure}
        \centering
        \includegraphics[width = 0.78\linewidth]{assets/G11-In-Control-Data.pdf}
        \caption{Guideline~11's percentage of participants (y-axes) responding from ``strongly disagree'' (1) to ``strongly agree'' (7) (x-axes) for the ``I would feel in control...'' dependent variable.
        \textbf{(a)}: Legend for this figure. 
        \textbf{(b)}: \vioProduct{}, which violated Guideline~11: a bimodal distribution, with median = 4.
        \textbf{({c})}: \appProduct{}, which applied Guideline~11:  still bimodal, but with median = 5.
        }
        \label{fig:G11-In-Control-Data}
        \FIXME{Change the legend to exclude the attitudes toward risk.}
\end{figure}

==> figure/z-Appendices/Facet-Survey.tex <==
\begin{figure}[b!]
    \centering
    \includegraphics[width = \columnwidth]{assets/Facet-Survey.png}
\end{figure}
% \begin{figure}[b!]
%     \centering
%     \includegraphics[width = \columnwidth]{assets/Facet-Survey-P2.png}
% \end{figure}
% \begin{figure}[b!]
%     \centering
%     \includegraphics[width = \columnwidth]{assets/Facet-Survey-P3.pdf}
% \end{figure}
\begin{figure}[b!]
    \centering
    \includegraphics[width = \columnwidth]{assets/Facet-Survey-P4.png}
    \label{fig:facet-survey}
    \caption{The GenderMag problem solving style survey.
            The left-most column shows which of the styles each question relates to, as well as the 3 attention check questions.
            On the first page, people respond from "strongly disagree" to "strongly agree."
            On the second page, people responses relate to which end of the question they align with more.}
\end{figure}

==> tables/00-Agg-vs-Dis.tex <==
\begin{table}[h]
\centering

\framebox[\linewidth]{For Measuring!}

\begin{tabular}
{
|p{0.22\linewidth}| %First Column
p{0.01\linewidth}| %G1
p{0.013\linewidth}| %G3
p{0.013\linewidth}| %G4
p{0.015\linewidth}| %G5
p{0.025\linewidth}| %G6
p{0.013\linewidth}| %G7
p{0.013\linewidth}| %G8
p{0.015\linewidth}| %G9
p{0.0255\linewidth}| %G10
p{0.0255\linewidth}| %G11
p{0.0255\linewidth}| %G12
p{0.0255\linewidth}| %G13
p{0.0255\linewidth}| %G14
p{0.0255\linewidth}| %G15
p{0.0255\linewidth}| %G17
p{0.0255\linewidth}| %G18
}


% %\rowcolor{LightCyan}
% \multicolumn{8}{p{.51\linewidth}|}{\cellcolor{LightCyan}These are the guidelines where 1 (or more) dependent variables' average had a significant distance between the guideline application by relevant facet (Table~\ref{table:personas} color $\implies$ average \textbf{higher})
%  } & 
% \multicolumn{9}{p{.427\linewidth}}{ %
% %\includegraphics[height = 2cm]{assets/Table-4-Examplepng.pdf}
% }\\%
% \hline
% \hline


& \textbf{1} %
& \textbf{3} %
& \textbf{4}%
& \textbf{5} %
& \textbf{6}%
& \textbf{7} %
& \textbf{8} %
& \textbf{9} %
& \textbf{10} %
& \textbf{11} %
& \textbf{12} %
& \textbf{13} %
& \textbf{14} %
& \textbf{15} %
& \textbf{17} %
& \textbf{18} %
\\%
\hline



\textbf{Aggregate:} 
& 
& 
& 
& 
& 
& 
& 
& 
& 
& 
&
&   
&
& 
& 
&  \\
\textbf{$|\mu_{App} - \mu_{Vio}| > 0.75$?} 
& 0
& 3
& 0
& 0
& 10
& 8
& 7
& 9
& 8
& 8
& 0
& 1
& 3
& 4
& 4
& 0 \\


\hline

\textbf{Disaggregation:} 
& 
& 
& 
& 
& 
& 
& 
& 
& 
& 
&
&   
&
& 
& 
&  \\
\textbf{How many possible differences?} 
& 7
& 35
& 18
& 10
& 107
& 81
& 77
& 86
& 84
& 71
& 2
& 58
& 41
& 45
& 34
&  35\\


% \textbf{Did disaggregation add value?} 
% & $\times$
% & $\times$
% &  
% & $\times$
% &  \checkmark
% &  \checkmark
% & 
% &  \checkmark 
% & 
% & 
% &
% & \checkmark  
% &
% & 
% & 
% & \checkmark \\




\end{tabular}
\vspace{5pt}
    \caption{This table's top row shows how many of the 10 dependent variables had a distance between the means of 0.75 or higher.}

    
    \label{table:SE-IP-Triangulations}
\end{table}




==> tables/01-G1-Results/G1-Risk-Table.tex <==
\begin{table}[h]
\centering

\includegraphics[width = \linewidth]{assets/001-Results-1/Tables/Table-4-Step-2.pdf}

%\framebox[\linewidth]{For Measuring!}

% \begin{tabular}
% {
% p{0.252\linewidth}| %First Column
% p{0.01\linewidth}| %G1
% p{0.01\linewidth}| %G3
% p{0.01\linewidth}| %G4
% p{0.01\linewidth}| %G5
% p{0.01\linewidth}| %G6
% p{0.01\linewidth}| %G7
% p{0.01\linewidth}| %G8
% p{0.01\linewidth}| %G9
% p{0.0255\linewidth}| %G10
% p{0.0255\linewidth}| %G11
% p{0.0255\linewidth}| %G12
% p{0.0255\linewidth}| %G13
% p{0.0255\linewidth}| %G14
% p{0.0255\linewidth}| %G15
% p{0.0255\linewidth}| %G17
% p{0.0255\linewidth}  %G18
% }


% % %\rowcolor{LightCyan}
% % \multicolumn{8}{p{.51\linewidth}|}{\cellcolor{LightCyan}These are the guidelines where 1 (or more) dependent variables' average had a significant distance between the guideline application by relevant facet (Table~\ref{table:personas} color $\implies$ average \textbf{higher})
% %  } & 
% % \multicolumn{9}{p{.427\linewidth}}{ %
% % %\includegraphics[height = 2cm]{assets/Table-4-Examplepng.pdf}
% % }\\%
% % \hline
% % \hline

% \diagbox[width = 1.1\linewidth] {\textbf{Facet}}{\textbf{Guideline}}
% & \textbf{1} %
% & \textbf{3} %
% & \textbf{4}%
% & \textbf{5} %
% & \textbf{6}%
% & \textbf{7} %
% & \textbf{8} %
% & \textbf{9} %
% & \textbf{10} %
% & \textbf{11} %
% & \textbf{12} %
% & \textbf{13} %
% & \textbf{14} %
% & \textbf{15} %
% & \textbf{17} %
% & \textbf{18} %
% \\%
% \hline
% \hline


% \textbf{Was there aggregate significance?} 
% & $\times$
% & $\times$
% &  
% & $\times$
% &  \checkmark
% &  \checkmark
% & 
% &  \checkmark 
% & 
% & 
% &
% & \checkmark  
% &
% & 
% & 
% & \checkmark \\


% \hline

% \textbf{Info. Processing} 
% & \cellcolor{AbiOrange}\checkmark 
% & \cellcolor{AbiOrange}\checkmark  
% & 
% & 
% & 
% & 
% & 
% & 
% &
% &
% & 
% & 
% & 
% &
% & 
% &  \\

% \hline 

% \textbf{Self-Efficacy} 
% & \cellcolor{TimBlue}\checkmark 
% & \cellcolor{TimBlue}\checkmark  
% &  
% & \cellcolor{TimBlue}\checkmark  
% & \cellcolor{AbiOrange} \checkmark
% & \cellcolor{TimBlue} \checkmark
% & 
% & \cellcolor{TimBlue} \checkmark 
% & 
% & 
% &
% & \cellcolor{TimBlue}\checkmark  
% &
% & 
% & 
% & \cellcolor{TimBlue}\checkmark \\

% \hline
% \textbf{Risk} 
% & \cellcolor{AbiOrange} \checkmark
% &  
% & \cellcolor{TimBlue} \checkmark  
% & \cellcolor{TimBlue} \checkmark  
% &  
% &  
% &  
% & \cellcolor{TimBlue} \checkmark 
% & \cellcolor{AbiOrange} \checkmark 
% & \cellcolor{TimBlue} \checkmark 
% &  
% & \cellcolor{TimBlue}\checkmark 
% & \cellcolor{TimBlue}\checkmark 
% & \cellcolor{TimBlue}\checkmark
% & 
% & \\





% \end{tabular}
    \caption{This table builds from Table~\ref{table:SE-IP-Triangulations}, also showing people's attitude towards risk.
    Notice that for attitude towards risk, \textit{more} than half of the experiments exhibited significant distances between the means, and 77.8\% of them were in favor of those with \colorboxBackgroundForegroundText{TimBlue}{black}{risk tolerant} participants.
    %The top row shows if the aggregate of participants for the \textit{same dependent variables} showed significance.
    %Notice that whether there was significance in the aggregate (\checkmark) or not ($\times$), there was still added value in disaggregating.  
    }
    \FIXME{MMB: update this when audits done for this table (see global TODO for audit type numberings: \\
    Audit1 (status: not done; by: nobody yet\\
    Audit2 (status: not done; by: nobody yet\\
    Audit3 (status: not done; by: nobody yet}

    
    \label{table:Triangulation-With-Risk}
\end{table}




==> tables/01-G1-Results/G1-SE-Table.tex <==
\begin{table}[h]
\centering

%\framebox[\linewidth]{For Measuring!}

\begin{tabular}
{
p{0.252\linewidth}| %First Column
p{0.01\linewidth}| %G1
p{0.01\linewidth}| %G3
p{0.01\linewidth}| %G4
p{0.01\linewidth}| %G5
p{0.01\linewidth}| %G6
p{0.01\linewidth}| %G7
p{0.01\linewidth}| %G8
p{0.01\linewidth}| %G9
p{0.0255\linewidth}| %G10
p{0.0255\linewidth}| %G11
p{0.0255\linewidth}| %G12
p{0.0255\linewidth}| %G13
p{0.0255\linewidth}| %G14
p{0.0255\linewidth}| %G15
p{0.0255\linewidth}| %G17
p{0.0255\linewidth}  %G18
}


% %\rowcolor{LightCyan}
% \multicolumn{8}{p{.51\linewidth}|}{\cellcolor{LightCyan}These are the guidelines where 1 (or more) dependent variables' average had a significant distance between the guideline application by relevant facet (Table~\ref{table:personas} color $\implies$ average \textbf{higher})
%  } & 
% \multicolumn{9}{p{.427\linewidth}}{ %
% %\includegraphics[height = 2cm]{assets/Table-4-Examplepng.pdf}
% }\\%
% \hline
% \hline

\diagbox[width = 1.1\linewidth] {\textbf{Facet}}{\textbf{Guideline}}
& \textbf{1} %
& \textbf{3} %
& \textbf{4}%
& \textbf{5} %
& \textbf{6}%
& \textbf{7} %
& \textbf{8} %
& \textbf{9} %
& \textbf{10} %
& \textbf{11} %
& \textbf{12} %
& \textbf{13} %
& \textbf{14} %
& \textbf{15} %
& \textbf{17} %
& \textbf{18} %
\\%
\hline
\hline


% \textbf{Was there aggregate significance?} 
% & $\times$
% & $\times$
% &  
% & $\times$
% &  \checkmark
% &  \checkmark
% & 
% &  \checkmark 
% & 
% & 
% &
% & \checkmark  
% &
% & 
% & 
% & \checkmark \\


\hline

\textbf{Info. Processing} 
& \cellcolor{AbiOrange}\checkmark 
& \cellcolor{AbiOrange}\checkmark  
& 
& 
& 
& 
& 
& 
&
&
& 
& 
& 
&
& 
&  \\

\hline 

\textbf{Self-Efficacy} 
& \cellcolor{TimBlue}\checkmark 
& \cellcolor{TimBlue}\checkmark  
&  
& \cellcolor{TimBlue}\checkmark  
& \cellcolor{AbiOrange} \checkmark
& \cellcolor{TimBlue} \checkmark
& 
& \cellcolor{TimBlue} \checkmark 
& 
& 
&
& \cellcolor{TimBlue}\checkmark  
&
& 
& 
& \cellcolor{TimBlue}\checkmark \\





\end{tabular}
\vspace{5pt}
    \caption{This shows which guidelines (columns) had dependent variables with significant distances between the application means for people's self-efficacy and information processing.
    Notice that for people's self-efficacy, half of the experiments exhibited significant distances between the means, and 87.5\% of them were in favor of those with \colorboxBackgroundForegroundText{TimBlue}{black}{higher self-efficacy} relative to their peers.
    %The top row shows if the aggregate of participants for the \textit{same dependent variables} showed significance.
    %Notice that whether there was significance in the aggregate (\checkmark) or not ($\times$), there was still added value in disaggregating.  
    }

\FIXME{MMB: update this when audits done for this table (see global TODO for audit type numberings: \\
    Audit1 (status: not done; by: nobody yet\\
    Audit2 (status: not done; by: nobody yet\\
    Audit3 (status: not done; by: nobody yet}

    
    \label{table:SE-IP-Triangulations}
\end{table}




==> tables/01-Vignettes/G01-Vignette.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline

\textbf{Guideline 1 Application Vignette} & \textbf{Guideline 1 Violation Vignette} \\
\hline

You are using a presentation app similar to Microsoft PowerPoint, Google Slides, Apple Keynote to make slides for a presentation.
It is called [Application AI product].
[Application AI product] has a capability called Presenter Coach that gives you feedback on your presentation skills as you practice your presentation in front of your computer.
& 

You are using a presentation app similar to Microsoft PowerPoint, Google Slides, Apple Keynote to make slides for a presentation.
It is called [Application AI product].
[Application AI product] has a capability called Presenter Coach that gives you feedback on your presentation skills as you practice your presentation in front of your computer.\\
 & \\
 
When you turn on Presenter Coach, it displays information like this: As you practice your presentation, we will give you feedback about your presentation style: how fast you speak, use of filler words (such as ``um'' and ``like''), use of inappropriate words (such as ``damn'').
&

When you turn on Presenter Coach, it displays information like this: We will help you improve your presentation style.\\
\hline


\end{tabular}

\caption{Guideline 1's vignettes for guideline application (left) and violation (right). }
    
\label{table:G1-Vignette-Appendix}

\end{table}

==> tables/01-Vignettes/G03-Vignette.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline

\textbf{Guideline 3 Application Vignette} & \textbf{Guideline 3 Violation Vignette} \\
\hline

You are using an email application called [Application AI product].
It is similar to Gmail, Outlook, Apple Mail, etc.
[Application AI product] pops up notifications on your screen when you have new emails.


& 

You are using an email application called [Violation AI product].
It is similar to Gmail, Outlook, Apple Mail, etc.
[Violation AI product] pops up notifications on your screen when you have new emails.\\

 
As you use [Application AI product], you notice that [Application AI product] stops the notifications when you are busy, for example, when giving a presentation.
&

As you use [Violation AI product], you notice that [Violation AI product] pops up notifications whenever a new email arrives, regardless of your activity.\\
\hline


\end{tabular}

\caption{Guideline 3's vignettes for guideline application (left) and violation (right). }
    
\label{table:G3-Vignette-Appendix}

\end{table}


==> tables/01-Vignettes/G04-Vignette.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline

\textbf{Guideline 4 Application Vignette} & \textbf{Guideline 4 Violation Vignette} \\
\hline

You are using a document editing app called [Application] to write documents.
It is similar to MS Word, Google Docs, Apple Pages.
It has a feature that defines meanings of acronyms.
For example, if you see an acronym such as ``CDC'' in a document, you can access an explanation of what CDC stands for (such as, Centers for Disease Control).
& 

You are using a document editing app called [Violation] to write documents.
It is similar to MS Word, Google Docs, Apple Pages.
It has a feature that defines meanings of acronyms.
For example, if you see an acronym such as ``CDC'' in a document, you can access an explanation of what CDC stands for (such as, Centers for Disease Control).\\
 & \\
 
When you highlight an acronym to see what it stands for, {[Application] shows you definitions that are used in your workplace and pertain to the topic of the current document.}
&

When you highlight an acronym to see what it stands for, {[Violation] shows you a standard list of possible definitions taken from a popular acronym dictionary.}\\
\hline


\end{tabular}

\caption{Guideline 4's vignettes for guideline application (left) and violation (right).}
    
\label{table:G4-Vignette-Appendix}

\end{table}

==> tables/01-Vignettes/G05-Vignette.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline

\textbf{Guideline 5 Application Vignette} & \textbf{Guideline 5 Violation Vignette} \\
\hline

You are using a document editing app called [Application AI product] to write documents.
It is similar to Microsoft Word, Google Docs, Apple Pages.
[Application AI product] has a feature that makes suggestions to improve your writing style.


& 

You are using a document editing app called [Violation AI product] to write documents.
It is similar to Microsoft Word, Google Docs, Apple Pages.
[Violation AI product] has a feature that makes suggestions to improve your writing style.\\

 
You are writing a document, and [Application AI product] presents its suggested options by saying:

``Consider using...''
&

You are writing a document, and [Violation AI product] presents its suggested options by saying:

``You made a mistake. Replace with...''\\
\hline


\end{tabular}

\caption{Guideline 5's vignettes for guideline application (left) and violation (right). }
    
\label{table:G5-Vignette-Appendix}

\end{table}


==> tables/01-Vignettes/G06-Vignette.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline

\textbf{Guideline 6 Application Vignette} & \textbf{Guideline 6 Violation Vignette} \\
\hline

You are using an online search engine called [Application AI product] to search for images of CEOs and doctors.


& 

You are using an online search engine called [Violation AI product] to search for images of CEOs and doctors.\\

 
On the first page, the search results show images of different types of people in terms of gender and skin tone, including people who look like you.
&

The search results don't show any images of women or people of color on the first page.\\
\hline


\end{tabular}

\caption{Guideline 6's vignettes for guideline application (left) and violation (right). }
    
\label{table:G6-Vignette-Appendix}

\end{table}


==> tables/01-Vignettes/G07-Vignette.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline

\textbf{Guideline 7 Application Vignette} & \textbf{Guideline 7 Violation Vignette} \\
\hline

You are using a presentation app similar to Microsoft PowerPoint, Google Slides, Apple Keynote to make slides for a presentation.
It is called [Application AI product].
[Application AI product] has a capability called Design Helper that provides alternative design ideas.
As you work on a slide and add text and images, Design Helper automatically provides you with design suggestions for alternative layouts.


& 

You are using a presentation app similar to Microsoft PowerPoint, Google Slides, Apple Keynote to make slides for a presentation.
It is called [Violation AI product].
[Violation AI product] has a capability called Design Helper that provides alternative design ideas.
As you work on a slide and add text and images, Design Helper automatically provides you with design suggestions for alternative layouts.\\


 
You are working on a slide and need some design help, but Design Helper hasn't automatically popped up any design suggestions.
You click a button visible on the interface to request suggestions and they appear on the side bar.

&

You are working on a slide and need some design help, but Design Helper hasn't automatically popped up any design suggestions.
There is no button visible on the interface that you could use to request suggestions from Design Helper.\\
\hline


\end{tabular}

\caption{Guideline 7's vignettes for guideline application (left) and violation (right). }
    
\label{table:G7-Vignette-Appendix}

\end{table}


==> tables/01-Vignettes/G08-Vignette.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline

\textbf{Guideline 8 Application Vignette} & \textbf{Guideline 8 Violation Vignette} \\
\hline

You are using a presentation app similar to Microsoft PowerPoint, Google Slides, Apple Keynote to make slides for a presentation.
It is called [Application AI product].
[Application AI product] has a capability called Design Helper that provides alternative design ideas.
As you work on a slide and add text and images, Design Helper automatically provides you with design suggestions for alternative layouts.


& 

You are using a presentation app similar to Microsoft PowerPoint, Google Slides, Apple Keynote to make slides for a presentation.
It is called [Violation AI product].
[Violation AI product] has a capability called Design Helper that provides alternative design ideas.
As you work on a slide and add text and images, Design Helper automatically provides you with design suggestions for alternative layouts.\\

 
You are working on a slide and Design Helper pops up, showing you some design suggestions.
You do not need any design help at this time, so you click on a button visible on screen to hide the design suggestions.

&

You are working on a slide and Design Helper pops up, showing you some design suggestions.
You do not need any design help at this time, but there is no way to hide the design suggestions.\\
\hline


\end{tabular}

\caption{Guideline 8's vignettes for guideline application (left) and violation (right). }
    
\label{table:G8-Vignette-Appendix}

\end{table}


==> tables/01-Vignettes/G09-Vignette.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline

\textbf{Guideline 9 Application Vignette} & \textbf{Guideline 9 Violation Vignette} \\
\hline

You are using a presentation app similar to Microsoft PowerPoint, Google Slides, Apple Keynote to make slides for a presentation.
It is called [Application AI product].
[Application AI product] has a capability called Design Helper that provides alternative design ideas.
As you work on a slide and add text and images, Design Helper automatically provides you with design suggestions for alternative layouts.


& 

You are using a presentation app similar to Microsoft PowerPoint, Google Slides, Apple Keynote to make slides for a presentation.
It is called [Violation AI product].
[Violation AI product] has a capability called Design Helper that provides alternative design ideas.
As you work on a slide and add text and images, Design Helper automatically provides you with design suggestions for alternative layouts.\\

 
You are working on a slide and Design Helper shows you a few design suggestions.
You click one of the suggestions, and the layout is applied to the current slide.
You decide you want to make a few changes to the layout, such as resizing or repositioning the images, which you can do directly on the slide.

&

You are working on a slide and Design Helper shows you a few design suggestions.
You click one of the suggestions, and the layout is applied to the current slide.
You decide you want to make a few changes to the layout, such as resizing or repositioning the images, but you see that it does not allow you to make changes.\\
\hline


\end{tabular}

\caption{Guideline 9's vignettes for guideline application (left) and violation (right). }
    
\label{table:G9-Vignette-Appendix}

\end{table}


==> tables/01-Vignettes/G10-Vignette.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline

\textbf{Guideline 10 Application Vignette} & \textbf{Guideline 10 Violation Vignette} \\
\hline

You are using a document editing app called [Application AI product] to write documents.
It is similar to Microsoft Word, Google Docs, Apple Pages.
[Application AI product] has a spelling assistant that can automatically detect typos.



& 

You are using a document editing app called [Violation AI product] to write documents.
It is similar to Microsoft Word, Google Docs, Apple Pages.
[Violation AI product] has a spelling assistant that can automatically detect typos.\\


 
You are writing a document, and you make a typo.
The spelling assistant isn't sure what word you intended to type, so it provides multiple options for you to choose from.

&

You are writing a document, and you make a typo.
The spelling assistant isn't sure what word you intended to type, so it replaces the typo with its best bet.
For example, if you type ``multipl'', it automatically replaces it with ``multiple'', even though other options might make sense--e.g., multiple, multiplex.\\
\hline


\end{tabular}

\caption{Guideline 10's vignettes for guideline application (left) and violation (right). }
    
\label{table:G10-Vignette-Appendix}

\end{table}


==> tables/01-Vignettes/G11-Vignette.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline

\textbf{Guideline 11 Application Vignette} & \textbf{Guideline 11 Violation Vignette} \\
\hline

You are using a spreadsheet app called [Application AI product] to analyze some data.
It is similar to MS Excel, Google Sheets, Apple Numbers.
[Application AI product] has a feature that suggests charts based on the data you have in a file.
For each suggested chart, the interface shows an interesting insight that summarizes the data--for example, ``People who walk to work drink more coffee than people who drive.''



& 

You are using a spreadsheet app called [Violation AI product] to analyze some data.
It is similar to MS Excel, Google Sheets, Apple Numbers.
[Violation AI product] has a feature that suggests charts based on the data you have in a file.
For each suggested chart, the interface shows an interesting insight that summarizes the data--for example, ``People who walk to work drink more coffee than people who drive.''\\

 
As you use [Application AI product], you wonder how each suggested chart and insight was generated, and you notice a button under each chart that you can click to access an explanation.
&

As you use [Violation AI product], you wonder how each suggested chart and insight was generated but are unable to access an explanation.\\
\hline


\end{tabular}

\caption{Guideline 11's vignettes for guideline application (left) and violation (right). }
    
\label{table:G11-Vignette-Appendix}

\end{table}


==> tables/01-Vignettes/G12-Vignette.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline

\textbf{Guideline 12 Application Vignette} & \textbf{Guideline 12 Violation Vignette} \\
\hline

You are using an email application called [Application AI product].
It is similar to Gmail, Outlook, Apple Mail, etc.



& 

You are using an email application called [Violation AI product].
It is similar to Gmail, Outlook, Apple Mail, etc.\\


 
When attaching a file, [Application AI product] shows a list of recent files you worked on to choose from, along with a file explorer you can use to navigate to other files not in the list.
&

When attaching a file, [Violation AI product] opens a file explorer window you can use to navigate to files.\\
\hline


\end{tabular}

\caption{Guideline 12's vignettes for guideline application (left) and violation (right). }
    
\label{table:G12-Vignette-Appendix}

\end{table}


==> tables/01-Vignettes/G13-Vignette.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline

\textbf{Guideline 13 Application Vignette} & \textbf{Guideline 13 Violation Vignette} \\
\hline

You are using a presentation app similar to Microsoft PowerPoint, Google Slides, Apple Keynote to make slides for a presentation.
It is called [Application AI product].
[Application AI product] has a capability called Design Helper that provides alternative design ideas.
As you work on a slide and add text and images, Design Helper automatically provides you with design suggestions for alternative layouts.


& 

You are using a presentation app similar to Microsoft PowerPoint, Google Slides, Apple Keynote to make slides for a presentation.
It is called [Violation AI product].
[Violation AI product] has a capability called Design Helper that provides alternative design ideas.
As you work on a slide and add text and images, Design Helper automatically provides you with design suggestions for alternative layouts.\\


 
As you make slides, you pick from the design suggestions offered by Design Helper.
You usually pick designs that feature the color blue.
After using [Application AI product] a few times, you notice it has learned your preferences and now features blue designs prominently.

&

As you make slides, you pick from the design suggestions offered by Design Helper.
You usually pick designs that feature the color blue.
After using [Violation AI product] a few times, you notice it has not learned your preferences, and blue designs appear in the same place among the suggested designs as the first time you used it.\\
\hline


\end{tabular}

\caption{Guideline 13's vignettes for guideline application (left) and violation (right). }
    
\label{table:G13-Vignette-Appendix}

\end{table}


==> tables/01-Vignettes/G14-Vignette.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline

\textbf{Guideline 14 Application Vignette} & \textbf{Guideline 14 Violation Vignette} \\
\hline

You are using a document editing app similar to Microsoft Word, Google Docs, Apple Pages, called [Application AI product]


& 

You are using a document editing app similar to Microsoft Word, Google Docs, Apple Pages, called [Violation AI product]\\


 
As you work on a document, the app automatically updates a small dedicated part of the menu bar at the top right, based on what functionality it thinks you'll need next.
The rest of the menu bar never changes.

&

As you work on a document, the app automatically updates the entire menu bar at the top based on what functionality it thinks you'll need next.\\
\hline


\end{tabular}

\caption{Guideline 14's vignettes for guideline application (left) and violation (right). }
    
\label{table:G14-Vignette-Appendix}

\end{table}


==> tables/01-Vignettes/G15-Vignette.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline

\textbf{Guideline 15 Application Vignette} & \textbf{Guideline 15 Violation Vignette} \\
\hline

You are using a spreadsheet app called [Application AI product] to analyze some data.
It is similar to MS Excel, Google Sheets, Apple Numbers.
[Application AI product] has a feature that suggests charts based on the data you have in a file.



& 

You are using a spreadsheet app called [Violation AI product] to analyze some data.
It is similar to MS Excel, Google Sheets, Apple Numbers.
[Violation AI product] has a feature that suggests charts based on the data you have in a file.\\


 
Below each suggested chart, [Application AI product] shows buttons you can use to provide feedback as to whether that suggestion is useful to you or not.
&

[Violation AI product] does not have a way for you to provide feedback as to whether any suggestion is useful to you or not.\\
\hline


\end{tabular}

\caption{Guideline 15's vignettes for guideline application (left) and violation (right). }
    
\label{table:G15-Vignette-Appendix}

\end{table}


==> tables/01-Vignettes/G17-Vignette.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline

\textbf{Guideline 17 Application Vignette} & \textbf{Guideline 17 Violation Vignette} \\
\hline

You are using an email application called [Application AI product].
It is similar to Gmail, Outlook, Apple Mail, etc.
[Application AI product] can automatically sort your emails into 2 categories: \textit{important} email and \textit{other} emails.



& 

You are using an email application called [Violation AI product].
It is similar to Gmail, Outlook, Apple Mail, etc.
[Violation AI product] can automatically sort your emails into 2 categories: \textit{important} email and \textit{other} emails.\\


 
As you use [Application AI product], you notice that emails from some important people (e.g., your boss, your mom) are not being marked as \textit{important}.
[Application AI product] provides a setting where you can enter the names of specific people to make sure they are always marked as \textit{important} going forward.
&

As you use [Violation AI product], you notice that emails from some important people (e.g., your boss, your mom) are not being marked as \textit{important}.
Going forward, you periodically check the \textit{other} email category to make sure you are not missing emails from those \textit{important} people.\\
\hline


\end{tabular}

\caption{Guideline 17's vignettes for guideline application (left) and violation (right). }
    
\label{table:G17-Vignette-Appendix}

\end{table}


==> tables/01-Vignettes/G18-Vignette.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline

\textbf{Guideline 18 Application Vignette} & \textbf{Guideline 18 Violation Vignette} \\
\hline

You are using an email application called [Application AI product].
It is similar to Gmail, Outlook, Apple Mail, etc.
[Application AI product] can automatically sort your emails into 2 categories: \textit{important} email and \textit{other} emails.



& 

You are using an email application called [Violation AI product].
It is similar to Gmail, Outlook, Apple Mail, etc.
[Violation AI product] can automatically sort your emails into 2 categories: \textit{important} email and \textit{other} emails.\\

 
Occasionally, [Application AI product] improves the way it sorts emails into \textit{important} and \textit{other}.
For example, one day it informs you that:

\begin{itemize}
    \item ``From now on, emails Sarah [your boss] will always appear in the important category and emails from Local News [some mailing lists] will no longer appear the important category.''
\end{itemize}
&

Occasionally, [Violation AI product] improves the way it sorts emails into \textit{important} and \textit{other}.
For example, as you use it, you notice that emails from your boss start to appear in the important category when they didn't always before and emails from some mailing lists no longer seem to appear in the important category.\\
\hline


\end{tabular}

\caption{Guideline 18's vignettes for guideline application (left) and violation (right). }
    
\label{table:G18-Vignette-Appendix}

\end{table}


==> tables/02-F1-Vignette/G1-Vignette.tex <==
\begin{table}[h]
\centering

\includegraphics[width = \linewidth]{assets/G1-Vignette.pdf}

\caption{Guideline 1's (make clear what the system can do) vignettes for application (left) and violation (right).
    Each vignette had 3 components: (1) a product and feature introduction, (2) the behavior description of the AI-powered component, (3) the AI performance description, which Li et al.  dropped from their analyses, since AI-optimality was only significant in one of the 16 experiments.    (Appendix~\ref{sec:Appendix-Boxplots} shows all 16 experiments' vignettes.)}
    
\label{table:G1-Vignette}

\vspace{-15pt}
\end{table}

==> tables/02-F1-Vignette/G4-Vignette.tex <==
\begin{table}[h]
\centering

\includegraphics[width = \linewidth]{assets/G4-Vignette.pdf}

\caption{Guideline 4's (show contextually relevant information) vignettes for application (left) and violation (right).
    The persistent gaps found in Section~\ref{sec:category-3} may have been because of people misinterpreting the AI product's abilities.}
    
\label{table:G1-Vignette}

\vspace{-15pt}
\end{table}

==> tables/03-Inclusivity-Risk-Walkthrough.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{0.2\linewidth}|c|c}
         Guideline&  Risk-Averse Inclusivity & Risk-Tolerant Inclusivity\\
         \toprule
         8: Support efficient dismissal
         & \includegraphics[width = 0.35\linewidth]{assets/05-All-BoxPlots/07-G8/Risk/G8-Not-Suspicious-ABI-WITHIN-RISK.png} 
         & \includegraphics[width = 0.35\linewidth]{assets/05-All-BoxPlots/07-G8/Risk/G8-Not-Suspicious-TIM-WITHIN-RISK.png}

    \end{tabular}
    \caption{Inclusivity example, from Guideline~8's experiment:  
    %For Guideline 8, participants' attitudes toward risk uncovers about their user experience inclusivity for their responses to the ``I would not be suspicious'' dependent variable in Guideline 8's experiment.
    The \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} participants were significantly more suspicious of the \vioProduct{} (top, hatched boxplots) than of the \appProduct{} (bottom, clear boxplots). Because the change was significant ({\color{FigureMaroon}{**}}), this was an inclusivity improvement for \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} participants.
    The same was true of the \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants.\\
    x = average, \textbrokenbar~= median.
    {\color{FigureMaroon}{*}} = p<.05, {\color{FigureMaroon}{**}} = p<.01, {\color{FigureMaroon}{***}} = p<.001, NS=not significant.
%    \textbf{Right:} The differences for the risk-averse (t(25) = 3.2354, \textit{p} = .003, \textit{d} = 0.648) and risk-tolerant (t(34) = 3.0020, \textit{p} = .005, \textit{d} = 0.507) were highly significant.
    }
    \label{fig:G8-inclusivity-illustrative-example}

    \FIXME{MMB @ any table guru: can you make the 1st cell's contents align at the top of the cell instead of the bottom? or even better, the vertical center?}
\end{table}

==> tables/04-Equity-Declined.tex <==

\begin{table}[h]
    \centering
    \begin{tabular}{p{0.25\linewidth}|c|c}
         Guideline &  Violation Equity & Application Equity \\
         \toprule
         18: Notify users about changes
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/16-G18/Risk/G18-Feel-Certain-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/16-G18/Risk/G18-Feel-Certain-APPLICATION-RISK.png} 
         \\
         
         \midrule
         18: Notify users about changes
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/16-G18/Risk/G18-Feel-Productive-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/16-G18/Risk/G18-Feel-Productive-APPLICATION-RISK.png}
         \\

         \midrule
         18: Notify users about changes
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/16-G18/Risk/G18-Perceived-Useful-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/16-G18/Risk/G18-Perceived-Useful-APPLICATION-RISK.png}
         \\

         \midrule
         18: Notify users about changes
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/16-G18/Risk/G18-Not-Harmful-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/16-G18/Risk/G18-Not-Harmful-APPLICATION-RISK.png}
         \\
         
         
         

    \end{tabular}
    \caption{Examples in which equity declined between the \vioProduct{} and \appProduct{}.
    Notice that in this category, there were significant user experience inequities between the risk-averse and risk-tolerant participants in both the \vioProduct{} and \appProduct{}.
    \FIXME{MMB@AAA: I don't understand how the last sentnece can be true}
    }
    \label{tab:no-equity-declined}
\end{table}

==> tables/04-Equity-Risk-Walkthrough.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{0.25\linewidth}|c|c}
         Guideline &  Violation Equity & Application Equity\\
         \toprule
        10: Scope services when in doubt
         
        & 
        \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/09-G10/Risk/G10-Feel-Certain-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/09-G10/Risk/G10-Feel-Certain-APPLICATION-RISK.png}     
    \end{tabular}
    \caption{Equity measurements for Guideline 10's experiment for both the \vioProduct{} (left) and \appProduct{} (right).
    Notice that in both of these cases, the distance between the average feelings of adequacy for the risk-averse (top boxes) and risk-tolerant (bottom boxes) was insignificantly small, meaning that both of these products were equitable for participants with diverse attitudes toward risk.}
\FIXME{MMB @ any table guru: If we keep this all 4's, reduce that 1st column to having just 1 row in it, with "4: ..." shown only once, turned on its side. eg: https://tex.stackexchange.com/questions/201696/how-to-rotate-text-in-a-cell-and-center-it-vertically-and-horizontally}
    \label{tab:equity-no-change-example}
\end{table}

==> tables/04-G4-Inclusivity-No-Change.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{0.1\linewidth}|c|c}
        Guideline&  Risk-Averse Inclusivity & Risk-Tolerant Inclusivity\\
        \toprule
        
        \multirow{8}{*}{\rotatebox[origin=c]{90}{\parbox[c][\linewidth]{270pt}{4: Show contextually relevant information}}}
        & 
        \includegraphics[width=0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk-Within/G4-Feel-Secure-ABI-WITHIN-RISK.png}
        & 
        \includegraphics[width=0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk-Within/G4-Feel-Secure-TIM-WITHIN-RISK.png}     
        \\\cmidrule{2-3}
         
         &
         \includegraphics[width=0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk-Within/G4-Feel-Adequate-ABI-WITHIN-RISK.png}
         & 
         \includegraphics[width=0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk-Within/G4-Feel-Adequate-TIM-WITHIN-RISK.png} 
         \\\cmidrule{2-3}
          
         &
         \includegraphics[width=0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk-Within/G4-Feel-Certain-ABI-WITHIN-RISK.png}
         & 
         \includegraphics[width=0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk-Within/G4-Feel-Certain-TIM-WITHIN-RISK.png} 
         \\\cmidrule{2-3}
         
         &
         \includegraphics[width=0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk-Within/G4-Feel-Productive-ABI-WITHIN-RISK.png}
         & 
         \includegraphics[width=0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk-Within/G4-Feel-Productive-TIM-WITHIN-RISK.png} 
         \\\cmidrule{2-3}
         
         &
         \includegraphics[width=0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk-Within/G4-Perceived-Useful-ABI-WITHIN-RISK.png}
         & 
         \includegraphics[width=0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk-Within/G4-Perceived-Useful-TIM-WITHIN-RISK.png} 
         \\\cmidrule{2-3}
         
         &
         \includegraphics[width=0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk-Within/G4-Not-Harmful-ABI-WITHIN-RISK.png}
         & 
         \includegraphics[width=0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk-Within/G4-Not-Harmful-TIM-WITHIN-RISK.png} 
         \\\cmidrule{2-3}
         
         &
         \includegraphics[width=0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk-Within/G4-Product-Reliable-ABI-WITHIN-RISK.png}
         & 
         \includegraphics[width=0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk-Within/G4-Product-Reliable-TIM-WITHIN-RISK.png} 
         \\\cmidrule{2-3}
         
         &
         \includegraphics[width=0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk-Within/G4-Trust-Product-ABI-WITHIN-RISK.png}
         & 
         \includegraphics[width=0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk-Within/G4-Trust-Product-TIM-WITHIN-RISK.png} 
         \\

    \end{tabular}
    \caption{**FIXME** 
    }
\FIXME{MMB @ any table guru: If we keep this all 4's, reduce that 1st column to having just 1 row in it, with "4: ..." shown only once, turned on its side. eg: https://tex.stackexchange.com/questions/201696/how-to-rotate-text-in-a-cell-and-center-it-vertically-and-horizontally}
    \label{tab:no-inclusivity-change}
\end{table}

==> tables/04-Inclusivity-Risk-Tolerant-Only.tex <==

\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c}
         Guideline&  Risk-Averse Inclusivity & Risk-Tolerant Inclusivity\\
         \toprule
        5: Match relevant social norms
        & 
        \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/01-G1/Risk-within/G1-Feel-In-Control-ABI-WITHIN-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/01-G1/Risk-within/G1-Feel-In-Control-TIM-WITHIN-RISK.png}     
         \\
        
         \midrule
         8: Support efficient dismissal
        & 
        \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/01-G1/Risk-within/G1-Feel-Adequate-ABI-WITHIN-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/01-G1/Risk-within/G1-Feel-Adequate-TIM-WITHIN-RISK.png}     
         \\

         
         \midrule 
         9: Support efficient correction
         &
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/04-G5/Risk-within/G5-Feel-Certain-ABI-WITHIN-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/04-G5/Risk-within/G5-Feel-Certain-TIM-WITHIN-RISK.png} 
         
         \\

         \midrule
         12: Remember recent interactions
         &
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/11-G12/Risk-within/G12-Feel-Secure-ABI-WITHIN-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/11-G12/Risk-within/G12-Feel-Secure-TIM-WITHIN-RISK.png} 
         \\


         \midrule
         14: Update and adapt cautiously
         &
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/15-G17/Risk-within/G17-Not-Suspicious-ABI-WITHIN-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/15-G17/Risk-within/G17-Not-Suspicious-TIM-WITHIN-RISK.png} 
         
         \\

         \midrule
         15: Encourage granular feedback
         &
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/16-G18/Risk-within/G18-Not-Harmful-ABI-WITHIN-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/16-G18/Risk-within/G18-Not-Harmful-TIM-WITHIN-RISK.png} 
         \\
         
         
         
         

    \end{tabular}
    \caption{Across the 16 experiments, HAI-UX inclusivity significantly changed for \textit{neither} the risk-averse nor the risk-tolerant participants 45 times.
    This table provides 6 examples to highlight that this category was not an isolated incident;
    the category arose across multiple experiments and dependent variables.
    }
% \FIXME{MMB @ any table guru: If we keep this all 4's, reduce that 1st column to having just 1 row in it, with "4: ..." shown only once, turned on its side. eg: https://tex.stackexchange.com/questions/201696/how-to-rotate-text-in-a-cell-and-center-it-vertically-and-horizontally}
    \label{tab:inclusivity-risk-tolerant}
\end{table}

==> tables/04-Risk-Equity-Frequency-Table.tex <==
\begin{table}[h]
    \centering
    \includegraphics[width = 0.8\linewidth]{assets/Risk-Equity-Frequency-Table.pdf}
    \caption{A summary of where the 23 equity phenomena occurred by both guideline experiment (columns) and dependent variable (rows).
    A vast majority of the time (137/160), equity did not change between the \vioProduct{}s and \appProduct{}s.
    However, in 5 cases, the \appProduct{} fixed HAI-UX equitability (the ``+'' cells).
    In another 18 cases, the \appProduct{} was \textit{less} equitable than the \vioProduct{} (the ``-'' cells).}
    \label{tab:Risk-Equity-Frequency}
\end{table}

==> tables/05-Discussion-Inclusivity-Equity.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{cc}
         \multicolumn{2}{c}{\vioProduct{} (Risk-Averse vs. Risk-Tolerant)}  \\
         \toprule
         \multicolumn{2}{c}{\includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/07-G8/Risk/G8-Not-Suspicious-VIOLATION-RISK.png}}\\
         Risk-Averse Inclusivity & Risk-Tolerant Inclusivity\\
         \midrule
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/07-G8/Risk/G8-Not-Suspicious-ABI-WITHIN-RISK.png}
         &  \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/07-G8/Risk/G8-Not-Suspicious-TIM-WITHIN-RISK.png}
         \\
         \multicolumn{2}{c}{\appProduct{} (Risk-Averse vs. Risk-Tolerant)}  \\
         \midrule
         \multicolumn{2}{c}{\includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/07-G8/Risk/G8-Not-Suspicious-APPLICATION-RISK.png}}\\
    \end{tabular}
    \caption{A table demonstrating how changes in inclusivity can positively impact equity.
    Notice that for the \vioProduct{} (top row), the risk-averse felt significantly more suspicious than the risk-tolerant, but because \textit{both} the risk-attitudes had significantly improved HAI-UX inclusivity (middle), they felt ``equitably suspicious'' of the \appProduct{} (bottom).}
    \label{tab:discussion-inclusivity-up-equity-same}
\end{table}

==> tables/05-Discussion-Inclusivity-Reduce-Equity.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{cc}
         \multicolumn{2}{c}{\vioProduct{} (Risk-Averse vs. Risk-Tolerant)}  \\
         \toprule
         \multicolumn{2}{c}{\includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/01-G1/RISK/G1-Feel-Productive-VIOLATION-RISK.png}}\\
         Risk-Averse Inclusivity & Risk-Tolerant Inclusivity\\
         \midrule
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/01-G1/Risk-within/G1-Feel-Productive-ABI-WITHIN-RISK.png}
         &  \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/01-G1/Risk-within/G1-Feel-Productive-TIM-WITHIN-RISK.png}
         \\
         \multicolumn{2}{c}{\vioProduct{} (Risk-Averse vs. Risk-Tolerant)}  \\
         \midrule
         \multicolumn{2}{c}{\includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/01-G1/RISK/G1-Feel-Productive-APPLICATION-RISK.png}}\\
    \end{tabular}
    \caption{A table demonstrating how changes in inclusivity can \textit{negatively} impact equity.
    Notice that for the \vioProduct{} (top row), the risk-averse and risk-tolerant felt equitably certain, but because \textit{only} the risk-averse had a significantly improved HAI-UX inclusivity (middle), there was an inequity between participants' feelings of certainty with the \appProduct{} (bottom).}
    \label{tab:discussion-inclusivity-reduce-equity}
\end{table}

==> tables/05-Equity-Improved.tex <==

\begin{table}[h]
    \centering
    \begin{tabular}{p{0.25\linewidth}|c|c}
         Guideline&  Risk-Averse Inclusivity & Risk-Tolerant Inclusivity\\
         \toprule
        6: Mitigate social biases %adequate
        & 
        \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/05-G6/Risk/G6-Feel-Adequate-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/05-G6/Risk/G6-Feel-Adequate-APPLICATION-RISK.png}     
         \\
        
         \midrule
         4: Show contextually relevant information %productive
        & 
        \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Feel-Productive-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Feel-Productive-APPLICATION-RISK.png}     
         \\

         
         \midrule 
         7: Support efficient invocation %control
         &
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/06-G7/Risk/G7-Feel-In-Control-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/06-G7/Risk/G7-Feel-In-Control-APPLICATION-RISK.png} 
         \\


         \midrule
         8: support efficient dismissal %suspicious
         &
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/07-G8/Risk/G8-Not-Suspicious-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/07-G8/Risk/G8-Not-Suspicious-APPLICATION-RISK.png} 
         
         \\

         \midrule
         14: update and adapt cautiously %certain
         &
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/13-G14/Risk/G14-Feel-Certain-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/13-G14/Risk/G14-Feel-Certain-APPLICATION-RISK.png} 
         \\
         
         
         
         

    \end{tabular}
    \caption{The HAI-UX equity improved between the \vioProduct{} and \appProduct{} for participants with diverse attitudes toward risk five times across 5 separate experiments and dependent variables.
    This table shows all five examples of this category.
    }
% \FIXME{MMB @ any table guru: If we keep this all 4's, reduce that 1st column to having just 1 row in it, with "4: ..." shown only once, turned on its side. eg: https://tex.stackexchange.com/questions/201696/how-to-rotate-text-in-a-cell-and-center-it-vertically-and-horizontally}
    \label{tab:equity-improved-general}
\end{table}

==> tables/05-Learn-Info-Inclusivity-Summary.tex <==
\begin{table}[h!]
\centering
    \begin{tabular}{c|c}

         Learning Style & Motivations \\
         \hline
         \includegraphics[width = 0.4\linewidth]{assets/Learn-Inclusivity-Frequency-Table.pdf} &  
        \includegraphics[width = 0.4\linewidth]{assets/Motiv-Inclusivity-Frequency-Table.pdf}\\
        
        
        Information Processing Style  & Computer Self-Efficacy\\
        \hline
        \includegraphics[width = 0.4\linewidth]{assets/Info-Inclusivity-Frequency-Table.pdf} & 
         \includegraphics[width = 0.4\linewidth]{assets/SE-Inclusivity-Frequency-Table.pdf}\\
         
    \end{tabular}  
    \caption{Thumbnails of summary similar to Table~\ref{tab:Risk-Inclusivity-Frequency}, but for the other four problem-solving styles.
    In the majority of cases, both the ``Abi''-like and ``Tim''-like participants' HAI-UX inclusivity improved, and there were only six inclusivity losses across these four problem-solving styles, all of which occurred in Guideline 4's experiment.
    }
    \label{tab:Learn-Info-Inclusivity-Frequency}
%    \FIXME{%MMB@AAA: these totals don't match various totals in text, which also don't agree with each other.  All of these numbers need to REALLY CAREFULLY checked (in figs AND in tables AND in captions AND in text for agreement.\\
%    MMB: morning 8/2, numeric discrepancies resolved, yay!}
\end{table}

==> tables/06-Everyone-Else.tex <==
\begin{table}[h]
        \centering
        \includegraphics[width = 0.4\linewidth]{assets/Inclusivity-Everyone-Else.pdf}
    \caption{}
    \label{tab:inclusivity-everyone-else}
\end{table}
\begin{table}[h]
        \centering
        \includegraphics[width = 0.4\linewidth]{assets/Equity-Everyone-Else.pdf}
    \caption{}
    \label{tab:equity-everyone-else}
\end{table}


==> tables/06-Risk-Gender-Comparison.tex <==

\begin{table}[h]
    \centering
    \begin{tabular}{l|c|c}
         Guideline&  Risk-Averse Inclusivity & Risk-Tolerant Inclusivity \\
         \toprule
         
        8: Support efficient dismissal
        &
        \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/07-G8/Risk/G8-Not-Suspicious-ABI-WITHIN-RISK.png} 
        &
        \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/07-G8/Risk/G8-Not-Suspicious-TIM-WITHIN-RISK.png}
         
         
         

    \end{tabular}
    \caption{The same fInclusivity gains: A few examples of the 75 times inclusivity improved for both \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} and \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants.
    E.g., in Guideline~8's experiment (second row), both the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} and the \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants were significantly more suspicious of the \vioProduct{} (top, hatched boxplots) than of the \appProduct{} (bottom, clear boxplots). 
%    The 3 rows help illustrate the breadth of these 75 occurrences (many different experiments and many different dependent variables), and also give visual close-ups of a few such distributions.
%    Every significant result ({\color{FigureMaroon}{*}}, {\color{FigureMaroon}{**}}, or {\color{FigureMaroon}{***}}) adheres to our definition of an inclusivity improvement.
    x = average, \textbrokenbar~= median.
    {\color{FigureMaroon}{*}} = p<.05, {\color{FigureMaroon}{**}} = p<.01, {\color{FigureMaroon}{***}} = p<.001, NS=not significant.
    % * = $p \in [0.01, 0.05]$, ** = $p \in [.001, .01)$, *** = $p < .001$
    }
    \label{tab:risk-gender-comparison}

    \FIXME{MMB @ any table guru: can we VERTICALLY center the guidelines?}
\end{table}



==> tables/10-Triangulation-Over-Facets.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width = 0.27\linewidth]{assets/05-All-BoxPlots/00-Legends/SE-Legend.pdf}
    \includegraphics[width = 0.17\linewidth]{assets/05-All-BoxPlots/01-G1/SE/G1-Feel-Adequate-SE.png}
    \caption{Guideline 1 - Participants' scores by computer self-efficacy for the ``Feel Adequate'' dependent variable.
    Notice that for both the Violation and the Application, the participants who had \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{lower self-efficacy} relative to their peers felt significantly less adequate, suggesting that something might not be meeting their needs when making clear what the system can do.}
    \label{fig:self-efficacy}
\end{figure}


%G1-SE --Done
%G6, Learn -- Done
%G12-Motiv -- Done
%G15, just Info

==> tables/11-When-Wrong-DVs.tex <==
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{p{0.46\linewidth}|p{0.22\linewidth}|c}
         \textbf{Guideline Name (G\#)} & \textbf{Dependent Variable} & \textbf{Application/Violation}  \\
         \hline
        Support efficient invocation (G7) &
        \cellcolor{TimBlueQuote}{Feel In Control} & Application \\
        \hline
         & \cellcolor{TimBlueQuote}{{Feel In Control}} & Application \\
         & \cellcolor{TimBlueQuote}{{Feel Adequate}} & Application \\
         Support efficient dismissal (G8) & \cellcolor{TimBlueQuote}{{Product Useful}} & Application \\
         & \cellcolor{TimBlueQuote}{{Product Reliable}} & Application\\
         & \cellcolor{TimBlueQuote}{{Trust Product}} & Violation \\
        \hline
        Scope services when in doubt (G10) & \cellcolor{TimBlueQuote}{{Not Harmful}} & Application \\
        \hline
        Make clear why the system did what it did (G11) & \cellcolor{TimBlueQuote}{{Feel Adequate}} & Violation \\
        \hline
    \end{tabular}
    \caption{Information processing style: Dependent variables in the  \colorboxBackgroundForegroundText{WhenWrongYellow}{black}{{When Wrong}} phase for which the \colorboxBackgroundForegroundText{TimBlueQuote}{black}{{selective}} information processors rated the system significantly lower than the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{{comprehensive}} information processors did.
    There was no immediately identifiable pattern between the phase and the impacted dependent variables, suggesting the need for further research.}
    \label{tab:when_wrong_dvs}
\end{table}

==> tables/12-One-More-Than-Other.tex <==
\begin{landscape}
\begin{figure}[h]
\footnotesize
    \centering
    
    \begin{tabular}{ll|ll|ll|ll|ll|ll|ll|ll}

    
        \multicolumn{2}{c|}{\includegraphics[width = 0.10\linewidth]{assets/G4-Card.pdf}} 
         &
         \multicolumn{2}{c|}{\includegraphics[width = 0.10\linewidth]{assets/G5-Card.pdf}} 
         &
         \multicolumn{2}{c|}{\includegraphics[width = 0.10\linewidth]{assets/G9-Card.pdf}} 
         & 
         \multicolumn{2}{c|}{\includegraphics[width = 0.10\linewidth]{assets/G10-Card.pdf}}
         & 
         \multicolumn{2}{c|}{\includegraphics[width = 0.10\linewidth]{assets/G11-Card.pdf}}
         &
         \multicolumn{2}{c|}{\includegraphics[width = 0.10\linewidth]{assets/G13-Card.pdf}}
         & 
         \multicolumn{2}{c|}{\includegraphics[width = 0.10\linewidth]{assets/G15-Card.pdf}}
         & 
         \multicolumn{2}{c}{\includegraphics[width = 0.10\linewidth]{assets/G18-Card.pdf}}
          \\
         
         %\hline
        
        \multicolumn{2}{l|}{\includegraphics[width = 0.10\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Perceived-Useful-RISK.png}}
         &
         \multicolumn{2}{l|}{\includegraphics[width = 0.10\linewidth]{assets/05-All-BoxPlots/04-G5/Risk/G5-Feel-Adequate-RISK.png}}
         &
         \multicolumn{2}{l|}{\includegraphics[width = 0.10\linewidth]{assets/05-All-BoxPlots/08-G9/Risk/G9-Perceived-Useful-RISK.png}}
         &
         \multicolumn{2}{l|}{\includegraphics[width = 0.10\linewidth]{assets/05-All-BoxPlots/09-G10/Risk/G10-Perceived-Useful-RISK.png}}
         
         &
         
         \multicolumn{2}{l|}{\includegraphics[width = 0.10\linewidth]{assets/05-All-BoxPlots/10-G11/Risk/G11-Feel-Adequate-RISK.png}}
         
         &
         
         \multicolumn{2}{l|}{\includegraphics[width = 0.10\linewidth]{assets/05-All-BoxPlots/12-G13/Risk/G13-Feel-Adequate-RISK.png}}
        &
        \multicolumn{2}{l|}{\includegraphics[width = 0.10\linewidth]{assets/05-All-BoxPlots/14-G15/Risk/G15-Feel-Adequate-RISK.png}}
        &
        
        \multicolumn{2}{l}{\includegraphics[width = 0.10\linewidth]{assets/05-All-BoxPlots/16-G18/Risk/G18-Perceived-Useful-RISK.png}}

        
         
        \\
        \multicolumn{2}{l|}{t(63) = -2.9810} & 
        \multicolumn{2}{l|}{t(67) = -2.0600} & 
         \multicolumn{2}{l|}{t(56) = -2.2058} & 
         \multicolumn{2}{l|}{t(62) = 2.13524} & 
         \multicolumn{2}{l|}{t(61) = -2.1964} &
         \multicolumn{2}{l|}{t(55) = -3.2194} &
         \multicolumn{2}{l|}{t(62) = -2.0013} &
         \multicolumn{2}{l}{t(64) = -2.8148} \\
         \textit{p}: .0040 & \textit{d}: .744 &
         \textit{p}: .0433 & \textit{d}: .497 &
         \textit{p}: .0320 & \textit{d}: .582 &
         \textit{p}: .0350 & \textit{d}: .539 &
         \textit{p}: .0320  & \textit{d}: .554 &
         \textit{p}: .0020 & \textit{d}: .854  &
         \textit{p}: .0497 & \textit{d}: .503  &
         \textit{p}:  .0060 & \textit{d}: .694\\
         
        %  &&&&&&&&&&&&\\
        
        % &&
        % &&
        % \multicolumn{2}{l|}{\includegraphics[width = 0.10\linewidth]{assets/05-All-BoxPlots/08-G9/Risk/G9-Feel-Productive-RISK.png}}
        
        %  &
         
        %  \multicolumn{2}{l|}{\includegraphics[width = 0.10\linewidth]{assets/05-All-BoxPlots/09-G10/Risk/G10-Product-Reliable-RISK.png}}
         
        %  &
         
         
         
        %  &
         
        %  \multicolumn{2}{l|}{\includegraphics[width = 0.10\linewidth]{assets/05-All-BoxPlots/16-G18/Risk/G18-Feel-Certain-RISK.png}}\\
        %   &&
        %   &&
        %   \multicolumn{2}{l|}{t(56) = -2.1404} & 
        %   \multicolumn{2}{l|}{t(61) = 2.4183} & 
        %   \multicolumn{2}{l|}{t(55) = -3.2194}& 
        %   \multicolumn{2}{l|}{t(65) = -2.0253}  & 
        %   \\
        %   &&
        %   &&
        %  \textit{p}: .037 & \textit{d}: .565  &
        %  \textit{p}: .019 & \textit{d}: .611  &
        %  \textit{p}: .002 & \textit{d}: .854 &
        %  \textit{p}: .032  & \textit{d}:.495 &
        %  &\\
         
         
    \end{tabular}
    \caption{Examples of dependent variables from all experiments where participants on one end of the risk spectrum was helped by the \appProduct{} \textit{more} than the other participants.
    This disparity resulted in a \applicationBox{significant difference between the means}.
    In 7 of these 8 examples, the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} participants rated the product  significantly lower than the \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants did.}
    \label{tab:one_helped_more}
    \vspace{0pt}
\end{figure}
\end{landscape}

==> tables/13-Only-One-Helped.tex <==
\begin{wrapfigure}{o}{.5\linewidth}
    \centering
    \begin{tabular}{cccc}
         \multicolumn{4}{c}{Guideline 18} \\

         
         
         \multicolumn{2}{c}{\includegraphics[width = 0.15\linewidth]{assets/05-All-BoxPlots/16-G18/Risk/G18-Feel-Productive-RISK.png}}
         & 
         \multicolumn{2}{c}{\includegraphics[width = 0.15\linewidth]{assets/05-All-BoxPlots/16-G18/Risk/G18-Not-Harmful-RISK.png}}\\
         \hline

         \multicolumn{2}{c}{t() = } & 
         \multicolumn{2}{c}{t() = }\\

         \textit{p}:  & \textit{d}:  &
         \textit{p}:  & \textit{d}: \\
         
         
    \end{tabular}
    \caption{All dependent variables from Guideline 18 where the \colorboxBackgroundForegroundText{TimBlueQuote}{black}{risk-tolerant} participants were helped by the Application product, yet the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} were unsupported.
     }
    \label{tab:only_one_helped}
\end{wrapfigure}

==> tables/15-Applications-Improved-Equity.tex <==

\begin{table}[h]
    \centering
    \begin{tabular}{c|cc|c}
         Guideline&  Violation Equity & Application Equity & Inclusiveness Change \\
         \toprule
         7: Support efficient invocation 
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/06-G7/Risk/G7-Feel-In-Control-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/06-G7/Risk/G7-Feel-In-Control-APPLICATION-RISK-App.png} & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/06-G7/Risk/G7-Control-RISK-Diff.pdf}\\
         
         \midrule
         8: Support Efficient Dismissal & \includegraphics[width = 0.25\linewidth]{assets/01-Risk-Example/Risk-Vio-Example.png} & \includegraphics[width = 0.25\linewidth]{assets/01-Risk-Example/Risk-App-Example.png}
         & \includegraphics[width = 0.25\linewidth]{assets/01-Risk-Example/G8-Suspicious-RISK-Diff.pdf}\\
        
         \midrule
         11: Make clear why the system... 
         &
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/10-G11/Risk/G11-Feel-In-Control-VIOLATION-RISK.png} 
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/10-G11/Risk/G11-Feel-In-Control-APPLICATION-RISK-App.png}
         &
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/10-G11/Risk/G11-Control-RISK-Diff.pdf}
         
         \\
         

    \end{tabular}
    \caption{Examples of the first user experience equity and inclusiveness pattern from these data.
    Notice how the significant inequities from the \vioProduct{} (middle column, left) were no longer significant in the \appProduct{} (middle column, right), fitting the definition of this pattern.
    Further, notice that the inclusiveness change (right) tended to benefit either the risk-averse or risk-tolerant more, which helps explain why the inequities disappeared.}
    \label{tab:inclusivity-improves}
\end{table}


==> tables/16-Inequities-Remain.tex <==

\begin{table}[h]
    \centering
    \begin{tabular}{p{0.25\linewidth}|c|c}
         Guideline &  Violation Equity & Application Equity \\
         \toprule
         4: Show contextually relevant information 
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Feel-Secure-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Feel-Secure-APPLICATION-RISK.png} 
         \\
         
         \midrule
         4: Show contextually relevant information & \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Feel-Adequate-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Feel-Adequate-APPLICATION-RISK.png}  
         \\
        
         \midrule
         4: Show contextually relevant information 
         &
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Feel-Certain-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Feel-Certain-APPLICATION-RISK.png} 
         \\

         \midrule
         4: Show contextually relevant information 
         &
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Not-Suspicious-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Not-Suspicious-APPLICATION-RISK.png} 
         \\

        \midrule
         4: Show contextually relevant information 
         &
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Not-Harmful-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Not-Harmful-APPLICATION-RISK.png}  
         \\

         \midrule
         4: Show contextually relevant information 
         &
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Product-Reliable-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Product-Reliable-APPLICATION-RISK.png} 
         \\

         \midrule
         4: Show contextually relevant information 
         &
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Trust-Product-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/03-G4/Risk/G4-Trust-Product-APPLICATION-RISK.png} 
         \\
         
         
         

    \end{tabular}
    \caption{Seven examples of the third equity category from Guideline 4's experiment.
    Notice that in this category, there were significant user experience inequities between the risk-averse and risk-tolerant participants in both the \vioProduct{} and \appProduct{}.
    }
    \label{tab:no-equity-change-G4}
\end{table}

==> tables/17-Demographics.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{0.15\linewidth}|p{0.4\linewidth}|p{0.06\linewidth}}
        Demographic & Category & Count\\
        \hline
        \multirow{6}{0.15\linewidth}{Age} & 18---24 years old & 125  \\
         & 25---34 years old & 422 \\
         & 35---44 years old & 259 \\
         & 45---54 years old & 138 \\
         & 55---64 years old & 58 \\
         & 65---74 years old & 14 \\
         \hline
         \multirow{7}{0.15\linewidth}{Gender} & Woman & 527 \\
         & Man & 478 \\
         & Non-Binary & 12 \\
         & Transgender & 4 \\
         & Gender Non-conforming & 2 \\
         & Declined to report & 2 \\
         & Intersex & 1 \\
         \hline
         \multirow{7}{0.15\linewidth}{Education} & Bachelors degree & 430 \\
         & Some college (no degree) & 199 \\
         & Advanced degree (MA/MS/Ph.D./M.D.) & 162 \\
         & Associates degree & 112 \\
         & At most high school & 91 \\
         & Trade/technical school & 22 \\
         \hline
         \multirow{29}{0.15\linewidth}{Employment Field} & Science/Technology/Programming & 176  \\
         & Education & 113 \\
         & Unemployed/other & 97 \\
         & Sales/Marketing & 83 \\
         & Administration/Clerical/Reception & 80 \\
         & Health care (Physical \& Mental ) & 66 \\
         & Customer service & 48 \\
         & Management (Senior/Corporate) & 42 \\
         & Arts/Leisure/Entertainment & 37 \\
         &  Operations/Logistics & 34 \\
         & Homemaker & 25 \\
         & Student & 24 \\
         & Restaurant/Food service & 24 \\
         & Construction & 23 \\
         & Social service & 21 \\
         & HR Management & 17 \\
         & Consulting & 17 \\
         & Real Estate & 15 \\
         & Production & 14 \\
         & Research & 11 \\
         & Distribution & 9 \\
         & News/Information & 9 \\
         & Advertisement/PR & 8 \\
         & Architecture/Design & 8 \\
         & Retired & 8 \\
         & Beauty/Fashion & 3\\
         & Planning (meeting, events, etc.) & 2 \\
         & Buying/Purchasing & 2 \\
         
    \end{tabular}
    \caption{Counts of participants by Age, Gender, Education, and Employment Field.}
    \label{tab:demographics}
\end{table}

==> tables/17-Equities-Form.tex <==

\begin{table}[h]
    \centering
    \begin{tabular}{c|cc|c}
         Guideline&  Violation Equity & Application Equity & Inclusiveness Change \\
         \toprule
         9: Support efficient correction 
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/08-G9/Risk/G9-Feel-Productive-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/08-G9/Risk/G9-Feel-Productive-APPLICATION-RISK-App.png} 
         & 
         \includegraphics[width = 0.25\linewidth]{}
         \\
         
         \midrule

         9: Support efficient correction 
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/08-G9/Risk/G9-Perceived-Useful-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/08-G9/Risk/G9-Perceived-Useful-APPLICATION-RISK-App.png} 
         & 
         \includegraphics[width = 0.25\linewidth]{}
         \\
         
         \midrule

         10: Scope services...
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/09-G10/Risk/G10-Product-Reliable-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/09-G10/Risk/G10-Product-Reliable-APPLICATION-RISK-App.png} 
         & 
         \includegraphics[width = 0.25\linewidth]{}
         \\
         
         \midrule

         13: Learn from user behavior
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/12-G13/Risk/G13-Perceived-Useful-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/12-G13/Risk/G13-Perceived-Useful-APPLICATION-RISK-App.png} 
         & 
         \includegraphics[width = 0.25\linewidth]{}
         \\
         
         \bottomrule

         1: Make clear what the system can do
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/01-G1/RISK/G1-Feel-Productive-VIOLATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{assets/05-All-BoxPlots/01-G1/RISK/G1-Feel-Productive-APPLICATION-RISK.png}
         & 
         \includegraphics[width = 0.25\linewidth]{}
         \\
         
         \\
         
         
         

    \end{tabular}
    \caption{**FIXME**
    Notice that in this pattern, there were \textit{no} significant user experience inequities between the risk-averse and risk-tolerant participants in the \vioProduct{}.
    However, an inequity formed between these participants with the \appProduct{}.
    The inclusiveness changes help to make sense of this.
    **FIXME**
    }
    \label{tab:equities-form}
\end{table}

==> tables/2-Facet-to-Persona-Reminder.tex <==
\begin{table}[h]
\centering

\includegraphics[width = 0.5\columnwidth]{assets/GM-Table.pdf}



% \end{tabular}
\vspace{5pt}
    \caption{The same five GenderMag problem-solving style types (rows) from, each type's range of possible values, and the set of values for each.
    We consider participants to be more \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{``Abi''-like} if their values for any type were from the left column.
    Similarly, we consider participants to be more \colorboxBackgroundForegroundText{TimBlueQuote}{black}{``Tim''-like} if their values were from the right column.}
    
    % \FIXME{MMB to all: *never* list only two personas for GenderMag. Not in tables, not in figures, not in text talking about GM's personas, .... Doing so shouts "binary" to too many readers. Always include all three.}
    \label{table:personas-reminder}
\end{table}

% \FIXME{Abi - Orange, Tim - Blue, Pat - light-grey \\
% MMB adds: In this table, please make Abi's and Tim's colors more washed out (eg, adjust the colors to have a lot more white in them.  Much like the colors in the paper you got these from.  (But the colors in the boxplots themselves are fine, don't change them. }

==> tables/4-Triangulation-table.tex <==
\begin{table}[h]
\vspace{-18pt}
 \includegraphics[width = \linewidth]{assets/Triangulation-Table.pdf}
    \caption{Each letter represents one of the inclusivity patterns from Section~\ref{subsec:3-categories}: Pattern \#1 showed when guidelines \underline{c}losed inclusivity gaps (C) in Section~\ref{subsec:category-1}, Pattern \#2 showed instances where those who have diverse problem solving style values received \underline{v}arying degrees of help (V) in Section~\ref{subsec:category-2}, and Pattern \#3 showed instances of \underline{p}ersistent gaps (P) from Section~\ref{sec:category-3}.
    The colors show who had the significantly lower average---the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{``Abi''-like} or \colorboxBackgroundForegroundText{TimBlueQuote}{black}{``Tim''-like} participants (Table~\ref{table:personas}).
    In total, disaggregating by the five problem solving style types revealed 112 instances of the three patterns in 15 of the 16 experiments.
    The ``Abi''-like participants had the significantly lower average in 95 of them.\\
    \textbf{Row-wise:} The patterns were triangulated by at least 8 instances (Motivations, 2nd row) for every problem solving style type.\\
    \textbf{Column-wise: } The patterns were triangulated by at least 2 instances in multiple experiments.
   % Notice that the least prevalent problem solving style (Motivations) still uncovered 8 inclusivity insights across 6 experiments, whereas the most prevalent (Attitudes toward Risk) uncovered 34 insights across 11 experiments.
   }
    \label{tab:triangulation-table}


\end{table}

==> tables/5-Man-Woman-Contingency.tex <==
\begin{table}[h]
%\framebox[\linewidth]{For Measuring!}
        \centering
        \footnotesize
        \begin{tabular}{c||cc}
          & 3 or more           &   less than 3 \\
          & ``Abi''-like styles & ``Abi''-like styles \\
         \toprule
         \cellcolor{WomanOrange}{\color{black}Woman}  & \cellcolor{white}277 & 249\\
         
         \cellcolor{ManBlue}{\color{white}Man} & 173 & 302 \\
         \bottomrule
         \cellcolor{white}Estimate (\textit{k}) & \multicolumn{2}{c}{236}\\
         \midrule
         \cellcolor{white}\textit{p}-value & \multicolumn{2}{c}{$< .0001$}\\

    \end{tabular}
        
        \caption{The 2x2 contingency table used for Fisher's exact test, represented in Figure~\ref{fig:anderson-facet-gender}, to investigate the counts of men and women who exhibit a majority (i.e., 3 or more) of the ``Abi'' problem solving styles from Table~\ref{table:personas}.
        Fisher's exact test statistic ($k$) is the estimated value of the top-left cell, calculated by $R_1(C_1)/T$, where $R_1$ \& $C_1$ are the first row and column totals respectively, and $T$ is the table total. The difference is highly significant.}
        \label{tab:Fisher-1}
\end{table}

==> tables/6-GM-Rules.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{0.3\linewidth}|c|c|c}
%         & \textbf{Inequality:} &  &  \\
       \textbf{problem solving style} & \textbf{Comparison} & \textbf{If True: } &\textbf{If False: }\\
       \hline
        Attitudes Toward Risk & $>$ median & \cellcolor{AbiOrangeQuote} more risk-averse & \cellcolor{TimBlueQuote} more risk-tolerant \\
        \hline
        Computer Self-Efficacy & $<$ median & \cellcolor{AbiOrangeQuote} lower & \cellcolor{TimBlueQuote} higher \\
        \hline
        Information Processing Style & $>$ median & \cellcolor{AbiOrangeQuote} more comprehensive & \cellcolor{TimBlueQuote} more selective \\
        \hline
        Motivations & $<$ median & \cellcolor{AbiOrangeQuote} more for task & \cellcolor{TimBlueQuote} more for fun \\
        \hline
        Learning Style & $<$ median & \cellcolor{AbiOrangeQuote} more by process & \cellcolor{TimBlueQuote} more by tinkering \\
    \end{tabular}
    \caption{The rules for each problem solving style spectrum, used to categorize which style participants exhibited from their survey responses, relative to other participants.}
    \label{tab:style_rules}
\end{table}

==> tables/7-Age-Facet-Contingency.tex <==
\begin{table}[h]
%\framebox[\linewidth]{For Measuring!}
        \centering
        \footnotesize
 %       \begin{tabular}{c||c|c||c|c||c|c||c|c||c|c}
        \begin{tabular}{c||cc||cc||cc||cc||cc}
         & \multicolumn{2}{c||}{18 -- 24} & \multicolumn{2}{c||}{25 -- 34} & \multicolumn{2}{c}{35 -- 44} & \multicolumn{2}{c}{45 -- 54} & \multicolumn{2}{c}{55 -- 64}\\
         % \cmidrule{2-3}  \cmidrule{5-6}  \cmidrule{8-9}  \cmidrule{11-12}  \cmidrule{14-15}
         
          & $\geq 3$  & $< 3$ & $\geq 3$  & $< 3$ & $\geq 3$  & $< 3$ & $\geq 3$  & $< 3$ & $\geq 3$  & $< 3$ \\
         \toprule
         \cellcolor{WomanOrange}{\color{black}Woman}  & 25 & 36 &  101 & 97 &  77 & 70 & 47 & 29 & 23 & 13 \\
         % \cmidrule{2-3}  \cmidrule{5-6}  \cmidrule{8-9}  \cmidrule{11-12}  \cmidrule{14-15}
         \cellcolor{ManBlue}{\color{white}Man}  & 19 & 40 & 77 & 142 & 37 & 71 & 23  & 38  & 12 & 10\\
         % \cmidrule{2-3}  \cmidrule{5-6}  \cmidrule{8-9}  \cmidrule{11-12}  \cmidrule{14-15}
         \midrule
         \cellcolor{white} Estimate (\textit{k}) & \multicolumn{2}{c||}{22} & \multicolumn{2}{c||}{85} & \multicolumn{2}{c||}{66} & \multicolumn{2}{c||}{39} & \multicolumn{2}{c}{22}\\
         % \cmidrule{2-3}  \cmidrule{5-6}  \cmidrule{8-9}  \cmidrule{11-12}  \cmidrule{14-15}
         \midrule
         \textit{p}-value & \multicolumn{2}{c||}{\cellcolor{white}.3482} & \multicolumn{2}{c||}{.0015*} & \multicolumn{2}{c||}{.0050*} & \multicolumn{2}{c||}{.0061*} & \multicolumn{2}{c}{\cellcolor{white}.5831}\\

    \end{tabular}
        
        \caption{The 2x2 contingency tables of each age group's number of participants, divided between whether they had three or more ``Abi''-like problem solving styles or not.
        The middle three age group categories had significant gender differences (Fisher's exact test).}
        \label{tab:fisher-ages}
\end{table}
 



==> tables/By-Phase-Applications-Table.tex <==
\begin{table}[h]
\centering

\includegraphics[width = 0.9\linewidth]{assets/Summary-Table.pdf}
%\includegraphics[width = 0.9\linewidth]{assets/Triangulation-Table-OLD.pdf}
    
    \caption{Summary of all 16 experiments (Figure~\ref{fig:human-AI-guidelines}), showing which of guidelines (G\#) had dependent variables exhibiting each of the three categories (columns) over the five problem solving styles (rows) from Table~\ref{table:personas}.
%    The ``Initially'' phase contains Guideline 1, ``During Interaction'' contains Guidelines 3--6, ``When Wrong contains Guidelines 7--11, and ``Over Time'' contains Guidelines 12--18. 
    The colors in the cells reflect which problem solving style had significantly lower average ratings for the AI products for that G\#:  the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{``Abi''-like} or the \colorboxBackgroundForegroundText{TimBlueQuote}{black}{``Tim''-like}) style.
     }
    \label{tab:summary-table}
    % \FIXME{MMB@AAA: Reader is wondering why risk averse is the same color as lower SE is the same as ....  Can you explain in 1 sentence by referring back to something in the GenderMag Background section?\\
    % AAA@MMB: Done!}
    
    % \FIXME{MMB@AAA: coauthor is wondering where the source for these graphics are, so that I can tint the Red such that it doesn't clash so much with the color scheme we're using in the paper  (for this Table and all the other tables that are using this Red). Not obvious where in our directory, so please give not only the FILENAME and URL but also the FOLDERNAME, in case names change or files get replaced. (P.S., are you by any chance a bit color-blind?)}
  
\end{table}

==> tables/By-Phase-Violations-Table.tex <==
\begin{table}[h]

    
    % \FIXME{MMB to all: *never* list only two personas for GenderMag. Not in tables, not in figures, not in text talking about GM's personas, .... Doing so shouts "binary" to too many readers. Always include all three.}
    
    \label{table:phase-application-insight}
    
        \begin{tabular}{p{0.15\linewidth}|c|c|c|c}
    
    \rowcolor{LightCyan}
    \multicolumn{5}{c}{Guideline Violation Means Significantly Different}\\
    \rowcolor{LightCyan}
    \multicolumn{5}{c}{(Color $\implies$ average \textit{higher})}\\
    \hline
    
         & & \textbf{During} & \textbf{When} & \textbf{Over} \\
         
         & \textbf{Initially} & \textbf{Interaction} & \textbf{Wrong} & \textbf{Time} \\
        
        & \textbf{(1)} & \textbf{(4)} & \textbf{(5)} & \textbf{(6)}\\
        \hline
        \hline
        
         Risk & & \colorboxBackgroundForegroundText{TimBlue}{black}{4, 6} &
         \colorboxBackgroundForegroundText{AbiOrange}{black}{7}\ \colorboxBackgroundForegroundText{TimBlue}{black}{8, 11} &
         \colorboxBackgroundForegroundText{TimBlue}{black}{13, 14, 18}\\
         
         \hline
         
         Self-Efficacy & 
         %Initially
         \colorboxBackgroundForegroundText{TimBlue}{black}{1} &
         %During Interaction
         \colorboxBackgroundForegroundText{TimBlue}{black}{4} &
         %When Wrong
         \colorboxBackgroundForegroundText{TimBlue}{black}{10} &
         %Over Time
         \colorboxBackgroundForegroundText{TimBlue}{black}{13, 18}\\
         
         \hline
         
         Information Processing & 
         %Initially
         &
         %During Interaction
         \colorboxBackgroundForegroundText{TimBlue}{black}{4} &
         %When Wrong
          &
         %Over Time
        \colorboxBackgroundForegroundText{TimBlue}{black}{13, 15} \\
         \hline
         
         Motivations & 
         %Initially
         
          & 
         %During Interaction
          \colorboxBackgroundForegroundText{TimBlue}{black}{5, 6}&
         %When Wrong
          &
         %Over Time
         \colorboxBackgroundForegroundText{TimBlue}{black}{13}\\
         \hline
         
         Learning Style & 
         %Initially
          & 
         %During Interaction
         \colorboxBackgroundForegroundText{AbiOrange}{black}{3}\  \colorboxBackgroundForegroundText{TimBlue}{black}{4, 6}&
         %When Wrong
          &
         %Over Time
         \colorboxBackgroundForegroundText{TimBlue}{black}{13, 14, 18}
         \\
         
         
         
    \end{tabular}
    
   \caption{Table showing which guidelines (numbers) demonstrated significant distances between the means of the \textit{violation} vignettes for each of the problem solving styles (rows) and which phase (columns).
    From Amershi et al.~\cite{amershi2019guidelines}, Guidelines 1 \& 2 are in the ``Initially'' phase, 3 -- 6 are ``During Interaction'', 7 - 11 are ``When Wrong'', and 12 -- 18 are ``Over Time''.  }
    \label{tab:by-phase-violation-diff}

    
\end{table}



==> tables/Discussion-Tables/01-G8-Recollection.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{0.25\linewidth}|c|c}
         Guideline&  Risk-Averse Inclusivity & Risk-Tolerant Inclusivity \\
         \toprule
         \parbox[c]{\linewidth}{8: Support efficient dismissal}
         &
         \parbox[c]{0.25\linewidth}{
         \includegraphics[width = \linewidth]{assets/05-All-BoxPlots/07-G8/Risk/G8-Not-Suspicious-ABI-WITHIN-RISK.png}}
         &
         \parbox[c]{0.25\linewidth}{
         \includegraphics[width = \linewidth]{assets/05-All-BoxPlots/07-G8/Risk/G8-Not-Suspicious-TIM-WITHIN-RISK.png}}\\
         \midrule
         \parbox[c]{\linewidth}{8: Support efficient dismissal}
         &
         \parbox[c]{0.25\linewidth}{
         \includegraphics[width =\linewidth]{assets/05-All-BoxPlots/07-G8/Risk/G8-Not-Suspicious-VIOLATION-RISK.png}}
         &
         \parbox[c]{0.25\linewidth}{
         \includegraphics[width = \linewidth]{assets/05-All-BoxPlots/07-G8/Risk/G8-Not-Suspicious-APPLICATION-RISK.png}}\\
         
         
         

    \end{tabular}
    \caption{**FIXETH ME**
    }
    \label{tab:G8-Recollection}

    \FIXME{MMB @ any table guru: can we VERTICALLY center the guidelines?}
\end{table}



==> tables/Learning/1-Learn-G1.tex <==
\begin{table}[h]
\centering

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}

Facet Value &	       F1 &	F2 &   F3 &	  F4 &	 F5 &	PU &   T1 &	 T2 &    T3 &	T4 \\
\hline
``Process'' & .012 & .041* & .015 & .003 & .027* & .013 & .016 & .000 & .009 & .000 \\
\hline
``Tinker''     & .004 & .013 & .004 & .040* & .019 & .017 & .000 & .008 & .021* & .006 \\



\end{tabular}

    \caption{The eta squared effect size for each of the 10 dependent variables for both ends of the Learning Style spectrum.}
    
    \label{table:gender-facets}
\end{table}

==> tables/Learning/2-Learn-G3.tex <==
\begin{table}[h]
\centering

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}

Facet Value &	       F1 &	F2 &   F3 &	  F4 &	 F5 &	PU &   T1 &	 T2 &    T3 &	T4 \\
\hline
``Process'' & .086* & .007 & .019 & .018 & .089* & .045* & .000 & .006 & .036* & .000 \\
\hline
``Tinker''     & .221** & .091* & .066* & .095* & .172** & .095* & .009 & .015 & .044* & .079* \\
\hline 
``Overall'' & .159** & .038* & .041* & .054* & .130** & .069* & .002 & .001 & .040* & .024*\\



\end{tabular}

    \caption{The eta squared ($\eta^2$) effect size for each of the 10 dependent variables for both ends of the Learning Style  spectrum.}
    
    \label{table:gender-facets}
\end{table}

==> tables/Learning/3-Learn-G4.tex <==
\begin{table}[h]
\centering

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}

Facet Value &	       F1 &	F2 &   F3 &	  F4 &	 F5 &	PU &   T1 &	 T2 &    T3 &	T4 \\
\hline
``Process'' & .017 & .012 & .000 & .039* & .006 & .000 & .025* & .001 & .000 & .008 \\
\hline
``Tinker''     & .001 & .000 & .001 & .000 & .019 & .017 & .006 & .019 & .007 & .001 \\



\end{tabular}

    \caption{The eta squared ($\eta^2$) effect size for each of the 10 dependent variables for both ends of the Learning Style  spectrum.}
    
    \label{table:gender-facets}
\end{table}

==> tables/Learning/4-Learn-G5.tex <==
\begin{table}[h]
\centering

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}

Facet Value &	       F1 &	F2 &   F3 &	  F4 &	 F5 &	PU &   T1 &	 T2 &    T3 &	T4 \\
\hline
``Process'' & .007 & .033* & .011 & .029* & .027* & .000 & .004 & .023* & .000 & .005 \\
\hline
``Tinker''     & .013 & .014 & .062* & .010 & .000 & .004 & .000 & .005 & .004 & .020* \\



\end{tabular}

    \caption{The eta squared ($\eta^2$) effect size for each of the 10 dependent variables for both ends of the Learning Style  spectrum.}
    
    \label{table:gender-facets}
\end{table}

==> tables/Learning/5-Learn-G6.tex <==
\begin{table}[h]
\centering

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}

Facet Value &	       F1 &	F2 &   F3 &	  F4 &	 F5 &	PU &   T1 &	 T2 &    T3 &	T4 \\
\hline
``Process'' & .364*** & .401*** & .233** & .324*** & .381*** & .343*** & .409*** & .281*** & .336*** & .443*** \\
\hline
``Tinker''     & .127** & .116** & .065* & .167** & .201** & .191** & .326*** & .165** & .082* & .203** \\



\end{tabular}

    \caption{The eta squared ($\eta^2$) effect size for each of the 10 dependent variables for both ends of the Learning Style  spectrum.}
    
    \label{table:gender-facets}
\end{table}

==> tables/Learning/6-Learn-G7.tex <==
\begin{table}[h]
\centering

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}

Facet Value &	       F1 &	F2 &   F3 &	  F4 &	 F5 &	PU &   T1 &	 T2 &    T3 &	T4 \\
\hline
``Process'' & .193** & .205** & .234** & .338*** & .236** & .110** & .130** & .090* & .058* & .215** \\
\hline
``Tinker''     & .207** & .119* & .080* & .118** & .215** & .234** & .005 & .039* & .117* & .081* \\



\end{tabular}

    \caption{The eta squared ($\eta^2$) effect size for each of the 10 dependent variables for both ends of the Learning Style  spectrum.}
    
    \label{table:gender-facets}
\end{table}

==> tables/Learning/7-Learn-G8.tex <==
\begin{table}[h]
\centering

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}

Facet Value &	       F1 &	F2 &   F3 &	  F4 &	 F5 &	PU &   T1 &	 T2 &    T3 &	T4 \\
\hline
``Process'' & .235** & .078* & .072* & .045* & .218** & .126* & .064* & .028* & .142** & .134** \\
\hline
``Tinker''     & .227** & .030* & .003 & .108* & .182** & .186** & .045* & .047* & .073* & .102* \\



\end{tabular}

    \caption{The eta squared ($\eta^2$) effect size for each of the 10 dependent variables for both ends of the Learning Style  spectrum.}
    
    \label{table:gender-facets}
\end{table}

==> tables/Learning/8-Learn-G9.tex <==
\begin{table}[h]
\centering

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}

Facet Value &	       F1 &	F2 &   F3 &	  F4 &	 F5 &	PU &   T1 &	 T2 &    T3 &	T4 \\
\hline
``Process'' & .315*** & .173** & .066* & .260*** & .151** & .178** & .085* & .034* & .140** & .144** \\
\hline
``Tinker''     & .354*** & .087* & .114* & .260*** & .238** & .335*** & .076* & .022* & .253** & .304** \\



\end{tabular}

    \caption{The eta squared ($\eta^2$) effect size for each of the 10 dependent variables for both ends of the Learning Style  spectrum.}
    
    \label{table:gender-facets}
\end{table}

==> tables/Learning/9-Learn-G10.tex <==
\begin{table}[h]
\centering

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}

Facet Value &	       F1 &	F2 &   F3 &	  F4 &	 F5 &	PU &   T1 &	 T2 &    T3 &	T4 \\
\hline
``Process'' & .262*** & .165** & .078* & .217** & .144** & .172** & .122* & .087* & .162** & .139** \\
\hline
``Tinker''     & .155** & .035* & .006 & .098* & .061* & .048* & .026* & .027* & .059* & .050* \\



\end{tabular}

    \caption{The eta squared ($\eta^2$) effect size for each of the 10 dependent variables for both ends of the Learning Style  spectrum.}
    
    \label{table:gender-facets}
\end{table}

==> tables/Learning/91-Learn-G11.tex <==
\begin{table}[h]
\centering

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}

Facet Value &	       F1 &	F2 &   F3 &	  F4 &	 F5 &	PU &   T1 &	 T2 &    T3 &	T4 \\
\hline
``Process'' & .102* & .074* & .024* & .057* & .050* & .044* & .050* & .002 & .080* & .095* \\
\hline
``Tinker''     & .119* & .099* & .060* & .132** & .080* & .119* & .131** & .015 & .103* & .143** \\



\end{tabular}

    \caption{The eta squared ($\eta^2$) effect size for each of the 10 dependent variables for both ends of the Learning Style  spectrum.}
    
    \label{table:gender-facets}
\end{table}

==> tables/Learning/92-Learn-G12.tex <==
\begin{table}[h]
\centering

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}

Facet Value &	       F1 &	F2 &   F3 &	  F4 &	 F5 &	PU &   T1 &	 T2 &    T3 &	T4 \\
\hline
``Process'' & .000 & .000 & .008 & .000 & .001 & .003 & .012 & .004 & .024* & .000 \\
\hline
``Tinker''     & .000 & .003 & .015 & .022* & .028* & .055* & .000 & .000 & .016 & .005 \\



\end{tabular}

    \caption{The eta squared ($\eta^2$) effect size for each of the 10 dependent variables for both ends of the Learning Style  spectrum.}
    
    \label{table:gender-facets}
\end{table}

==> tables/Learning/93-Learn-G13.tex <==
\begin{table}[h]
\centering

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}

Facet Value &	       F1 &	F2 &   F3 &	  F4 &	 F5 &	PU &   T1 &	 T2 &    T3 &	T4 \\
\hline
``Process'' & .130** & .040* & .053* & .043* & .076* & .228** & .011 & .022* & .023* & .121* \\
\hline
``Tinker''     & .003 & .015 & .018 & .025* & .031* & .163** & .001 & .043* & .023* & .036* \\



\end{tabular}

    \caption{The eta squared ($\eta^2$) effect size for each of the 10 dependent variables for both ends of the Learning Style  spectrum.}
    
    \label{table:gender-facets}
\end{table}

==> tables/Learning/94-Learn-G14.tex <==
\begin{table}[h]
\centering

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}

Facet Value &	       F1 &	F2 &   F3 &	  F4 &	 F5 &	PU &   T1 &	 T2 &    T3 &	T4 \\
\hline
``Process'' & .044 & .001 & .018 & .097 & .085 & .049 & .026 & .043 & .049 & .038 \\
\hline
``Tinker''     & .148 & .047 & .040 & .084 & .043 & .110 & .005 & .060 & .072 & .050 \\



\end{tabular}

    \caption{The eta squared ($\eta^2$) effect size for each of the 10 dependent variables for both ends of the Learning Style  spectrum.}
    
    \label{table:gender-facets}
\end{table}


==> tables/Learning/95-Learn-G15.tex <==
\begin{table}[h]
\centering

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}

Facet Value &	       F1 &	F2 &   F3 &	  F4 &	 F5 &	PU &   T1 &	 T2 &    T3 &	T4 \\
\hline
``Process'' & .078 & .023 & .029 & .082 & .039 & .135 & .102 & .032 & .006 & .035 \\
\hline
``Tinker''     & .059 & .031 & .050 & .026 & .016 & .025 & .029 & .001 & .028 & .043 \\



\end{tabular}

    \caption{The eta squared ($\eta^2$) effect size for each of the 10 dependent variables for both ends of the Self Efficacy spectrum.}
    
    \label{table:gender-facets}
\end{table}

==> tables/Learning/96-Learn-G17.tex <==
\begin{table}[h]
\centering

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}

Facet Value &	       F1 &	F2 &   F3 &	  F4 &	 F5 &	PU &   T1 &	 T2 &    T3 &	T4 \\
\hline
``Process'' & .061 & .001 & .005 & .033 & .097 & .101 & .016 & .019 & .019 & .068 \\
\hline
``Tinker''     & .151 & .032 & .008 & .056 & .039 & .036 & .018 & .019 & .037 & .049 \\



\end{tabular}

    \caption{The eta squared ($\eta^2$) effect size for each of the 10 dependent variables for both ends of the Self Efficacy spectrum.}
    
    \label{table:gender-facets}
\end{table}

==> tables/Learning/97-Learn-G18.tex <==
\begin{table}[h]
\centering

\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}

Facet Value &	       F1 &	F2 &   F3 &	  F4 &	 F5 &	PU &   T1 &	 T2 &    T3 &	T4 \\
\hline
``Process'' & .047 & .079 & .011 & .039 & .028 & .040 & .020 & .008 & .026 & .035 \\
\hline
``Tinker''     & .016 & .016 & .000 & .021 & .003 & .012 & .000 & .001 & .021 & .011 \\



\end{tabular}

    \caption{The eta squared ($\eta^2$) effect size for each of the 10 dependent variables for both ends of the Self Efficacy spectrum.}
    
    \label{table:gender-facets}
\end{table}

==> tables/Risk/1-G1.tex <==
\begin{table}[h]
\centering

\begin{tabular}{c|c|c|c|c}

 &	\multicolumn{2}{c|}{\textbf{F5}}  &	\multicolumn{2}{c}{\textbf{PU}}  \\
\hline
$Diversity\ \eta^2$ &
\colorboxBackgroundForegroundText{AbiOrange}{black}{.091} & 
\colorboxBackgroundForegroundText{TimBlue}{black}{.004} & 
\colorboxBackgroundForegroundText{AbiOrange}{black}{.042} & 
\colorboxBackgroundForegroundText{TimBlue}{black}{.005} \\
\hline
$Aggregate\ \eta^2$ & \multicolumn{2}{c|}{.022}  &	\multicolumn{2}{c}{.015}  \\



\end{tabular}

    \caption{The eta squared effect size for each of the 10 dependent variables for both ends of the Self Efficacy spectrum.}
    
    \label{table:Risk-G1}
\end{table}

==> tables/Risk/2-G4-PostStrat.tex <==
\begin{table}[h]

%\framebox[\linewidth]{For Measuring!}
\centering
\footnotesize

    \begin{tabular}{p{0.22\columnwidth}|c|c|c|c|c|c|c}
    
    \rowcolor{LightGray}\multicolumn{8}{c}{\textbf{Violation AI Product}}\\
    \hline
    \textbf{Dependent}  & \textbf{Distance b/w} &  &  & & \textbf{Bonferroni} &  \\
    \textbf{variable} & \textbf{Means} &  \textbf{df} &  \textbf{t-val} &   \textbf{p-value}  & \textbf{correction} & \textbf{Cohen's \textit{d}} & \textbf{Pattern \#} \\
    \hline
    
    I would feel in control & 0.4444 & 61 &  1.6268 & .109 & 1 & 0.410 & \#2 \\
    \hline
    
    I would feel secure & 0.6667 & 62 & 2.3006 & \cellcolor{AbiOrangeQuote}{.0248*} & {.248} & 0.580 & \#3 \\
    \hline
    
    I would feel adequate & 0.8704 & 61 & 2.9179 & \cellcolor{AbiOrangeQuote}{.0049*} &  \cellcolor{AbiOrangeQuote}.049* & 0.743 & \#3 \\
    \hline
    
    I would feel certain & 1.2798 &  62 & 3.6258 & \cellcolor{AbiOrangeQuote}{.0005*} & \cellcolor{AbiOrangeQuote}.005* & 0.910 & \#3 \\
    \hline
    
    I would feel productive & 0.5397 & 62  & 2.2066 & \cellcolor{AbiOrangeQuote}.0311* & .311 & 0.556 & \#1 \\
    \hline
    
    I perceived it as useful &  0.5119 & 62  & 1.6623 & .102 & 1   & 0.419 & \#2\\
    \hline
    
    I would not be suspicious & 1.6468 & 34   & 4.8630  & \cellcolor{AbiOrangeQuote}$< .0001$* & \cellcolor{AbiOrangeQuote}$< .001$* & 1.337 & \#3  \\
    \hline
    
    It would not be harmful & 0.7893 & 39  & 2.8694  & \cellcolor{AbiOrangeQuote}.0066*  & .066   & 0.763 & \#3  \\
    \hline
    
    I find the product reliable & 0.6312 & 49 & 2.0046   & .051  & .510  & 0.518 & \#2 \\
    \hline
    
    I would trust the product & 0.7519 &  63  & 2.6615  & \cellcolor{AbiOrangeQuote}.010* & .100  & 0.664 & \#3 \\
    \hline
    
    
    
    
    \rowcolor{LightGray}\multicolumn{8}{c}{\textbf{Application AI Product}}\\
    \hline
    \textbf{Dependent}  & \textbf{Distance b/w} &  &  & & \textbf{Bonferroni} &  \\
    \textbf{variable} & \textbf{Means} &  \textbf{df} &  \textbf{t-val} &   \textbf{p-value}  & \textbf{correction} & \textbf{Cohen's \textit{d}} & \textbf{Pattern \#} \\
    \hline
    
    I would feel in control & 0.9643 & 62 &  3.2128  &  \cellcolor{AbiOrangeQuote}.0021*  & \cellcolor{AbiOrangeQuote}.021*  & 0.810 & \#2  \\
    \hline
    
    I would feel secure & 1.0093 & 61 & 3.1984 & \cellcolor{AbiOrangeQuote}{.0022}* & \cellcolor{AbiOrangeQuote}{.022*} & 0.814 & \#3\\
    \hline
    
    I would feel adequate & 0.8492 & 62 & 2.4955 & \cellcolor{AbiOrangeQuote}{.0153}* &  .153 & 0.629 & \#3\\
    \hline
    
    I would feel certain & 1.6916 &   63 & 4.7513 & \cellcolor{AbiOrangeQuote}{$<.0001$}* & \cellcolor{AbiOrangeQuote}{$<.001$}* & 1.186 & \#3\\
    \hline
    
    I would feel productive & 0.4598 & 63  & 1.8462  & .0696  & .696  & 0.461 & \#1  \\
    \hline
    
    I perceived it as useful &  0.7854 & 63  & 2.981  &  \cellcolor{AbiOrangeQuote}.0041*  & \cellcolor{AbiOrangeQuote}.041*   & 0.744  & \#2 \\
    \hline
    
    I would not be suspicious & 1.8008 & 42   & 5.1692  & \cellcolor{AbiOrangeQuote}$< .0001$* & \cellcolor{AbiOrangeQuote}{$<.001$}* & 1.364  & \#3 \\
    \hline
    
    It would not be harmful & 0.9607 & 44  & 3.1328  & \cellcolor{AbiOrangeQuote}.0031*  & \cellcolor{AbiOrangeQuote}.031*  & 0.821 & \#3 \\
    \hline
    
    I find the product reliable & 0.8170 & 50 & 2.6298  & \cellcolor{AbiOrangeQuote}.0113*  & .113  &  0.678 & \#2 \\
    \hline
    
    I would trust the product & 1.0635 &  62  & 3.7170  & \cellcolor{AbiOrangeQuote}.0004*  & \cellcolor{AbiOrangeQuote}.004*  & 0.937 & \#3
    
    
    \end{tabular}

    \caption{Guideline 4's t-test results %(\checkmark if Welch's t-test) 
    for risk-averse vs. risk-tolerant participants' average ratings of the independent Violation AI product (top) and Application AI product (bottom) for all 10 dependent variables.
    (Bonferroni corrections not strictly needed here, since the hypotheses were all stated up-front, but we include them for readers who crave them anyway.)
    The colorized cells show that, in this experiment it was always the \colorboxBackgroundForegroundText{AbiOrangeQuote}{black}{risk-averse} participants who had the significantly lower average ratings.
    }
    \label{tab:G4-Stats}

\end{table}

==> zz-Leftovers.tex <==
Li et al.'s stuff below


%\subsection{Independent and Confounding Variables}



% We assessed this impact under two AI performance conditions: optimal and sub-optimal. We treated AI performance as a confounding variable, because it added realism to the vignettes and enabled us to inquire whether guideline Application might be able to mitigate effects of sub-optimal AI performance on UX.

% We used compliance with the guideline as a within-subject factor, to collect evidence about how users compare products that apply or violate each guideline. AI performance served as a between-subject factor.

% In each factorial survey, we showed each respondent two vignettes. Both described interaction with almost identical AI products of the same level of AI performance. The product in one vignette applied the guideline [Product \textbf{A}] and the other violated the guideline [Product \textbf{V}]. The two vignettes were presented in random order.

% \subsection{Vignette Development}
% All vignettes described interactions with products from the productivity category: document and slide editors, search engines, email Applications, spreadsheet Applications. 
%We selected this category of products considering the severity of UX impact for guideline compliance and AI performance. 
%We reasoned that the UX impact might be unnoticeable for low-stakes products such as music recommenders, so we excluded the entertainment category. 
%We also excluded high-stakes products such as autonomous vehicles and healthcare Applications, which can lead to extreme harms and might need additional guidelines~\cite{guidelines_HAII}.

% Each vignette used the same three-part structure to describe interaction with an AI-powered feature:

% \textit{(1) Product and feature introduction.} A short statement introducing the fictional product and one of its AI-powered features that the user was described to interact with. Each fictional product was positioned as similar to multiple real products in the same category to help align it with the respondents' experience. The introduction included a user interaction with the product (e.g., ``When you do X, the product displays/does...''). The introductory statement was the same in all vignettes.

% \textit{(2) Product behavior description.} A statement describing the product's behavior under the guideline Application or Violation conditions. This statement was used to manipulate the independent variable.

% \textit{(3) AI performance description.} A statement about the product's performance, which was used to manipulate the confounding variable. The statements about AI performance were identical across all vignettes. For optimal  AI performance, the statement was: ``After using it for a few weeks, you notice that [Product Name] sometimes made mistakes, \textbf{but most of the time} worked well.'' For sub-optimal AI performance, it was: ``After using it for a few weeks, you notice that [Product Name] sometimes made mistakes, \textbf{and sometimes} worked well.''

% We used fictional, gender-neutral names (Kelso and Ione) to refer to the products in the vignettes in order to avoid the influence of brand loyalty and to make the vignettes realistic and the products easy to recall in the survey. The fictional names were randomized to avoid product preference due to names. The vignettes we used are included in \autoref{app:vignettes}.

% To illustrate, the vignettes used to manipulate compliance with \textsc{G1: Make clear what the system can do},  in the optimal AI performance condition, were:

% \smallskip
% \begin{quote}
% \textit{Application Vignette}\\
% You are using a presentation app similar to Microsoft PowerPoint, Google Slides, Apple Keynote to make slides for a presentation. It is called [Product Name]. [Product Name] has a capability called Presenter Coach that gives you feedback on your presentation skills as you practice your presentation in front of your computer.
% \end{quote}

% When you turn on Presenter Coach, it displays information like this:
% \begin{quote}
%     \smallskip

%     As you practice your presentation, we will give you feedback about your presentation style: how fast you speak, use of filler words (such as "um" and "like"), use of inappropriate words (such as "damn").

%      \smallskip
% \end{quote}
% After using it for a few weeks, you notice that [Product Name] sometimes made mistakes, but most of the time it worked well.

% \medskip
% \textit{Violation Vignette}\\
% You are using a presentation app similar to Microsoft PowerPoint, Google Slides, Apple Keynote to make slides for a presentation. It is called [Product Name]. [Product Name] has a capability called Presenter Coach that gives you feedback on your presentation skills as you practice your presentation in front of your computer.

% When you turn on Presenter Coach, it displays information like this:
% \begin{quote}
%     \smallskip

%     We will help you improve your presentation style.

%     \smallskip
% \end{quote}
% After using it for a few weeks, you notice that [Product Name] sometimes made mistakes, but most of the time it worked well.

% As we developed the vignettes, we followed recommended best practices to make them simple, clear, and realistic~\cite{Auspurg2009}. We illustrated some with images to facilitate understanding of the interaction described in the vignette. We took an iterative approach to developing them and piloted them as recommended by~\cite{Hughes2004}. We conducted two rounds of piloting. In the first round, we got qualitative feedback from 7 HCI researchers not familiar with the project on the vignettes' clarity, realism, and variable manipulation. We clarified the vignettes through several rounds of editing with the team, aiming for conciseness, consistency, realism, and clear manipulation of the variables. Based on the first pilot's results, we also shortened the dependent variable survey to eliminate items that did not apply, and decided to use fictional product names to facilitate the connection between the product described in the vignettes and the survey items. We then conducted a second pilot study with the updated vignettes on Amazon Mechanical Turk (MTurk). We added to the pilot study a survey that assessed the efficacy of the independent variable manipulation and the clarity of the vignettes' writing style. Each vignette was piloted with five participants, and no issues were identified at this stage. 

% \subsection{Dependent Variables}
% For each guideline, we collected data about product preference and impact on UX metrics. For product preference, the survey asked participants to choose which product they preferred and to provide their reasons in an open-ended field.
% We assessed impact on UX metrics by using survey questions adapted from published scales. The order of the questions was randomized for each vignette. We assessed UX metrics that fall into three major categories: feelings, trust, and metrics related to perceived product quality.

% \textit{Feelings.} Following the approach to feelings in UX in~\cite{benedek2002measuring}, we measured with 7-point Likert scales how guideline compliance influenced feeling in control, inadequate (reverse-coded), productive, secure, and uncertain (reverse-coded).

% \textit{Trust.} Trust plays an important factor in how much people accept and use smart systems~\cite{SHERIDAN1989427}. Jiun-Yin et al. identified 12 factors of trust between human and automated systems~\cite{trust_survey}. Considering the nature of our vignettes and the feedback from the 7 HCI researchers in the pilot study, we adopted four trust-related items, all measured with 7-point Likert scales, from~\cite{trust_survey}): trust, reliability, suspicion, and expectation of harm. The latter two were reversed coded. 

% \textit{Perceived product quality.} We also collected metrics related to perceived product quality and user acceptance: perceived usefulness, perception of product performance, behavioral intention to use the product, and Net Promoter Score (NPS) ~\cite{reichheld2011ultimate}. These metrics are known to be related to acceptance and use of AI-infused systems. The technology acceptance model (TAM)~\cite{10.2307/249008} suggests that when users are presented with a new technology, factors such as perceived usefulness (PU) and perceived ease-of-use (PEOU) influence their decision about how and when they will use it. Their general perception of the technology~\cite{perception} influences behavioral intent, which is a predictor of behavior~\cite{AJZEN1991179}. We excluded PEOU from our dependent variables because we found in the pilot studies it could not be assessed from reading a vignette.

% In addition to the survey items assessing the dependent variables, we also included three types of gate-keeping questions for each vignette's survey:

% \textit{Attention check.} We asked an attention check question to verify if the respondent read the vignette carefully before answering the dependent variable survey questions. The attention check asked about AI performance and also served as a manipulation check~\cite{aronson1998experimentation} for the confounding variable.

% \textit{Vignette comprehension.} We asked two questions to check if the participant was able to understand the vignette and whether the consequences of the product's behavior were indeed perceived as medium-stake.

% \textit{Manipulation check.} We asked two manipulation check~\cite{aronson1998experimentation} questions, one closed, and one open-ended, to verify that the respondent perceived the independent variable manipulation. The closed-ended manipulation check questions took the form of statements mirroring the text of the guidelines themselves. The open-ended manipulation check question asked participants to describe in their own words the difference between the two products.



%-------------
% \subsection{Participants \& Procedure}
 
% Li et al.'s participants were Amazon Mechanical Turk (MTurk) Human Intelligence Task (HIT) respondents with high acceptance rates in the United States over the age of 18, paid \$0.20 for participating and given a \$3 bonus if they completed the entire survey.


% \textit{Participant Screening.}
% Once workers accepted the HIT, they were presented with our institution's IRB consent form.
% Upon electronic agreement with the consent form, the worker was asked three screening questions.
% The first two questions asked about their experience with a type of productivity software described in the vignettes. 
% The third question asked the worker's age, to confirm participants were at least 18 years old, per IRB regulations.
% All crowd workers who completed the screening were paid \$0.20. We screened out workers with little or no experience with the type of product (e.g., used the product for less than one year, and less than once every few months).


% \textit{Factorial Survey.}
% Participants who qualified for the study were then shown  two vignettes. The vignettes were almost identical, except one violated a HAI guideline and the other applied it. Participants were asked to complete the survey questions about the dependent variables after reading each vignette.

% After finishing the survey questions for both vignettes, participants were asked to describe the differences between the two products, select which product they preferred, explain why, and fill out a questionnaire about demographic information and attitudes towards AI. This information about participants enabled us to monitor whether extreme attitudes towards AI might have influenced their answers. We used the attitudes towards AI items from~\cite{Zhang2019}. 



%------------

% \subsubsection{Open-ended questions}
% One of the authors analyzed the short answers to the two open-ended questions in the factorial surveys using thematic analysis~\cite{braunclarke2006}. The short answers to the question that asked participants to describe the difference between [Product A] and [Product V] were coded to check whether each participant perceived the independent variable manipulation (Yes/No). For example, the following is a comment that described the difference between the two products for \textsc{G1: Make clear what the system can do}: \textit{"[Product V] doesn't specifically state what features it has. It simply says that [Product V] would help me with my presentation. However, [Product A] does state that it will help me improve by giving me feedback on my use of filler words or profanity."} This comment captured the difference between the products and was coded as passing the manipulation check. 

% The other open-ended question asked the participants to provide reasons for their preference for the product from the two vignettes, [Product A], or [Product V].
% One of the authors read the open-ended answers provided in each factorial survey repeatedly, until codes began to emerge. Then, the codes were recorded and each comment was coded. Codes were mutually exclusive, so a comment counted towards only one code. Once codes were identified and all comments were coded, the same author merged codes into themes. Other team members conducted spot checks to verify the qualitative coding. The resulting themes for each guideline are listed in~\autoref{app:vignettes}.


% \subsubsection{User-eXperience (UX) Metrics}

% For the impacts on UX metrics, in addition to tests of significance, we also investigated effect sizes measured by the index generalized eta-squared~\cite{Olejnik2003GeneralizedEA}. 
% The American Statistical Association (ASA) released a statement~\cite{american2016american} that explicitly advised against drawing scientific conclusions based on P values alone.
% Eta-squared is a useful estimate of the percentage of variance accounted for by a variable--in our case, compliance with a guideline.

% Generalized eta-squared provides comparability across between-subjects and within-subjects designs ~\cite{Bakeman2005}. We categorized the effect sizes into four categories: unsubstantiated ($\eta_G^2<0.02$), small ($0.02\le\eta_G^2<0.13$), medium ($0.13\le\eta_G^2<0.26$), and large ($\eta_G^2\ge0.26$) using the thresholds recommended by Bakeman~\cite{Bakeman2005}.

% Because the factorial surveys for each guideline are independent of each other and used different vignettes, we have to consider each guideline's study in isolation and cannot perform comparisons across guidelines.
